Multi-channel Autobidding with Budget and ROI Constraints

In digital online advertising, advertisers procure ad impressions simultaneously on multiple platforms, or so-called channels, such as Google Ads, Meta Ads Manager, etc., each of which consists of numerous ad auctions. We study how an advertiser maximizes total conversion (e.g. ad clicks) while satisfying aggregate return-on-investment (ROI) and budget constraints across all channels. In practice, an advertiser does not have control over, and thus cannot globally optimize, which individual ad auctions she participates in for each channel, and instead authorizes a channel to procure impressions on her behalf: the advertiser can only utilize two levers on each channel, namely setting a per-channel budget and per-channel target ROI. In this work, we first analyze the effectiveness of each of these levers for solving the advertiser's global multi-channel problem. We show that when an advertiser only optimizes over per-channel ROIs, her total conversion can be arbitrarily worse than what she could have obtained in the global problem. Further, we show that the advertiser can achieve the global optimal conversion when she only optimizes over per-channel budgets. In light of this finding, under a bandit feedback setting that mimics real-world scenarios where advertisers have limited information on ad auctions in each channels and how channels procure ads, we present an efficient learning algorithm that produces per-channel budgets whose resulting conversion approximates that of the global optimal problem. Finally, we argue that all our results hold for both single-item and multi-item auctions from which channels procure impressions on advertisers' behalf.

==> 2_model_v0.tex <==
{\color{red} I think this section can be better structured. We keep switching between the global problem and each channel autobidding setting. Could we make it more structured? }
\textbf{Advertisers' conversion optimization problem in practice.} Consider an advertiser running a digital ad campaign to procure ad impressions on $M \in \N$ platforms such as Google Ads, Meta Ads Manager etc., each of which we call a \textit{channel}. Each channel requests from the advertiser  certain target procurement parameters and then procures impressions on behalf of the advertiser through autonomous programs (we call this programatic process \textit{autobidding}). In this work, we consider the setting where an advertiser is allowed to input \textit{at most} two channel-specific parameters for each channel $j \in [M]$ to convey her expectations for the channel's procurement performance, namely a channel ROI $0\leq \gamma_{j} < \infty$, and a channel budget $\rho_{j} \in [0,\rho]$ for some $\rho>0$. Then, the channel inputs these metrics in its autobidding algorithm to procure ads, and returns the total conversion $\totv_{j}(\gamma_{j},\rho_{j};\bm{z}_{j})\geq 0$ (e.g. number of clicks), as well as total spend $\totc_{j}(\gamma_{j},\rho_{j};\bm{z}_{j})\geq 0$ to the advertiser, where $\bm{z}_{j}$ is some randomness that originates from the procurement process in channel $j$; $\totv_{j}$, $\totc_{j}$ and $\bm{z}_{j}$ will be further specified later. {\color{red} the concept of ROI needs to be formally defined;  }

As the advertiser has the freedom of choice to input either per-channel ROI's, budgets, or both, we consider three options for the advertiser: 1. input only a per-channel ROI for each channel; 2. input only a per-channel budget for each channel; 3. input both per-channel ROI and budgets for each channel. Such options correspond to the following decision sets for $(\gamma_{j},\rho_{j})_{j\in [M]}$:
\begin{align}
\begin{aligned}
\label{eq:option}
    & \textbf{Per-channel budget only option: } \mathcal{I}_{\budg} = \{(\gamma_{j},\rho_{j})_{j\in [M]}\in \R_{+}^{2\times M}: \gamma_{j} = 0, \rho_{j}\in [0,\rho]\text{ for } \forall j\}\\
    & \textbf{Per-channel ROI only option: } \mathcal{I}_{\roi} = \{(\gamma_{j},\rho_{j})_{j\in [M]} \in \R_{+}^{2\times M}: \gamma_{j}\geq 0, \rho_{j} = \infty \text{ for } \forall j\}\\
    & \textbf{General option: }\mathcal{I}_{G} = \{(\gamma_{j},\rho_{j})_{j\in [M]}: \gamma_{j}\geq 0,\rho_{j}\in [0,\rho]\text{ for } \forall j\}
\end{aligned}
\end{align}
The advertiser's goal is to maximize total conversion of procured ad impressions, while subject to a \textit{ return-on-investment (ROI)} {\color{red} this should be discussed upfront. Also, you already used ROI abbreviation above} constraint that states total conversion across all channels is no less than $\gamma $ times total spend for some pre-specified ROI $0 < \gamma < \infty$, as well as a budget constraint that states total spend over all channels is no greater than the total budget $\rho\geq 0$. Mathematically, for any option $\mathcal{I} \in\{\mathcal{I}_{\budg} ,\mathcal{I}_{\roi} ,\mathcal{I}_{G}\}$, the advertiser's optimization problem can be written as {\color{red} the random variable $\matahbf z$ has not been defined yet. }
\begin{align}
\label{eq:chopt}
\begin{aligned}
   \textsc{CH-OPT}(\mathcal{I})=  \max_{(\gamma_{j},\rho_{j})_{j\in [M]}\in \mathcal{I}} ~&~ \sum_{j \in M} \E\left[\totv_{j}(\gamma_{j},\rho_{j};\bm{z}_{j})\right]\\
    \text{s.t. } &  \sum_{j \in M} \E\left[\totv_{j}(\gamma_{j},\rho_{j};\bm{z}_{j})\right] \geq \gamma \sum_{j \in M} \E\left[\totc_{j}(\gamma_{j},\rho_{j};\bm{z}_{j})\right]\\
   &   \sum_{j\in [M]}\rho_{j} \leq \rho
    \end{aligned}
\end{align}
where the expectation is taken w.r.t. randomness in $\bm{z}_{j}$.

The conversion and spend functions $(\totv_{j}, \totc_{j})$  as well as randomness $\bm{z}_{j}$ are specified by channel $j$'s autobidding behavior as well as the auctions mechanisms that sell impressions. In this work, we study a general autobidding procurement process where channel $j$ participates in $M_{j}\geq 2$ parallel ad auctions, each of which corresponds to the sale of an ad impression.\footnote{Ad auctions for each channel may be run by the channel itself or other external ad inventory suppliers such as web publishers.} {\color{red} our result also works for position auctions I assume. is that correct? If yes,let's clarify it.} Each ad auction $n\in [M_{j}]$ is associated with a value $v_{j,n}\geq 0$ that represents the expected conversion of the impression on sale, and a cost $d_{j,n}\geq 0$ which is required for the purchase of the impression; e.g. the cost in a single second-price auction is the highest competing bid of competitors in the market, and in a posted price auction the cost is simply the posted price by the seller of the impression. Writing $\bm{v}_{j} = (v_{j,n})_{n\in[M_{j}]}$ and $\bm{d}_{j} = (d_{j,n})_{n\in[M_{j}]}$, we assume that $\bm{z}_{j}:= (\bm{v}_{j},\bm{d}_{j})$ is sampled from some discrete distribution {\color{red} What is the exact information that is known to each channel? I am asking because it seems that implicitly it is assumed that there is a mechanism that convert $\rho_j$, $\gamma_j$, and perhaps the advertisers' values for different impressions to bids. We need to clarify this.  or at least we can say we abstract away from this because of XXX and YYY} $\bm{p}_{j}$ supported on some finite set $F_{j}\subseteq \R_{+}^{M_{j}} \times \R_{+}^{M_{j}}$. In hindsight, channel $j$'s autobidding optimization problem can be formulated as {\color{red} here it is assumed that the channel needs to solve this problem for any realization. We need to comment on this, explaining why this is OK and how this can be relaxed. }
\begin{align}
\begin{aligned}
\label{eq:budperchannelsol}
    \bm{x}_{j}^{*}(\gamma_{j},\rho_{j};\bm{z}_{j}) ~=~ \arg\max_{\bm{x}\in [0,1]^{M_{j}}} ~&~ \bm{v}_{j}^{\top} \bm{x}
     \text{s.t. }\quad   \bm{v}_{j}^{\top} \bm{x}\geq \gamma_{j}\quad \bm{d}_{j}^{\top} \bm{x} \bm{d}_{j}^{\top} \bm{x}\leq \rho_{j}
    \end{aligned}
\end{align} 
where $\bm{x}\in [0,1]^{M_{j}}$ denotes the vector of probabilities to win each of the parallel auctions, i.e. $x_{n}\in [0,1]$ is the probability to win auction $n\in [M_{j}]$ in channel $j$. Therefore, the corresponding conversion and spend functions are given by
\begin{align}
\begin{aligned}
\label{eq:budperchannel}
    & \totv_{j}(\gamma_{j},\rho_{j};\bm{z}_{j}) = \bm{v}_{j}^{\top} \bm{x}_{j}^{*}(\gamma_{j},\rho_{j};\bm{z}_{j})\quad \text{ and }\quad \totv_{j}(\gamma_{j},\rho_{j}) = \E[\totv_{j}(\gamma_{j},\rho_{j};\bm{z}_{j})] 
    \\ 
    & 
    \totc_{j}(\gamma_{j},\rho_{j};\bm{z}_{j}) = \bm{d}_{j}^{\top} \bm{x}_{j}^{*}(\gamma_{j},\rho_{j};\bm{z}_{j})  \quad \text{ and }\quad  \totc_{j}(\gamma_{j},\rho_{j}) = \E[ \totc_{j}(\gamma_{j},\rho_{j};\bm{z}_{j})]
    \,.
\end{aligned}
\end{align}
Here, the expectation is taken w.r.t. randomness in $\bm{z}_{j} = (\bm{v}_{j},\bm{d}_{j})$.

\textbf{The 
(hypothetical) advertiser optimization problem.} 
We note that the problem $\textsc{CH-OPT}(\mathcal{I})$ in Eq.\eqref{eq:chopt} represents an advertiser's optimization conversion goals in real-world scenarios, where the advertiser can only control for key input parameters (i.e. per-channel ROI and budget), and let channels procure ads on behalf of her. Here, we consider
a hypothetical setup where the advertiser has the authority to determine individual auctions across all channels from which she would like to procure ads. Mathematically, we define this hypothetical optimization problem as followed: {\color{red} try to better explain why this is hypothetical}
\begin{align}
\label{eq:glopt}
\begin{aligned}
\textsc{GL-OPT} ~=~\max_{\bm{x}_{1}\in [0,1]^{N_{1}} \ldots \bm{x}_{M}\in [0,1]^{N_{M}}} ~&~ \sum_{j\in [M]}\E\left[\bm{v}_{j}^{\top} \bm{x}_{j}\right] \\
     \text{s.t. } & \sum_{j\in [M]}\E\left[\bm{v}_{j}^{\top} \bm{x}_{j}\right]~\geq~ \gamma \sum_{j\in [M]} \E\left[\bm{d}_{j}^{\top} \bm{x}_{j}\right]\\
     & \sum_{j\in [M]} \E\left[\bm{d}_{j}^{\top} \bm{x}_{j}\right] ~\leq~\rho 
    \end{aligned}
\end{align} {\color{red} it is not clear why $M_j$ is not seen in the optimization problem. Also, somewhere we need to clarify $M_j$ is not a function of $\rho_j$ and $\gamma_j$}
where the expectation is taken w.r.t. randomness in $\bm{z} = (\bm{z}_{j})_{j\in [M]} = (\bm{v}_{j},\bm{d}_{j})_{j\in [M]}$ as well as the solutions $\bm{x} = (\bm{x})_{j\in[M]}$. 

\textbf{Key focuses and organization of this work.} In this paper, we address two key questions:
\begin{enumerate}
    \item For each of the advertiser options $\mathcal{I} \in\{\mathcal{I}_{\budg} ,\mathcal{I}_{\roi} ,\mathcal{I}_{G}\}$ defined in Eq. \eqref{eq:option}, what is the discrepancy between $\textsc{CH-OPT}(\mathcal{I})$, i.e. the optimal conversion an advertiser can achieve in practice, versus the hypothetical optimal $\textsc{GL-OPT}$? 
    \item Can advertisers develop efficient optimization algorithms to solve for $\textsc{CH-OPT}(\mathcal{I})$? 
\end{enumerate}
In Section \ref{sec:futil}, we address the first question to determine the gap between $\textsc{CH-OPT}(\mathcal{I})$ and $\textsc{GL-OPT}$ for different advertiser options. In Section \ref{sec:online}, we develop an efficient algorithm to solve for per-channel parameters that optimize $\textsc{CH-OPT}(\mathcal{I})$. 



% \subsection{Sequential multi-channel campaigns}
% In practice, advertisers generally run a series of campaigns sequentially on multiple channels to learn the optimal per-channel ROIs and budgets in light of Eq. \eqref{eq:chopt}. 
% Thus we extend our single campaign model introduced in Section \ref{subsec:singlecamp} to a sequential campaign model. 

% Consider an advertiser repeatedly running campaigns over $T$ periods on $M$ channels with a target ROI $\gamma \geq 1$ and total budget $\rho T$ for some $\rho \geq 0$. Here, each period for example corresponds to the duration of 1 hour or 1 day. At the beginning of period $t$, the advertiser sets per-channel target ROIs and budgets $(\gamma_{j,t},\rho_{j,t})_{j\in [M]}$, while simultaneously values and costs $(\bm{v}_{j,t}, \bm{d}_{j,t})\in \R_{+}^{M_{j}}\times \R_{+}^{M_{j}}$ are sampled (independently in each period) from some finite support $F_{j}$ associated with discrete distribution $\bm{p}_{j}$ in every channel $j \in [M]$. Each channel $j$ then takes as input $(\gamma_{j,t},\rho_{j,t})$ and procures ads on behalf of the advertiser, and returns  total conversion $\totv_{j,t}(\gamma_{j},\rho_{j})\geq 0$ as well as total spend $\totc_{j,t}(\gamma_{j},\rho_{j})\geq 0$ to the advertiser, where 

% Here, we highlight that the advertiser receives \textit{bandit feedback} from channels, i.e. the advertiser only knows the numerical values $\totv_{j,t}(\gamma_{j},\rho_{j})$ and $\totc_{j,t}(\gamma_{j},\rho_{j})$, but does not know 
% $\totv_{j,t}$ and $\totc_{j,t}$ evaluated at other per-channel ROI and budget pairs  $(\gamma_{j}',\rho_{j}')\neq (\gamma_{j},\rho_{j})$. 

% The advertiser's hindsight optimization problem if she could optimize decisions over all individual auctions and periods across channels is 
% \begin{align}
% \label{eq:gloptT}
% \begin{aligned}
%  % \textsc{GL-OPT}_{T} =  \E\left[\textsc{OPT}_{T}(\bm{v},\bm{d})\right] ~\text{ where  }~
%  \textsc{GL-OPT}_{T}(\bm{v}_{1:T},\bm{d}_{1:T}) ~=~\max_{\bm{x}_{1}\in [0,1]^{N_{1}} \ldots \bm{x}_{M}\in [0,1]^{N_{M}}} ~&~ \sum_{t\in[T]}\sum_{j\in [M]}\bm{v}_{j,t}^{\top} \bm{x}_{j,t}\\
%      \text{s.t. } & \sum_{t\in[T]}\sum_{j\in [M]}\bm{v}_{j,t}^{\top} \bm{x}_{j,t}\geq \gamma \sum_{t\in[T]}\sum_{j\in [M]} \bm{d}_{j,t}^{\top} \bm{x}_{j,t}\\
%      & \sum_{t\in[T]} \sum_{j\in [M]} \bm{d}_{j,t}^{\top} \bm{x}_{j} \leq \rho T
%     \end{aligned}
% \end{align}
% where the expectation is taken w.r.t. randomness in $\bm{v}_{1:T} = (\bm{v}_{j,t})_{j\in [M], t\in [T]}$ and  $\bm{d}_{1:T} = (\bm{d}_{j,t})_{j\in [M],t\in[T]}$.

% The sequential advertiser hindsight optimization problem in Eq. \eqref{eq:gloptT} relates to the single-campaign hindsight optimization problem in Eq. \eqref{eq:glopt} through the following proposition.
% \begin{proposition}
% \label{prop:ubsequentialbench}
% Recall the definitions of $\textsc{GL-OPT}$ and $\textsc{GL-OPT}$, respectively in Eq.\eqref{eq:glopt} and \eqref{eq:gloptT}, respectively. Then, we have
% \begin{align}
%     \E\left[\textsc{GL-OPT}_{T}(\bm{v}_{1:T},\bm{d}_{1:T})\right]
%     ~\leq~ T\cdot \textsc{GL-OPT}
%     \end{align}
% where the expectation is taken w.r.t. randomness in $(\bm{v}_{1:T},\bm{d}_{1:T})$ and $(\bm{v},\bm{d})$.
% \end{proposition}
% The advertiser's objective in this sequential multi-channel setup is to develop an online decision-making strategy that satisfies long-term ROI and budget constraints, namely 
% \begin{align}
% \begin{aligned}
% \label{eq:constraintT}
%  &  \text{ROI:} \quad  \E\left[\sum_{t\in[T]}\sum_{j \in M} \totv_{j}(\gamma_{j,t},\rho_{j,t})\right] \geq \gamma \left[ \sum_{t\in[T]}\sum_{j \in M} \totc_{j}(\gamma_{j,t},\rho_{j,t})\right]\\
%  & \text{Budget:} \quad  \E\left[\sum_{t\in[T]} \sum_{j\in [M]}\rho_{j,t}\right] \leq \rho T
%  \end{aligned}
% \end{align}
% while simultaneously minimizing total regret over $T$ periods, which is defined as
% \begin{align}
% \label{eq:regret}
%     \textsc{Reg}_{T} = \E\left[\textsc{OPT}_{T}(\bm{v}_{1:T},\bm{d}_{1:T})\right] -  \E\left[\sum_{t\in [T]}\sum_{j\in[M]}\totv_{j}(\gamma_{j,t},\rho_{j,t})\right]\,.
% \end{align}
% The expectations in Eq. \eqref{eq:constraintT} and \eqref{eq:regret} are taken w.r.t. randomness in $(\bm{v}_{1:T},\bm{d}_{1:T})$ and (possibly) $(\gamma_{j,t},\rho_{j,t})_{t\in[T]}$.


==> 4_online_exact.tex <==
\subsection{Extension to strict constraint satisfaction: UCB-SGD-II}
In Theorem \ref{thm:regret}, we showed that the final output of the UCB-SGD Algorithm \ref{alg:omducb} outputs a per-channel budget profile $\overline{\bm{\rho}}_{T} = \left(\frac{1}{T}\sum_{t\in[T]} \rho_{j,t}\right)_{j\in [M]}$ that satisfies both ROI and budget constraints in $\textsc{CH-OPT}(\mathcal{I}_{\budg})$ approximately, i.e. there can be at most violations in the magnitude of $\mathcal{O}(T^{-1/2})$ for both constraints. In this subsection, we present a modification to UCB-SGD that enables us to achieve no-constraint violations, while still maintaining the $\mathcal{O}(T^{-1/3})$ accuracy in total conversion. Similar modification techniques have been introduced in \cite{balseiro2022best,feng2022online}. 

Our modification strategy handles ROI and budget constraint satisfactions differently. For budget constraints, we simply maintain a budget balance $B_{t}$ in each period starting from $B_{1} = \rho T$, and decrease the balance by the expenditure in each period. When the balance nears 0, i.e. total spend comes close to $\rho T$, we simply terminate the algorithm. Regarding the ROI constraint, we develop two phases. Phase 1 is a ``safety phase'' where we conservatively utilize channel levers to accumulate a positive ``ROI balance'', i.e. in this phase (assume ending in period $T'$) we hope to achieve $\sum_{t\in [T']}g_{1,t} \geq \Theta(\sqrt{T})$, where we recall $g_{1,t}$ defined in step 4 of Algorithm \ref{alg:omducb} can be viewed as the ROI constraint violations in period $t$. For phase 2, we then naively run SGD-UCB. Here, we aim to have a positive ROI balance in phase 1 that will be used to  compensate possible constraint violations in phase 2 when we run SGD-UCB. 

We remark that in order to implement the safety phase to attain a positive ROI balance, we resort to per-channel ROIs $(\gamma_{j})_{j\in[M]}$, since setting $\gamma_{j} = \gamma$ for all channels will ensure that our ROI balance increases.\footnote{ Setting $\gamma_{j} = \gamma$ for all channels implies total realized conversion as at least $\gamma$ times spend, i.e. $\totv_{j}(\gamma, \rho_{j,t};\bm{z}_{j,t}) \geq \gamma \totv_{j}(\gamma, \rho_{j,t};\bm{z}_{j,t})$ due to Eq. \eqref{eq:budperchannelsol}. Hence the ROI balance, namely $g_{1,t} = \totv_{j}(\gamma, \rho_{j,t};\bm{z}_{j,t})  - \gamma \totv_{j}(\gamma, \rho_{j,t};\bm{z}_{j,t})$ is nonnegative, and thus in phase 1 the cumulative ROI balance increases in each period.} From a high level,  SGD-UCB attempts to approximate the optimal solution for $\textsc{CH-OPT}(\mathcal{I}_{\budg})$ by solely using the per-channel budget lever, whereas in the above modification with the usage of per-channel ROIs hopes to approximate an optimal solution to 
$\textsc{CH-OPT}(\mathcal{I}_{G})$ 
for the general option (see Eq. \eqref{eq:option}) which is inspired by the fact that  $\textsc{CH-OPT}(\mathcal{I}_{G}) = \textsc{CH-OPT}(\mathcal{I}_{\budg})=\textsc{GL-OPT}$ according to Lemma \ref{cor:roiredund} and Corollary \ref{cor:roiredund}. We call this modified algorithm SGD-UCB-II, and summarize details in Algorithm \ref{alg:omducb2}. 

\begin{algorithm}[H]
    \centering
    \caption{SGD-UCB-II}\label{alg:omducb2}
    \footnotesize
    \begin{algorithmic}[1]
    \Require{Set $B_{1}=0$, and $g_{1,0} = 0$, ROI buffer $\beta > 0$} 
    \phase{Accumulate ROI buffer}
    \While{$\sum_{t' \in [t-1]}g_{1,t'} \leq \sqrt{T}\log(T)$}
    \If{$B_{t} + M\rho  > \rho T$}
         \State Terminate  algorithm and output $\overline{\bm{\rho}} = \left(\frac{1}{T}\sum_{t'\in[t]} \rho_{j,t'}\right)_{j\in [M]}$ and $\overline{\bm{\lambda}}  =  \left(\frac{1}{T}\sum_{t'\in[t]} \lambda_{j,t'}\right)_{j\in [M]}$.
    \EndIf
    \State  Set $\gamma_{j,t} = \gamma + \beta$ and $\rho_{j,t} = \beta$ for all $j \in [M]$ 
    \State Observe conversion and costs $\totv_{j}(\gamma+\beta, \rho;\bm{z}_{t}),\totc_{j}(\gamma+\beta, \beta;\bm{z}_{t}) $ for all channels $j \in [M]$. Calculate
    \begin{align*}
        g_{1,t} = \sum_{j \in M} \left(\totv_{j}(\gamma_{j,t}, \rho_{j,t};\bm{z}_{t}) -  \gamma \cdot \totc_{j}(\gamma_{j,t}, \rho_{j,t};\bm{z}_{t})\right)\,.
    \end{align*}
    \State Calculate $B_{t+1} = B_{t} + \sum_{j\in [M]}\rho_{j,t}$.
    \State Increment $t \leftarrow t+1$
	\EndWhile
 \State Denote end period of Phase 1 as $T_{1} = t-1$.
 \phase{Run SGD-UCB}
 \State For remaining $T - T_{1}$ periods, run SGD-UCB  in Algorithm \ref{alg:omducb} with a spend balance check during each period $t$:
 \If{$B_{t} + M\rho  > \rho T$}
 \State Terminate and output 
 $\overline{\bm{\rho}} = \left(\frac{1}{T}\sum_{t'\in[t]} \rho_{j,t'}\right)_{j\in [M]}$ and $\overline{\bm{\lambda}}  =  \left(\frac{1}{T}\sum_{t'\in[t]} \lambda_{j,t'}\right)_{j\in [M]}$ where  $\lambda_{j,t'} = 0$ for any $t'> T_{1}$.
 \Else 
 \State Set per-channel budgets $\{\rho_{j,t}\}_{j\in[M]}$ according to SGD-UCB, and set per-channel ROI $\gamma_{j,t} = 0$ for all channels. 
 \State Update spend balance $B_{t+1} = B_{t} + \sum_{j\in [M]}\rho_{j,t}$.
 \EndIf
    \end{algorithmic}
\end{algorithm}



\begin{lemma}[Bounding length of Phase 1]
\label{lem:boundphase1}
Recall $T_{1}$ is the end period of Phase 1 in the SGD-UCB-II algorithm (see step 10). Denote the event $\mathcal{E} = \{T_{1}\geq 2\sqrt{T}\log^{3}(T)\}$, and take ROI buffer $\beta = \frac{1}{\log(T)}$ in the SGD-UCB-II algorithm.  Then, under Assumption \ref{ass:feas}, for large enough $T$ we have $\prob\left(\mathcal{E}\right)\leq \frac{1}{T}$. 
\end{lemma}

\textit{Proof.}

\begin{claim}
\label{clm:smallbudgetbinding}
Assume Assumption \ref{ass:channelfeas} holds. Let $\beta = \frac{1}{\log(T)}$ and assume the global ROI target $\gamma > 0$ is independent of $T$. For large enough $T$, the per-channel optimization problem in Eq. \eqref{eq:budperchannelsol} w.r.t. per-channel ROI $\gamma + \beta$ and per-channel budget $\beta$ is budget binding, i.e. $D_{j}(\gamma + \beta, \beta; \bm{z}_{j}) = \beta$
\end{claim}


Consider the hypothetical version of SGD-UCB-II where we ignore the budget balance condition $B_{t}< M\rho$ in step 2 of the algorithm, and terminate phase 1 only when 
 the condition $\sum_{t' \in [t-1]}g_{1,t'} \leq \sqrt{T}\log(T)$ in Step 1 holds. Denote this hypothetical stopping time 
as $\widetilde{T}_{1}$, defined to be 
\begin{align}
\label{eq:fakeT1}
\begin{aligned}
    \widetilde{T}_{1} = \min\Big\{t\in [T]:\sum_{t' \in [t]}  \underbrace{\sum_{j \in M} \left(\totv_{j}(\gamma+\beta, \rho;\bm{z}_{t'}) -  \gamma \cdot \totc_{j}(\gamma+\beta, \rho;\bm{z}_{t'})\right)}_{:=h_{t'}} > \sqrt{T}\log(T)\Big\}
    \end{aligned}
\end{align}
It is easy to see that with probability 1,  we have $\widetilde{T}_{1} \geq T_{1}$ where we recall  $T_{1}$ is the real stopping time of Phase 1 in SGD-UCB-II. Hence we have 
\begin{align}
\label{eq:usefakeT1}
    \prob\left(T_{1}\geq R\right) \leq  \prob\left(\widetilde{T}_{1}\geq R\right)
\end{align}
Now, it is not difficult to see $\{h_{t}\}_{t}$ where $h_{t}$ defined in  Eq. \eqref{eq:fakeT1} are i.i.d. random variables, since the only randomness comes from the realization of value-cost pairs $\{\bm{z}_{t}\}_{t\in[T]}$ which are i.i.d.. Further, by definition of conversion and spend functions $\totv_{j},\totc_{j}$ defined in Eq. \eqref{eq:budperchannelsol},  and \eqref{eq:budperchannel}, for any $t \in [T]$ we have 
\begin{align}
\label{eq:Elower}
\begin{aligned}
    & \sum_{j \in M} \left(\totv_{j}(\gamma+\beta, \rho;\bm{z}_{t}) -  (\gamma + \beta) \cdot \totc_{j}(\gamma+\beta, \rho;\bm{z}_{t})\right)\overset{(i)}{\geq} 0 \\
    ~\Longrightarrow~& h_{t} :=  \sum_{j \in M} \left(\totv_{j}(\gamma+\beta, \rho;\bm{z}_{t}) -  \gamma \cdot \totc_{j}(\gamma+\beta, \rho;\bm{z}_{t})\right) \\
    & \quad \geq \beta \sum_{j \in M}\totc_{j}(\gamma+\beta, \rho;\bm{z}_{t})\overset{(ii)}{\geq} \beta M \underline{D}\\ 
    ~\Longrightarrow~& \Bar{h}:= \E[h_{t}] \geq \beta M \underline{D} > 0
    \end{aligned}
\end{align}
where (i) follows from the fact that when we input per-channel target ROI $\gamma + \beta$ to each channel, the realized ROI for that channel will be at least $\gamma + \beta$; in (ii) we defined 
$ \underline{D} = \min_{j\in [M]} \min_{\bm{z}_{j}\in F_{j}} \totc_{j}(\gamma+\beta, \rho;\bm{z}_{j}) > 0 $ where the inequality follows from Assumption \ref{ass:feas} such that there is at least 1 channel's optimization problem is feasible with per-channel ROI $\gamma + \beta = \gamma + \frac{1}{\log(T)}$ for large enough $T$; in the final inequality we let $ \Bar{h}$ be the mean of the i.i.d. random variables $\{h_{t}\}_{t\in [T]}$.

We note that $\widetilde{T}_{1}> R$ implies that the sum of the first $R$ $h_{t}$'s do not exceed $\sqrt{T}\log(T)$ (see definition of $\widetilde{T}_{1}$ in Eq. \eqref{eq:fakeT1}), hence we have 
\begin{align}
\label{eq:boundfakeT1}
\begin{aligned}
    \prob\left(\widetilde{T}_{1} > R \right) ~\leq~ &   
   \prob\left(\sum_{t =1}^{\lceil R\rceil} h_{t} \leq  \sqrt{T}\log(T)\right)\\
   ~=~ &   
   \prob\left(\sum_{t =1}^{\lceil R\rceil} (h_{t} -\Bar{h})\leq  \sqrt{T}\log(T) - \lceil R\rceil \cdot \Bar{h}\right)\\
    ~\overset{(i)}{\leq}~ &   \prob\left(\sum_{t =1}^{\lceil R\rceil} (h_{t} -\Bar{h})\leq  \sqrt{T}\log(T) - R\beta M\underline{D}\right) \\
     ~\overset{(ii)}{=}~ &   \prob\left(\sum_{t =1}^{\lceil R\rceil} (h_{t} -\Bar{h})\leq  -\sqrt{T}\log(T) \right) \\
      ~\overset{(iii)}{\leq}~ &   \exp\left(-\frac{T\log^{2}(T)}{2\lceil R\rceil M^{2}\Bar{\totv}^{2}}\right)\\
       ~\overset{(iv)}{\leq}~ &   \frac{1}{T}
\end{aligned}
\end{align}
Here (i) follows from $\Bar{h}\geq \beta M \underline{D}$ in Eq. \eqref{eq:Elower}; (ii) follows from the definition that $R = 2\sqrt{T}\log^{3}(T)$ and $\beta = \frac{1}{\log(T)}$ so  $R\beta M \underline{D} = 
2M \underline{D} \sqrt{T}\log^{2}(T) 
\geq 2\sqrt{T}\log(T) $ for large enough $T$ such that $\log(T) > \frac{1}{M\underline{D}}$; (iii) follows from Azuma Hoefding's inequality given that $h_{t} \in [0, M\Bar{\totv}]$ for any $t\in [T]$; and finally (iv) follows from $T\geq \lceil R\rceil$, and $\log(T) >  M^{2}\Bar{\totv}^{2}$ for large enough $T$. 
Hence, combining Eq. \eqref{eq:boundfakeT1} and \eqref{eq:usefakeT1} yields the desired statement of the lemma. 
\halmos

\begin{assumption}[Strictly feasible per-channel ROI constraints]
\label{ass:channelfeas}
Fix any channel $j\in [M]$ and any realization of value-cost pairs  $\bm{z}_{j} =(\bm{v}_{j},\bm{d}_{j}) \in F_{j}$, the channel's optimization problem in Eq. \ref{eq:budperchannelsol} is strictly feasible, i.e. the set $\left\{\bm{x}_{j} \in [0,1]^{m_{j}}: \bm{v}_{j}^{\top} \bm{x}_{j} > \gamma\bm{d}_{j}^{\top}\bm{x}_{j}\right\}$ is nonempty.\footnote{Equivalently, for any realization of value-cost pairs  $\bm{z}_{j} = (\bm{v}_{j},\bm{d}_{j})$ there always exists an auction $n\in [m_{j}]$ in this channel  whose value-to-cost ratio is at least $\gamma$, i.e. $v_{j,n} >  \gamma d_{j,n}$.}
\end{assumption}

Our main result in this subsection is the following Theorem \ref{thm:regret2}:
\begin{theorem}
\label{thm:regret2}
    Let $T_{2} \in [T]$ be the termination period of SGD-UCB-II, and recall
    $\overline{\bm{\rho}} = \left(\frac{1}{T}\sum_{t\in[T_{2}]}\rho_{j,t}\right)_{j\in [M]}$ and  $\overline{\bm{\lambda}} = \left(\frac{1}{T}\sum_{t\in[T_{2}]}\rho_{j,t}\right)_{j \in [M]}$ are the final outputs of  SGD-UCB-II in Algorithm \ref{alg:omducb2}. Then under Assumptions \ref{ass:budgetbind} and \ref{ass:channelfeas} and the same SGD-UCB parameter choices in Theorem \ref{thm:regret}, for large enough $T$ we have 
    $ \textsc{GL-OPT} - \sum_{j \in [M]}\E\left[\totv_{j}(\overline{\gamma}_{j},\overline{\rho}_{j})\right]\leq \mathcal{O}(T^{-1/3})$, and further $\sum_{j \in [M]}\E\left[\totv_{j}(\overline{\gamma}_{j},\overline{\rho}_{j}) -\gamma \totc_{j}(\overline{\gamma}_{j},\overline{\rho}_{j})\right]\geq 0 $ and $ \sum_{j \in [M]} \E\left[\totc_{j}(\overline{\gamma}_{j},\overline{\rho}_{j})\right]\leq \rho$. 
\end{theorem}

\textit{Proof.}


\textbf{Part I. Bounding global budget constraint violation.}

\begin{align}
    \sum_{j\in [M]}\totc_{j}(\Bar{\gamma}_{j},\Bar{\rho}_{j}) \overset{(i)}{\leq}\sum_{j}\totc_{j}(0,\Bar{\rho}_{j}) \leq \Bar{\rho}_{j} = \frac{1}{T}\sum_{t\in [T_{2}]}\sum_{j\in [M]} \rho_{j,t} \overset{(ii)}{<}\rho \,.
\end{align}
Here (i) is due to the fact that for any value-cost realization $\bm{z}_{j}$, per-channel budget $\rho_{j}\in [0,\rho]$ and per-channel ROI $\gamma_{j} \geq 0$, we have
$\totc_{j}(\gamma_{j},\rho_{j};\bm{z}_{j}) \leq \totc_{j}(0,\rho_{j};\bm{z}_{j}) $, since we are effectively ignoring the per-channel ROI constraint in $ \totc_{j}(0,\rho_{j};\bm{z}_{j})$, so this also holds in expectation w.r.t. randomness in $\bm{z}_{j}$;  (ii) is due to the design of SGD-UCB so that the per-channel budget decisions never sum up to exceed $\rho T - M\rho $.

\textbf{Part II. Bounding global ROI constraint violation.}

Recall the event $\mathcal{E} = \{T_{1}\geq 2\sqrt{T}\log^{3}(T)\}$ defined in Lemma \ref{lem:boundphase1} where $T_{1}$ is the end period of Phase 1 in the SGD-UCB-II algorithm (see step 10). We consider two scenarios, namely when event $\mathcal{E}$ holds and doesn't hold. Recall $g_{1,t} = \sum_{j\in[M]}\left(\totv_{j}(\gamma_{j,t},\rho_{j,t};\bm{z}_{t}) - \gamma \totc_{j}(\gamma_{j,t},\rho_{j,t};\bm{z}_{t})\right)$

When event $\mathcal{E} $ holds, then 
\begin{align}
\begin{aligned}
\label{eq:badeventroi}
    % & \E\left[T_{2}\cdot  \textsc{GL-OPT} - \sum_{t\in [T_{2}]}\sum_{j\in[M]}\totv_{j}(\gamma_{j,t},\rho_{j,t}) ~\Big |~ \mathcal{E}\right] \overset{(i)}{\leq}  \textsc{CH-OPT}(\mathcal{I}_{G}) \leq M\Bar{V} T\\
    & \E\left[\sum_{t\in [T_{2}]}g_{1,t} ~\Big |~ \mathcal{E}\right] 
 \geq - T\gamma M\rho
 % \\
 %  & \E\left[\sum_{t\in [T_{2}]}\sum_{j\in[M]}\totc_{j}(\gamma_{j,t},\rho_{j,t}) ~\Big |~ \mathcal{E}\right] 
 % \leq M \rho T\,. 
 \end{aligned}
\end{align}

When event  $\mathcal{E} $ does not hold, Phase 1 terminates within  the first $2\sqrt{T}\log^{3}(T)$ periods, i.e.
$T_{1} < 2\sqrt{T}\log^{3}(T)$, and the total spend balance in Phase 1 is at most 
\begin{align*}
    \sum_{t\in [T_{1}]} \sum_{j\in [M]}\rho = M\rho T_{1} <  2M\rho\sqrt{T}\log^{3}(T) < \rho T - \rho M
\end{align*}
where the final inequality holds for large enough $T$. This implies that Phase 1 terminates because the ROI buffer condition in step 1 is met, i.e. 
\begin{align}
\label{eq:goodeventroi1}
    \sum_{t\in [T_{1}]} g_{1,t}> \sqrt{T}\log(T)
\end{align}
Now in periods $t = T_{1}+1 \dots T_{2}$, following the proof of Lemma \ref{lem:approxconst}, we have
\begin{align}
\label{eq:goodeventroi2}
    \sum_{t = T_{1}+1}^{T_{2}}g_{1,t} \geq \frac{1}{\eta} \left(\lambda_{T_{1}} - \lambda_{T_{2}}\right) \overset{(i)}{\geq} -\frac{\dualub_{F}}{\eta} = \dualub_{F} \sqrt{T}
\end{align}
we (i)  follows from $ 0\leq \lambda_{t} \leq \dualub_{F}$ for any $t\in [T]$ for some absolute constant $\dualub_{F} >0$ that only depends on the support of value-cost pairs $F = F_{1}\times \ldots \times F_{M}$. Hence, combining Eq. \eqref{eq:badeventroi}, \eqref{eq:goodeventroi1}, \eqref{eq:goodeventroi2}, we have
\begin{align}
\begin{aligned}
      & \sum_{j\in [M]}\left(\totv_{j}(\Bar{\gamma}_{j},\Bar{\rho}_{j};\bm{z}_{t})  - \gamma \totc_{j}(\Bar{\gamma}_{j},\Bar{\rho}_{j};\bm{z}_{t}) \right) \\
      ~\geq~ & \sum_{j\in [M]}\left(\totv_{j}(\Bar{\gamma}_{j},\Bar{\rho}_{j};\bm{z}_{t})  - \gamma \totc_{j}(0,\Bar{\rho}_{j};\bm{z}_{t}) \right) \\
      ~\overset{(i)}{=}~& \sum_{j\in [M]}\left(\totv_{j}(\Bar{\gamma}_{j},\Bar{\rho}_{j};\bm{z}_{t})  - \gamma \Bar{\rho}_{j}) \right) \\
       ~\overset{(ii)}{\geq}~& \frac{1}{T}\sum_{t\in [T_{2}]}\sum_{j\in [M]}\left(\totv_{j}(\gamma_{j,t},\rho_{j,t};\bm{z}_{t})  - \gamma \rho_{j,t}) \right) \\
        ~=~& \frac{1}{T}\sum_{j\in [M]}\left(\sum_{t\in [T_{1}]}\left(\totv_{j}(\gamma +\beta ,\beta;\bm{z}_{t})  - \gamma \beta) \right) +  \sum_{t=T_{1}+1}^{T_{2}}\left(\totv_{j}(0,\rho_{j,t};\bm{z}_{t})  - \gamma \rho_{j,t}) \right)\right)\\
         ~\overset{(iii)}{=}~& \frac{1}{T}\sum_{j\in [M]}\left(\sum_{t\in [T_{1}]}\left(\totv_{j}(\gamma +\beta ,\beta;\bm{z}_{t})  - \gamma \totc_{j}(\gamma +\beta ,\beta;\bm{z}_{t})) \right) +  \sum_{t=T_{1}+1}^{T_{2}}\left(\totv_{j}(0,\rho_{j,t};\bm{z}_{t})  - \gamma \rho_{j,t}) \right)\right)
\end{aligned}
\end{align}

\textbf{Part III. Bounding estimation error.}
Similar to the proof of Theorem \ref{thm:regret}, we only need to bound
$T_{2}\cdot  \textsc{GL-OPT} - \E\left[\sum_{t\in [T_{2}]}\sum_{j\in[M]}\totv_{j}(\gamma_{j,t},\rho_{j,t})\right] $


We first show that $T - T_{2}\leq $


\begin{align}
    \sum_{t\in [T_{2}]}\sum_{j\in[M]}\totv_{j}(\gamma_{j,t},\rho_{j,t})
\end{align}
\halmos


We conclude with the insight that if satisfying ROI and budget constraints approximately as in Theorem \ref{thm:regret} for the UCB-SGD algorithm is acceptable, then considering the per-channel budget lever along would suffice. Yet, when advertisers hope to respect constraints strictly, advertisers may need resort to the per-channel ROI lever unde the UCB-SGD-II framework.

==> 4_online_v0.tex <==
In this section, we develop an efficient algorithm to solve for per-channel budgets that optimize
$\textsc{CH-OPT}(\I_{\budg})$ defined in Eq. \eqref{eq:chopt}, which achieves the theoretical optimal conversion, namely $\textsc{GL-OPT}$, as illustrated in Theorem \ref{thm:budgonlysuff}. In particular, we consider algorithms that run over $T > 0$ periods, where each period for example corresponds to the duration of 1 hour or 1 day. At the end of $T$ periods, the algorithm  produces some per-channel budget profile $(\rho_{j})_{j\in [M]}\in [0,\rho]^{M}$ that approximates $\textsc{CH-OPT}(\I_{\budg})$,  and satisfies aggregate budget and ROI constraints, namely 
\begin{align}
\begin{aligned}
\label{eq:constraintT}
 &  \text{ROI:} \quad  \sum_{j \in M} \totv_{j}(\rho_{j}) \geq \gamma \sum_{j \in M} \totc_{j}(\rho_{j}), ~\text{ and }~ \text{Budget:} \quad  \sum_{j\in [M]}\totc_{j}(\rho_{j})\leq \rho\,,
 \end{aligned}
\end{align}
where we recall the expected conversion and spend functions $(\totv_{j}(\rho_{j}),\totc_{j}(\rho_{j}))$ defined in Eq. \eqref{eq:budperchannel}.

The algorithm proceeds as follows: at the beginning of period $t\in [T]$, the advertiser sets per-channel budgets $(\rho_{j,t})_{j\in [M]}$, while simultaneously values and costs $\bm{z}_{t}=(\bm{v}_{j,t}, \bm{d}_{j,t})\in \R_{+}^{M_{j}}\times \R_{+}^{M_{j}}$ are sampled (independently in each period) from  finite support $F = F_{1}\times \dots F_{M}$ according to discrete distributions $(\bm{p}_{j})_{j\in[M]}$. Each channel $j$ then takes as input $\rho_{j,t} \in [0,\rho]$ and procures ads on behalf of the advertiser, and reports the total realized conversion $\totv_{j}(\rho_{j,t};\bm{z}_{t})$ as well as total spend $\totc_{j}(\rho_{j,t};\bm{z}_{t}) $ to the advertiser, where $\totv_{j}(\rho_{j,t};\bm{z}_{t})$ and $\totc_{j}(\rho_{j,t};\bm{z}_{t})$ are defined in Eq. \eqref{eq:budperchannel}. For simplicity we also assume for any realization $\bm{z} = (\bm{v}_{j},\bm{d}_{j}) \in F$ we have the ordering $\frac{v_{j,1}}{d_{j,1}} > \frac{v_{j,2}}{d_{j,2}} > \dots  > \frac{v_{j,m_{j}}}{d_{j,m_{j}}}$ for all channels $j \in [M]$.

Here, we highlight that the advertiser receives \textit{bandit feedback} from channels, i.e. the advertiser only observes the numerical values $\totv_{j}(\rho_{j,t}; \bm{z}_{t})$ and $\totc_{j}(\rho_{j,t}; \bm{z}_{t})$, but does not get to observe 
$\totv_{j}(\rho_{j}'; \bm{z}')$ and $\totc_{j}(\rho_{j}'; \bm{z}')$ evaluated at any other per-channel budget $\rho_{j}'\neq \rho_{j,t}$ and realized value-cost pairs $\bm{z}'\neq \bm{z}_{t}$. More discussions on challenges that arise from this bandit feedback structure can be found in 
Section \ref{subsec:algo}.

% \begin{algorithm}[H]
%     \centering
%     \caption{Explore-exploit under noisy bandit feedback}\label{alg:ee}
%     \footnotesize
%     \begin{algorithmic}[1]
%     \Require Exploration length $E$, budget discretization $\discerr > 0$ s.t. $\budgset = \{\budg_{h}\}_{h\in \left[{\rho}/{\discerr}\right]}$ where $\budg_{h} = h\discerr$. Stepsizes $\{\eta\}_{t\in[T]}$.
% {\Statex{\textbf{Exploration}}}:
%     \For{$h \in \left[\frac{\rho}{\discerr}\right]$ and $j\in [M]$}
%         \State Set budget $\budg_{h}$ for $E$ periods in channel $j$, and record empirical channel value $\Bar{\totv}_{j}(\budg_{h})$
%     \EndFor
%     {\Statex{\textbf{Exploitation}}}:
% 	\For{$t = EM  \left[{\rho}/{\discerr}\right]\dots T$ }
% 	 \State For each channel $j\in [M]$ set primal decision
%         \begin{align}
%           \rho_{j,t} = \arg\max_{\rho_{j}\in \budgset}\quad (1+\lambda_{t})\Bar{\totv}_{j}(\rho_{j}) - \left(\lambda_{t} \gamma + \mu_{t} \right)\rho_{j} 
%           \end{align}
%     \State Update dual variables
%         with realized values $\left\{\widetilde{\totv}_{j}(\rho_{j,t}) \right\}_{j \in [M]}$
%         \begin{align}
%         & \lambda_{t+1} =\lambda_{t} - \eta \cdot \left(\sum_{j \in M} \widetilde{\totv}_{j} -  \gamma \rho_{j,t}\right)\\
%         &  \mu_{t+1}  = \mu_{t} - \eta \cdot \left(\rho - \sum_{j\in [M]} \rho_{j,t}\right)
%         \end{align}
% 	\EndFor
%     \end{algorithmic}
% \end{algorithm}

We also make the following Assumption \ref{ass:budgetbind} that states that if the advertiser allocates any feasible per-channel budget to a channel $j\in [M]$, the channel will almost surely deplete the entire budget in the impression procurement process. This is a natural assumption that mimics practical scenarios, e.g. small businesses who have moderate-sized budgets.
\begin{assumption}[Moderate budgets]
\label{ass:budgetbind}
 We assume the total budget is finite, i.e. $\rho < \infty$, and for any channel $j \in [M]$, value-cost realization $\bm{z} = (\bm{v}, \bm{d}) \in F_{j}$, and per-channel budget $\rho_{j} \in [0,\rho]$, the optimal solution $\bm{x}_{j}^{*}(\rho;\bm{z})$ defined in Eq. \eqref{eq:budperchannelsol} is budget binding, i.e. $\totc_{j}(\rho_{j};\bm{z}) = \bm{d}_{j}^{\top}\bm{x}_{j}^{*}(\rho_{j};\bm{z}) = \rho$.
\end{assumption}
% Under Assumption \ref{ass:budgetbind}, we can show that the total spend in each channel exactly matches the input per-channel budget, and we present the proof in Appendix \ref{pf:prop:budgetbind} 
% \begin{proposition}
% \label{prop:budgetbind}
% Under Assumption \ref{ass:budgetbind}, for any channel $j\in [M]$ and per-channel budget $\rho_{j}\in [0,\rho]$, the optimal solution $\bm{x}_{j}^{*}(\rho_{j};\bm{z})$ defined in Eq. \eqref{eq:budperchannelsol} is budget binding, i.e. $\totc_{j}(\rho_{j};\bm{z}) =\bm{d}_{j}^{\top}\bm{x}_{j}^{*}(\rho_{j};\bm{z}) = \rho_{j}$. 
% \end{proposition}

\subsection{The SGD-UCB algorithm to optimize per-channel budgets}
\label{subsec:algo}
Here, we describe our algorithm to solve for optimal per-channel budgets w.r.t.  $\textsc{CH-OPT}(\mathcal{I}_{\budg})$. Similar to most algorithms for constrained optimization, we take a dual stochastic gradient descent (SGD) approach; see a comprehensive survey on dual descent methods in \cite{bertsekas2014constrained}. First, we consider the Lagrangian functions w.r.t. $\textsc{CH-OPT}(\mathcal{I}_{\budg})$ where we let  $\cont = (\lambda, \mu) \in \R_{+}^{2}$ be the dual variables corresponding to the ROI and budget constraints, respectively:
\begin{align}
    \label{eq:Lagrangian}
    \mathcal{L}_{j}(\rho_{j}, \cont; \bm{z}_{j}) =  (1+\lambda)\totv_{j}(\rho_{j};\bm{z}_{j}) - (\lambda \gamma  + \mu) \rho_{j} ~\text{ and }~\mathcal{L}_{j}(\rho_{j}, \cont) = \E\left[  \mathcal{L}_{j}(\rho_{j}, \cont; \bm{z}_{j})\right]\,.
\end{align}
With this lagrangification, SGD decouples the aggregate constraints over channels, and further operates on both primal and dual domains to update per-channel budgets for each channel independently, as well dual variables, respectively:
In each period $t\in [T]$ given dual  variables $\cont_{t} = (\lambda_{t},\gamma_{t})$, SGD decides on a primal decision, i.e. per-channel budget $(\rho_{j,t})_{j\in[M]}$ by solving the following optimization problem 
\begin{align}
\label{eq:SGDprimal}
    \rho_{j,t} ~=~ \arg\max_{\rho_{j}\in [0,\rho]}\mathcal{L}_{j}(\rho_{j}, \cont_{t};\bm{z}_{t})\,.
\end{align}
 Then, having observed the realized values $\left(\totv_{j}(\rho_{j,t};\bm{z}_{t})\right)_{j\in[M]}$ (note that spend is $(\rho_{j,t})_{j\in [M]}$ in light of Proposition \ref{prop:budgetbind}),  we calculate the current period violation in budget and ROI constraints, namely  $g_{1,t}:= \sum_{j \in M} \left(\totv_{j}(\rho_{j,t};\bm{z}_{t}) -  \gamma \rho_{j,t}\right)$ and $g_{2,t} = \rho - \sum_{j\in [M]} \rho_{j,t}$. Next, we update dual variables via $ 
\lambda_{t+1} = \left(\lambda_{t} - \eta g_{1,t}\right)_{+} \text{ and } \mu_{t+1}  = \left(\mu_{t} - \eta g_{2,t}\right)_{+}$, where $\eta$ is some pre-specified step size.\footnote{Here, the dual updates follow the vanilla gradient descent approach, and one can also employ more general mirror descent updates; see e.g. \cite{balseiro2022best}.}

{\color{blue} However, the above SGD approach faces a fatal drawback, namely we cannot realistically find the primal decisions by solving Eq. \eqref{eq:SGDprimal} since the function $\mathcal{L}_{j}(\cdot, \cont_{t};\bm{z}_{t})$ is unknown due to the  bandit feedback  structure. Therefore, we provide a modification to SGD to handle this issue. Before we present our approach, we briefly note that although bandit feedback prevents the naive application of SGD for our problem of interest, this may not be the case in other online advertising scenarios that involve relevant learning tasks, underlining the challenges of our problem; see following Remark \ref{rmk:banditfeedback} for details.
\begin{remark}
\label{rmk:banditfeedback}
Our problem of interest under bandit feedback is more difficult than similar problems in related works that study online bidding strategies under budget and ROI constraints; see e.g. \cite{balseiro2017budget,balseiro2022best,feng2022online}. To illustrate, consider for instance  \cite{balseiro2017budget} in which a budget constrained advertiser's primal decision at period $t$ is to submit a bid value  $b_{t}$ after observing her value $v_{t}$. The advertiser competes with some unknown  highest competing bid $d_{t}$ in the market, and after submitting bid $b_{t}$, does not observe $d_{t}$ if she does not win the competition, which involves a semi-bandit feedback structure. Nevertheless, the corresponding Lagrangian under SGD takes the special form $\mathcal{L}_{j}(b, \mu_{t};\bm{z}_{t}) =\left(v_{t} - (1+\mu_{t})d_{t}\right)\I\{b_{t} \geq d_{t}\}$ where $\mu_{t}$ is the dual variable w.r.t. the budget constraint.  This simply allows an advertiser to optimize for her primal decision by bidding $\arg\max_{b\geq 0} \mathcal{L}_{j}(b, \cont_{t};\bm{z}_{t}) = \frac{v_{t}}{1+\mu_{t}}$. So even though \cite{balseiro2017budget,balseiro2022best,feng2022online} study dual SGD under bandit feedback, the special structures of their problem instances permits SGD to effectively optimize for primal decisions in each period, as opposed to Eq. \eqref{eq:SGDprimal} in our setting which can not be  solved.
\end{remark}}
To resolve challenges that arise with bandit feedback in our model, we take a natural approach to augment SGD with the \textit{upper-confidence bound (UCB)} algorithm, which is arguably the first resort to solve learning problems under bandit feedback such as the famous multi-arm bandit problem;\yuan{Are we the first to combine SGD and UCB? If yes, could you highlight this? if not, could you add some citations for comparison?} \negin{agree with this comment. also, when  you say this is ``the first resort" implies that there are prior works that use this technique. If this is not the case, please paraphrase that sentence. } see an introduction to multi-arm bandits in \cite{slivkins2019introduction}. In particular, we first discretize our per-channel buudget decision set $[0,\rho]$ into granular ``arms'' that are separated by some distance $\discerr > 0$, so that the discretized per-channel budget decisions become
\begin{align}
\label{eq:budgetdisc}
    \budgset(\discerr) = \{a_{k}\}_{k \in [K]} \text{ where } a_{k} = (k-1)\discerr \text{ and }K := \lceil{\rho}/{\discerr}\rceil + 1\,.
\end{align}
In the following we will use the terms ``per-channel budget'' and ``arm'' interchangeably. {\color{red} I suggest this we discuss these (rewards and contexts) when we present the proof in the next section. Here, we can mainly focus on describing the novelty of the design.} Then, we perceive dual variables $\{\cont_{t}\}_{t\in[T]}$ to be \textit{adversarial contexts}, and the Lagrangian $\mathcal{L}_{j}(a_{k},\cont_{t};\bm{z}_{t})$ to be the reward function that maps any arm-context pair $(a_{k},\cont_{t})$ to a (stochastic) payoff. Then following UCB, in each period $t$ we maintain some estimate $\left(\Bar{\totv}_{j}(a_{k})\right)_{j\in[M]}$ of the conversions $\left(\totv_{j}(a_{k})\right)_{j\in [M]}$ as well as an upper confidence bound $\ucb_{j,t}(a_{k})$ for each arm $a_{k}$ using historical payoffs from periods in which arm $a_{k}$ is pulled. Finally, we update primal decisions for each channel $j\in[M]$ using the ``best arm'' $\rho_{j,t} = \arg\max_{a_{k}\in \budgset(\discerr)}~(1+\lambda_{t})\left(\Bar{\totv}_{j,t}(a_{k}) +  \ucb_{j,t}(a_{k})\right) - \left(\lambda_{t} \gamma + \mu_{t} \right)a_{k}$. We summarize our algorithm, called SGD-UCB, in the following Algorithm \ref{alg:omducb}.

\begin{algorithm}[H]
    \centering
    \caption{SGD-UCB$(\gamma,\rho)$}\label{alg:omducb}
    \footnotesize
    \begin{algorithmic}[1]
    \Require Global target ROI $\gamma$ and global budget parameter $\rho$. Budget discretization $\discerr > 0$ and set of arms $\budgset(\discerr)$ defined in Eq.\eqref{eq:budgetdisc} with $|\budgset(\discerr)| =K$. Step size $\eta > 0$ and strictly convex regularizer $h:\R\to\R$. Initialize $ N_{j,1}(a_{k}) = \Bar{\totv}_{j,1}(a_{k})  = 0$ for all $j \in [M]$ and $k\in [K]$.
    Initialize dual variables $\lambda_{1} = \mu_{1}= 0$.
    % \For{$t = 1 \dots K$ }
    % \State Set identical budgets in each channel with the $t$'th arm, i.e. $\bm{\rho}_{t} = (a_{t},a_{t}\dots a_{t})\in \budgset(\discerr)^{M}$.
    % \EndFor
    \\
    \textbf{Output:} Per channel budget.   
	\For{$t = 1 \dots T$ }
	 \State \textbf{Update (primal) per-channel budget.} For each channel $j\in [M]$ set (primal) per-channel budget:
  \begin{itemize}
      \item If $t \leq K$, set $\rho_{j,t} = a_{t}$.
      \item If $t > K$, set
      \begin{align}
        \begin{aligned}
          & \rho_{j,t} = \arg\max_{a_{k}\in \budgset(\discerr)}~(1+\lambda_{t})\left(\Bar{\totv}_{j,t}(a_{k}) +  \ucb_{j,t}(a_{k})\right) - \left(\lambda_{t} \gamma + \mu_{t} \right)a_{k}, ~\text{ where } \ucb_{j,t}(a_{k}) = \sqrt{\frac{2\log(T)}{N_{j,t}(a_{k})}} 
           \end{aligned}
          \end{align}
  \end{itemize}
    \State  Observe realized values $\left\{\totv_{j}(\rho_{j,t};\bm{z}_{t}) \right\}_{j \in [M]}$, and update for each arm $k \in [K]$:{\color{red}NG: $\rho_{j,t} = a_{k}$ instead of $\rho_{j,\tau} = a_{k}$?}
    \begin{align}
    \begin{aligned}
        & N_{j,t+1}(a_{k}) =  N_{j,t}(a_{k}) + \I\{\rho_{j,\tau} = a_{k}\}\\
        & \Bar{\totv}_{j,t+1}(a_{k}) = \frac{1}{N_{j,t+1}(a_{k})} \left(N_{j,t}(a_{k}) \Bar{\totv}_{j,t}(a_{k}) + \totv_{j}(\rho_{j,t};\bm{z}_{t}) \I\{\rho_{j,\tau} = a_{k}\}\right) \quad, \text{ for } j = 1 \dots M
        \end{aligned}
    \end{align}
    \State \textbf{Update dual variables.} Update dual variables with $g_{1,t}:= \sum_{j \in M} \left(\totv_{j}(\rho_{j,t};\bm{z}_{t}) -  \gamma \rho_{j,t}\right)$ and $g_{2,t} = \rho - \sum_{j\in [M]} \rho_{j,t}$:
    % \begin{align}
    %     \label{eq:dualupdate}
        % \begin{aligned}
        % & \dot{h}(\widetilde{\lambda}_{t+1})= \dot{h}(\lambda_{t}) - \epsilon g_{1,t} \text{ and } \dot{h}(\widetilde{\mu}_{t+1})= \dot{h}(\mu_{t}) - \epsilon g_{2,t} \\
        % &  \lambda_{t+1}  = \arg\min_{\lambda\geq 0} \breg_{h}(\lambda,\widetilde{\lambda}_{t+1}) \text{ and }  \mu_{t+1}  = \arg\min_{\mu\geq 0} \breg_{h}(\mu,\widetilde{\mu}_{t+1})
        % \end{aligned}
        % \end{align}
        % where $\breg_{h}(x,y) = h(x) - h(y) - \dot{h}(y)(y-x)$ is the Bregman divergence w.r.t. $h:\R \to \R$.
        \begin{align}
        \label{eq:dualupdate}
        \begin{aligned}
     \lambda_{t+1} = \left(\lambda_{t} - \eta g_{1,t}\right)_{+} \text{ and } \mu_{t+1}  = \left(\mu_{t} - \eta g_{2,t}\right)_{+}
        \end{aligned}
        \end{align}
	\EndFor
 \State Output $\overline{\bm{\rho}}_{T} = \left(\frac{1}{T}\sum_{t\in[T]} \rho_{j,t}\right)_{j\in [M]}$.
    \end{algorithmic}
\end{algorithm}


\subsection{Analyzing the SGD-UCB algorithm}
\label{subsec:algo}
In this subsection, we analyze the performance of SGD-UCB in Algorithm \ref{alg:omducb}. At first sight, our algorithm faces a setup that involves discretizing a continuum of arms (i.e. the continuous per-channel budget decision set $[0,\rho]$), as well as contextual bandit rewards {\color{red} as I said before, let's define the contextual bandit setting here and please elaborate more on this using equation (10) so that readers can better understand this. }, both of which have been notoriously difficult to handle without special structures in the reward function (in our case the Lagrangian $\mathcal{L}_{j}(\rho_{j},\cont;\bm{z})$ defined in Eq. \ref{eq:Lagrangian}; see e.g. discussions in \cite{agrawal1995continuum} and \cite{agarwal2014taming} for continuum-arm bandits and contextual bandits, respectively. Fortunately, the specific form of conversion functions $\totv(\rho_{j};\bm{z})$ {\color{red} NG: not sure if we have done it already. But, please make sure that in the model section we define the term ``conversion functions."} defined in Eq. \eqref{eq:budperchannelsol} imposes a salient structure on the Lagrangian, or equivalently the reward function for pulling an arm. Specifically, the following lemma shows that the Lagrangian is continuous, piecewise linear, concave, and unimodal\footnote{We say a real-valued function $f:\R\to \R$ is unimodal if there exists some $y^{*}$ such that $f(y)$ strictly increases when $y \leq y^{*}$ and  strictly decreases when $y \geq y^{*}$. {\color{red} NG: why strictly?}}; we present the proof in Appendix \ref{pf:lem:Vstruct}
% \begin{definition}[Unimodal functions]
% We say a real-valued function $f:\R\to \R$ is unimodal if there exists some $y^{*}$ such that $f(y)$ strictly increases when $y \leq y^{*}$ and  strictly decreases when $y \geq y^{*}$.
% \end{definition}
\begin{lemma}[Structural properties of conversion  and Lagrangian functions]
\label{lem:Vstruct}
\begin{itemize}
\item
For any channel $j\in [M]$ and per-channel budget $\rho_{j}$ the conversion function $\totv_{j}(\rho_{j})$ is continuous, piece-wise linear, strictly increasing, and concave. In particular,  $\totv_{j}(\rho_{j})$ takes the form
\begin{align}
\label{eq:Vstruct}
        \totv_{j}(\rho_{j}) = \sum_{n\in [S_{j}]} \left(s_{j,n} \rho_{j} + b_{j,n}\right)\I\{r_{j,n-1}\leq \rho_{j} \leq r_{j,n}\}\,,
\end{align}
where the parameters $S_{j} \in \N$ and $\{(s_{j,n},b_{j,n},r_{j,n})\}_{n\in [S_{j}]}$ only depend on the support $F_{j}$ and distribution $\bm{p}_{j}$ from which value-to-cost pairs are sampled.  These parameters satisfy
$s_{j,1} > s_{j,2} > \dots > s_{j,S_{j}} > 0$ and $0=r_{j,0} < r_{j,1} < r_{j,2} < \dots < r_{j,S_{j}} =\rho$, as well as $b_{j,n} > 0$ s.t. $s_{j,n} r_{j,n} + b_{j,n} = s_{j,n+1} r_{j,n} + b_{j,n+1}$ for all $n \in [S_{j}-1]$, implying $\totv_{j}(\rho_{j}) $ is continous  in $\rho_j$.
\item For any dual variables $\cont = (\lambda,\mu) \in \R_{+}^{2}$, the Lagrangian function $ \mathcal{L}_{j}(\rho_{j},\cont)$ defined in Eq. \eqref{eq:Lagrangian} is continuous, piece-wise linear, concave, and unimodal in $\rho_{j}$. In particular,
\begin{align}
\label{eq:lagrrep}
        \mathcal{L}_{j}(\rho_{j}, \cont) =  \sum_{n\in [S_{j}]} \left( \slope_{j,n}(\cont) \rho_{j} + (1+\lambda)b_{j,n}\right)\I\{r_{j,n-1}\leq \rho_{j} \leq r_{j,n}\}\,,
\end{align}
where the slope $\slope_{j,n}(\cont) = (1+\lambda) s_{j,n} -(\mu + \gamma \lambda)$. 
Then, this also implies $\arg\max_{\rho_{j}\geq 0} \mathcal{L}_{j}(\rho_{j}, \cont) = \max\{r_{j,n}:n=0,1\dots, S_{j}~,\slope_{j,n}(\cont) \geq 0\}$.
\end{itemize}
\end{lemma}
In fact,  for any realized value-cost pairs $\bm{z}$, the ``realization 
versions'' of the conversion functions and Lagrangians {\color{red}NG: Lagrangians or Lagrangians? We have both. Let's be consistent. Also, let's call it Lagrangian function as it is a function that maps the dual variables to some (virtual) reward. Using this terminology, you can better define the contextual bandit setting.}, namely $\totv_{j}(\rho_{j};\bm{z}) $ and $\mathcal{L}_{j}(\rho_{j}, \cont;\bm{z})$,  also satisfy the same properties as those of $\totv_{j}(\rho_{j})$ and $\mathcal{L}_{j}(\rho_{j}, \cont)$, respectively. See  Lemma \ref{lem:Vstruct}. We provide a visual illustration for these structural properties in Figure \ref{fig:lagr}. 

In light of concavity for the conversion functions $\left(\totv_{j}(\rho_{j})\right)_{j \in [M]}$, the 
advertiser's optimization problem $\textsc{CH-OPT}(\mathcal{I}_{\budg})$ in Eq. \eqref{eq:chopt} effectively becomes a convex problem (as we maximize a concave function in $\textsc{CH-OPT}(\mathcal{I}_{\budg})$, and it is apparent {\color{red} NG: it is not very apprent to me. Do we show this formally somewhere?} that the feasible region for $\textsc{CH-OPT}(\mathcal{I}_{\budg})$ is convex).  Here, we make an important remark that distinguishes our work with  related literature on convex optimization.

{\color{red}NG: I suggest we present this remark at the end of this section as it is a distraction and is hurting the flow. the point of the remark would be  better received after presenting our regret bound. Another option is to put a short version of this in the intro or related work section and then  quickly revisit that discussion here. }
\begin{remark}
\label{rmk:onepoint}
Given the advertiser's optimization problem  $\textsc{CH-OPT}(\mathcal{I}_{\budg})$ is convex, it may be tempting for one to directly employ off-the-shelf convex optimization algorithms. However, our problem instance involves stochastic bandit feedback, and more importantly, \textit{uncertain constraints}, meaning that during each period a primal decision is made, we cannot analytically determine whether the primal decision satisfies the constraints of the problem. For example, in $\textsc{CH-OPT}(\mathcal{I}_{\budg})$, for some primal decision $(\rho_{j})_{j\in[M]}$, we cannot determine whether the ROI and budget constraints  $\sum_{j \in M} \E\left[\totv_{j}(\gamma_{j},\rho_{j};\bm{z}_{j})\right] \geq \gamma \sum_{j \in M} \E\left[\totc_{j}(\gamma_{j},\rho_{j};\bm{z}_{j})\right]$ and $\sum_{j\in [M]}\E\left[\totc_{j}(\gamma_{j},\rho_{j};\bm{z}_{j})\right]\leq \rho$ hold because the distributions $(\bm{p}_{j})_{j\in[M]}$ from which $\bm{z}$ is sampled are unknown. In other words, we cannot evaluate the expectations. To the best of our knowledge, there are only two recent works that handle a similar stochastic bandit feedback, and uncertain constraint setting, namely \cite{usmanova2019safe} and \cite{nguyen2022stochastic}. Nevertheless, our setting is more challenging because these works consider a ``two-point estimation'' regime where one can make function evaluations to the objective and constraints twice each period, whereas our setting lies in the ``one-point estimation'' such that we can only make function calls once per period. Finally, we also point out that optimal oracle optimization complexities for unknown constrained (non-smooth) convex optimization with one-point bandit feedback, remains an open problem. We refer readers to Table 4.1 in \cite{larson2019derivative} for a survey on best known bounds under different one-point bandit feedback settings.
\end{remark}


\begin{figure}[h]
\includegraphics[width=\textwidth]{lagr.png}
\caption{Illustration of Lagrangian functions defined in Eq. \eqref{eq:Lagrangian} with $M_{j} = 2$ auctions in channel $j$, and support $F_{j}$ that contains 3 elements,  $\bm{z}_{(1)} = (\bm{v}_{(1)},\bm{d}_{(1)}) = ((8,2), (2,3))$, $\bm{z}_{(2)} = ((3,4), (1,4))$, $\bm{z}_{(3)} = ((8,1), (4,2))$, and context $\cont = (\lambda,\mu) = (4,2)$. In the context of Lemma \ref{lem:Vstruct}, $S_{j} = 5$, where the ``turning points'' $r_{j,0} \dots r_{j,S_{j}}$ are indicated on the x-axis, and the optimal budget w.r.t. $\cont$ is $\arg\max_{\rho_{j}\in [0,\rho]}\mathcal{L}_{j}(\rho_{j};\cont) = r_{j,2}$. The adjacent slopes in Eq. \eqref{eq:adj} are $\slope_{j}^{-}(\cont) = \slope_{j,2}(\cont)$, and  $\slope_{j}^{+}(\cont) = \slope_{j,3}(\cont)$, respectively.}
\label{fig:lagr}
\end{figure}

% \begin{lemma}[Unimodalilty of expected conversion]
% For any channel $j\in [M]$, let $(\bm{v},\bm{d}) \in \supp(F_{j})$ be any element in the support of the discrete distribution $F_{j}$, and without loss of generality assume we have a value-to-cost ordering $\frac{v_{1}}{d_{1}} >\frac{v_{2}}{d_{2}} >\dots > \frac{v_{M_{j}}}{d_{M_{j}}}$. Then $ \totv_{j}(\rho_{j};\bm{v},\bm{d}) $ is piecewise linear and strictly increasing in $\rho_{j}$; in particular
% \begin{align}
%         \totv_{j}(\rho_{j};\bm{v},\bm{d}) = \sum_{n\in [M_{j}]} \left(\frac{v_{n}}{d_{n}} \rho_{j} + c_{n}\right)\I\{d_{0} + d_{1}\dots + d_{n-1}\leq \rho_{j} \leq d_{0}+\dots + d_{n-1} + d_{n}\}\end{align}
%  where we denote $d_{0} = 0$ and $\{c_{n}\}_{n\in[M_{j}]}$ are some positive constants. Further, for any $\lambda, \mu \geq 0$, the Lagrangian function $\mathcal{L}(\rho_{j},\lambda,\mu)$ is piecewise linear and unimodal.
%  % ; in particular, 
%  %    \begin{align}
%  %    \label{eq:dualfuncturning}
%  %     \mathcal{L}(\rho_{j},\lambda,\mu) = \sum_{n\in [M_{j}]} 
%  %       \arg\max_{\rho_{j}\geq 0}\quad (1+\lambda)\totv_{j}(\rho_{j}) - \left(\lambda \gamma + \mu \right)\rho_{j}  = d_{1,j}  + \dots d_{\kappa_{j},j} \quad \text{where } \kappa_{j} = \min\left\{k \in [K]: \frac{v_{k,j}}{d_{k,j}} < \frac{\lambda \gamma + \mu}{1+\lambda}\right\}
%  %    \end{align}
% \end{lemma}

% \begin{corollary}[Local Lipschitz continuity]
% For any per-channel budget $\rho_{j}$, define $n^{(\ell)} \in [M_{j}]$ such that $\rho_{j} \in [s_{n^{(\ell)}-1}, s_{n^{(\ell)}}]$, and define $\mathcal{S}_{j}^{\ell}(\rho_{j}) = [s_{n^{(\ell)}-1}, s_{n^{(\ell)}}]$ to be the line segment of . Further, define $\mathcal{S}_{j}(\rho_{j}) = \cap_{\ell \in [L_{j}]} \mathcal{S}_{j}^{\ell}(\rho_{j})$. For any $\lambda, \mu \geq 0$ let $\rho_{j}^{*} = \arg\max_{\rho_{j}\geq 0} \mathcal{L}(\rho_{j},\lambda, \gamma )$. Then for any $\rho \in \mathcal{S}_{j}(\rho_{j}^{*})$, we have
%  \begin{align}
%    \min \left\{\left|C_{j}^{-} - \frac{\mu + \gamma\lambda}{1+\lambda}\right|,\left|C_{j}^{+} - \frac{\mu + \gamma\lambda}{1+\lambda}\right|\right\}\leq  \frac{\left| \mathcal{L}(\rho_{j}^{*},\lambda, \gamma ) -  \mathcal{L}(\rho_{j},\lambda, \gamma )\right| }{(1+\lambda)\cdot \left|\rho_{j}^{*} - \rho_{j}\right|}\leq  \max \left\{\left|C_{j}^{-} - \frac{\mu + \gamma\lambda}{1+\lambda}\right|,\left|C_{j}^{+} - \frac{\mu + \gamma\lambda}{1+\lambda}\right|\right\}
%     \end{align}
%     where $ C_{j}^{-}= $ and $C_{j}^{+}=$. 
% \end{corollary}


% \begin{corollary}[Local Lipschitz continuity]
%     Let $\kappa_{j}$ be defined as in Eq. \eqref{eq:dualfuncturning}, and $\ell_{j} = \min\{d_{\kappa_{j}-1,j}, d_{\kappa_{j}+1,j}\}$.
%     Then, for any $\rho_{j} \in [\sum_{k=1}^{ \kappa_{j}}d_{k,j} - \ell_{j},\sum_{k=1}^{ \kappa_{j}}d_{k,j} + \ell_{j}]$, we have
%     \begin{align}
%    \min\left\{c_{j,1},c_{j,2} \right\} \leq  \frac{\left| \mathcal{L}(\rho_{j},\lambda, \gamma ) -  \mathcal{L}(\rho_{j}',\lambda, \gamma )\right| }{\left|\rho_{j} - \rho_{j}'\right|}\leq  \max\left\{c_{j,1},c_{j,2} \right\} 
%     \end{align}
%     where $c_{j,1} = \left|\frac{v_{\kappa_{j}-1,j}}{d_{\kappa_{j}-1,j}} -\frac{\lambda \gamma + \mu}{1+\lambda}\right|$ and $c_{j,2} = \left|\frac{v_{\kappa_{j},j}}{d_{\kappa_{j},j}} -\frac{\lambda \gamma + \mu}{1+\lambda}\right|$. 
% \end{corollary}

% \begin{theorem}
% For a given exploration length $E > 0$ and discretization width $\discerr$, we have
%     \begin{align}
%      T \cdot \textsc{GL-OPT} - \sum_{t\in [T]} \sum_{j\in[M]}\totv(\rho_{j,t}) \leq E  \frac{\rho}{\discerr} + M\Bar{\lambda} T\left(\discerr + \mathcal{O}\left(\sqrt{\frac{1}{E}}\right)\right) + \mathcal{O}(\sqrt{T})\,.
% \end{align}
% Setting $\discerr = E^{-\frac{1}{2}} = T^{-\frac{1}{4}}$ yields a regret in the order of $\mathcal{O}(T^{\frac{3}{4}})$.
% \end{theorem}

% \textit{Proof.}
% \begin{proof}
% For any $\lambda, \mu \geq 0$, we have 
% \begin{align}
%   & \textsc{GL-OPT} \\
%   ~=~ & \textsc{CH-BUD-OPT}\\
%   ~\leq~ & \mu\rho + \max_{\bm{\rho} \in \R_{+}^{M}} \sum_{j\in [M]}(1+\lambda)\totv_{j}(\rho_{j}) - \left(\lambda \gamma + \mu \right)\rho_{j} \\
%   ~\overset{(i)}{\leq}~ & \frac{1}{T}\sum_{t\in[T]} \mu_{t} \rho +\frac{1}{T}\sum_{t\in[T]}\max_{\bm{\rho} \in \R_{+}^{M}} \sum_{j\in [M]}(1+\lambda_{t})\totv_{j}(\rho_{j}) - \left(\lambda_{t}\gamma + \mu_{t} \right)\rho_{j} \\
%   ~:=~ & \frac{1}{T}\sum_{t\in[T]} \mu_{t} \rho +\frac{1}{T}\sum_{t\in[T]} \sum_{j\in [M]}(1+\lambda_{t})\totv_{j}(\rho_{j,t}^{*}) - \left(\lambda_{t}\gamma + \mu_{t} \right)\rho_{j,t}^{*} \\
%  ~\overset{(ii)}{\leq}~& \frac{1}{T}\sum_{t\in[T]} \mu_{t} \rho +\frac{1}{T}\sum_{t\in[T]} \sum_{j\in [M]}(1+\lambda_{t})\Bar{\totv}_{j}(\rho_{j,t}^{*}) + M(1+\Bar{\lambda})  \mathcal{O}(\frac{1}{\sqrt{E}}) - \left(\lambda_{t}\gamma + \mu_{t}
%  \right)\rho_{j,t}^{*} \\
%  ~\leq~& \frac{1}{T}\sum_{t\in[T]} \mu_{t} \rho + \frac{1}{T}\sum_{t\in[T]} \max_{\bm{\rho}\in \R_{+}^{M}}\sum_{j\in [M]}(1+\lambda_{t})\Bar{\totv}_{j}(\rho_{j}) - \left(\lambda_{t}\gamma +\mu_{t}\right)\rho_{j}+ M(1+\Bar{\lambda}) \mathcal{O}(\frac{1}{\sqrt{E}})\\
%  ~\leq~& \frac{1}{T}\sum_{t\in[T]} \mu_{t} \rho + \frac{1}{T}\sum_{t\in[T]} \sum_{j\in [M]}\underbrace{\max_{\rho_{j}\in \R_{+}}(1+\lambda_{t})\Bar{\totv}_{j}(\rho_{j}) - \left(\lambda_{t}\gamma +\mu_{t}\right)\rho_{j}}_{X} + M(1+\Bar{\lambda}) \mathcal{O}(\frac{1}{\sqrt{E}})
% \end{align}
% where in (i) we take $\mu = \frac{\sum_{t\in[T]}\mu_{t}}{T}$ and $\lambda = \frac{\sum_{t\in[T]}\lambda_{t}}{T}$, and applied convexity of the dual function; in (ii) we used the fact that $\left|\Bar{\totv}(\rho_{j,t})  - \totv(\rho_{j,t}) \right|\leq \mathcal{O}(\sqrt{1/E})$.
% On the other hand, we have
% \begin{align}
% \begin{aligned}
% & \Bar{\totv}(\rho_{j,t}) +  \lambda_{t}\left(\Bar{\totv}(\rho_{j,t}) - \gamma \rho_{j,t}\right) + \mu_{t} \rho_{j,t} \\~=~ &  \max_{\rho_{j} \in \budgset} ~(1+\lambda_{t})\Bar{\totv}_{j}(\rho_{j}) - \left(\lambda_{t}\gamma + \mu_{t} \right)\rho_{j} \\
%  ~\geq~ &  \max_{\rho_{j} \in \R_{+}} ~(1+\lambda_{t})\Bar{\totv}_{j}(\rho_{j}) - (1+\Bar{\lambda})\discerr - \left(\lambda_{t}\gamma + \mu_{t} \right)\rho_{j} 
%  \end{aligned}
% \end{align}
% Therefore,
% \begin{align}
% \begin{aligned}
% \totv(\rho_{j,t}) ~\geq~ & \Bar{\totv}(\rho_{j,t}) - \mathcal{O}(\frac{1}{\sqrt{E}}) \\
% ~\geq~ &  \underbrace{\max_{\rho_{j} \in \R_{+}} ~(1+\lambda_{t})\Bar{\totv}_{j}(\rho_{j})- \left(\lambda_{t}\gamma + \mu_{t} \right)\rho_{j} }_{X} - (1+\Bar{\lambda})\discerr  - \left(\lambda_{t}\left(\Bar{\totv}(\rho_{j,t}) - \gamma \rho_{j,t}\right) - \mu_{t} \rho_{j,t}\right)
% \end{aligned}
% \end{align}

% Finally, combining the above we havce
% \begin{align}
% & T \cdot \textsc{GL-OPT} - \sum_{t\in [T]} \sum_{j\in[M]}\totv(\rho_{j,t})\\
%      ~\leq~ & E  \frac{\rho}{\discerr} + M\Bar{\lambda} T\left(\discerr + \mathcal{O}(\sqrt{\frac{1}{E}})\right) + \underbrace{\sum_{t \in [T]}\lambda_{t}\left(\Bar{\totv}(\rho_{j,t}) - \gamma \rho_{j,t}\right)  + \sum_{t \in [T]}\mu_{t}\left(\rho - \sum_{j\in[M]}\rho_{j,t}\right)}_{
%      =\mathcal{O}(\sqrt{T})}
%      \,.
% \end{align}
% Setting $\discerr = E^{-\frac{1}{2}} = T^{-\frac{1}{4}}$, we have $  T \cdot \textsc{GL-OPT} - \sum_{t\in [T]} \sum_{j\in[M]}\totv(\rho_{j,t}) \leq \mathcal{O}(T^{\frac{3}{4}})$. 
% \end{proof}



With the salient structural properties of the Lagrangian functions illustrated in Lemma \ref{lem:Vstruct}, we now present results to analyze the performance of UCB-SGD Algorithm \ref{alg:omducb}. Our strategy is to show $T\cdot  \textsc{GL-OPT} - \E\left[\sum_{t\in [T]}\sum_{j\in[M]}\totv_{j}(\rho_{j,t})\right] = \mathcal{O}(T^{\zeta})$ for some $\zeta \in (0,1)$, because using concavity of the $\totv_{j}(\cdot)$ functions directly yields an optimization accuracy $\textsc{GL-OPT} - \E\left[\sum_{j\in[M]}\totv_{j}\left(\frac{\sum_{t\in [T]\rho_{j,t}}}{T}\right)\right]\leq \mathcal{O}(T^{-(1-\zeta})$. Now, the following Proposition \ref{prop:ubbenchlag} allows us to decompose $T\cdot  \textsc{GL-OPT} - \E\left[\sum_{t\in [T]}\sum_{j\in[M]}\totv_{j}(\rho_{j,t})\right]$ into two main parts, namely the error induced by the UCB in our algorithm, and the error due to SGD (or what is typically viewed as the deviations from  complementary slackness):

\begin{proposition}
\label{prop:ubbenchlag}
For any channel $ j\in [M]$ define $\rho_{j}^{*}(t) = \arg\max_{\rho_{j\in[M]}}\mathcal{L}_{j}(\rho_{j};\cont)$ to be the optimal per-channel budget w.r.t. dual variables $\cont_{t}=(\lambda_{t},\mu_{t})_{t\in [T]}$ during period $t\in[T]$. Then we have 
 \begin{align}
 \begin{aligned}
 \label{eq:decompregret}
     & T \cdot\textsc{GL-OPT} - \E\left[\sum_{t\in [T]}\sum_{j\in[M]}\totv_{j}(\rho_{j,t})\right] \\ ~\leq~&  M\Bar{V}K +
     \sum_{j\in [M]}\underbrace{\sum_{t> K} 
     \E\left[\mathcal{L}_{j}(\rho_{j}^{*}(t), \lambda_{t}, \mu_{t})  - \mathcal{L}_{j}(\rho_{j,t}, \lambda_{t}, \mu_{t})\right]}_{\text{UCB error}}+ \underbrace{\sum_{t >K}\E\left[\lambda_{t}g_{1,t} + \mu_{t}g_{2,t}\right]}_{\text{SGD complementary slackness deviations}}\,,
      \end{aligned}
 \end{align}
\end{proposition}
 where we recall the definitions of $g_{1,t}$ and $g_{2,t}$ in step 4 of Algorithm \ref{alg:omducb}, and the fact that the conversion $ \totv_{j}(\rho_{j};\bm{z}_{j})$ is bounded above by absolute constant $\Bar{\totv} \in (0,\infty)$ almost surely for any channel $j\in[M]$, $(\gamma_{j},\rho_{j})$ and realization $\bm{z}_{j}$.
 
 Before we move on to bound the UCB error, we first need to show that the UCB rewards are bounded under all arms and contexts, or in other words, the Lagrangian function is bounded for for all arms and dual variables. Boundedness on rewards is typically assumed to hold in general multi-arm bandit setups, but in our case, the rewards, i.e. the Lagrangian depends scales linearly with dual variables, which may seemingly violate boundedness conditions that can make UCB fail.  {\color{red} NG: recall the definition of the Lagrangian function by referring to its equation.} Fortunately, we show that 
  the Lagrangian functions, as well as dual variables, are indeed bounded by some absolute constants in the following Lemma \ref{lem:dualvarub} under a mild feasibility Assumption \ref{ass:feas} stated below:
\begin{assumption}[Strictly feasible global ROI constraints]
\label{ass:feas}
For any realization of value-cost pairs  $\bm{z} =(\bm{v}_{j},\bm{d}_{j})_{j\in[M]} \in F_{1}\times \dots F_{M}$, the realized version of the ROI constraint in \textsc{GL-OPT} defined in Eq. \ref{eq:glopt} is strictly feasible, i.e. the set $\left\{\bm{x}= (\bm{x}_{j})_{j\in [M]}: \bm{x}_{j} \in [0,1]^{m_{j}} \text{ for }\forall j\in [M],~\sum_{j\in[M]}\bm{v}_{j}^{\top} \bm{x}_{j} > \gamma\sum_{j\in[M]}\bm{d}_{j}^{\top}\bm{x}_{j}\right\}$ is nonempty.\footnote{Equivalently, for any realization of value-cost pairs  $\bm{z} = (\bm{v}_{j},\bm{d}_{j})_{j\in[M]}$ there always exists a channel $j\in [M]$ and an auction  $n\in [m_{j}]$ in this channel  whose value-to-cost ratio is at least $\gamma$, i.e. $v_{j,n} >  \gamma d_{j,n}$.}
\end{assumption}
\begin{lemma}[Bounding dual variables and Lagrangian functions]
\label{lem:dualvarub}
Let $(\lambda_{t},\mu_{t})_{t\in [T]}$ be the variables generated from Algorithm \ref{alg:omducb}. Under Assumption \ref{ass:feas}, and assuming the step size $\eta > 0$ satisfies $\eta < \frac{1}{M \cdot \max\left\{\bar{\totv}, \rho, \bar{\totv}^{2}\right\}}$, there exists some absolute constant $\dualub_{F} > 0$ that depends only on the support of value-cost pairs  $F = F_{1} \times \dots \times F_{M}$ as well as aggregate target ROI and budget $(\gamma,\rho)$ such that $\lambda_{t},\mu_{t} \leq \dualub_{F}$ for all $t \in [T]$. Moreover, for any for any $t\in [T]$, $j\in [M]$ and $\rho_{j} \in [0,\rho]$ we have 
\begin{align}
   -\left(1+\gamma \right)\rho\dualub_{F}
   ~\leq~ \mathcal{L}_{j}(\rho_{j},\lambda_{t},\mu_{t})~\leq~(1+\dualub_{F})\Bar{\totv}\,.
\end{align}
\end{lemma}
See proof in Appendix \ref{pf:lem:dualvarub}.

We now move on to bound the UCB error, which is the main technical challenge in this section. As illustrated before,
 the salient structures of the Lagrangian function as illustrated in Lemma \ref{lem:Vstruct} allows us to handle the contextual, and discretized continuum-arm aspects of the problem. However, there is an additional caveat that remains unhandled: namely the ``flatness'' of the reward function that depends on adversarial contexts, and makes arm exploration difficult. To illustrate (see e.g. Figure \ref{fig:lagr}), we define the slopes that are adjacent to the optimal budget $\arg\max_{\rho_{j}\in[0,\rho]} \mathcal{L}_{j}(\rho_{j},\cont)$ for any $\cont = (\lambda,\mu)$ as followed: assuming the optimal budget $\arg\max_{\rho_{j}\in[0,\rho]} \mathcal{L}_{j}(\rho_{j},\cont)$ is located at the $n$th ``turning point'' $r_{j,n}$ we have
\begin{align}
\label{eq:adj}
\begin{aligned}
    & \slope_{j}^{-}(\cont) = \slope_{j,n}(\cont) 
    ~\text{ and }~ \slope_{j}^{+}(\cont) = \slope_{j,n+1}(\cont)
  \end{aligned}  
\end{align}
Similar to standard multi-arm bandits, the flatter the slope (e.g. $\slope_{j}^{-}(\cont)$ is close to 0), the more pulls required to accurately estimate rewards for sub-optimal arms on the slope, but the lower the loss in conversion for pulling sub-optimal arms. Our setting is challenging because the magnitude of this tradeoff depends on the adversarial contexts $\cont_{t}$, i.e., the dual variables, which requires delicate treatments. In the following Lemma  \ref{lem:ucbregret} where we bound the UCB error, we handle this context-dependent tradeoff by separately analyzing periods during which the adjacent slopes $\slope_{j}^{-}(\cont)$ and $\slope_{j}^{+}(\cont)$ are less or greater than some parameter $\underline{\slope}$, and characterize the context-dependent tradeoff w.r.t. flatness of adjacent slopes using $\underline{\slope}$.
\begin{lemma}[Bounding UCB error in primal per-channel budgets]
\label{lem:ucbregret}
Assume the discretization width $\discerr$ satisfies $\discerr < \underline{r}_{j}:= \min_{n \in [S_{j}]}r_{j,n} - r_{j,n-1}$, where $S_{j}$ and $\{r_{j,n}\}_{n=0}^{S_{j}}$ are defined in Lemma \ref{lem:Vstruct}. Then we have
\begin{align}
        \sum_{t\in[T]} 
     \E\left[\mathcal{L}_{j}(\rho_{j,t}^{*}, \lambda_{t}, \mu_{t}) - \mathcal{L}_{j}(\rho_{j,t}, \lambda_{t}, \mu_{t})\right]~\leq~ \mathcal{O}\left(\discerr T + \underline{\slope} T + \frac{1}{\underline{\slope}\discerr}\right)
    \end{align}
where $\underline{\slope} > 0$ is any small positive number. {\color{red} why is this a good bound? Can we tune $\underline{\slope}$ later?}
\end{lemma}
We refer the readers to Appendix \ref{pf:lem:ucbregret} for the proof. On the other hand,  the bound on SGD complementary slackness violation is presented in the following Lemma \ref{lem:boundcs}, and follows a standard argument for analyses on SGD; we refer readers to the proof in Appendix \ref{pf:lem:boundcs}. 
\begin{lemma}[Bounding complementary slackness deviations]
\label{lem:boundcs}
Recall $g_{1,t} = \sum_{j\in [M]}\left(\totv_{j}(\rho_{j,t};\bm{z}_{t}) - \gamma \rho_{j,t}\right)$, $g_{2,t} = \rho - \sum_{j\in [M]}\rho_{j,t}$ and $\eta > 0$ the step size defined in Algorithm \ref{alg:omducb}. Then we have
    \begin{align}
    \sum_{t\in[T]} \E\left[\lambda_{t}g_{1,t} + \mu_{t}g_{2,t}  \right] ~\leq~ 
    \mathcal{O}\left( \eta  T + \frac{1}{\eta}\right)
    \end{align}
\end{lemma}
Putting Lemmas \ref{lem:ucbregret} and \ref{lem:boundcs}  together into Eq. \eqref{eq:decompregret}, we obtain the main result of this section in the following Theorem \ref{thm:regret} whose proof we detail in Appendix \ref{pf:thm:regret}
\begin{theorem}[Putting everything together]
\label{thm:regret}
Assume assumptions  \ref{ass:budgetbind} and \ref{ass:feas} hold. Let $(\rho_{j,t})_{j\in [M], t\in [T]}$ be the per-channel budgets generated from Algorithm \ref{alg:omducb} and assume we take step size $\eta = \Theta(1/\sqrt{T})$,discretization width $\discerr = \Theta(T^{-1/3}) $, and $\underline{\slope} = \Theta(T^{-1/3})$ in Lemma \ref{lem:ucbregret}. Then we have 
\begin{align}
\label{eq:finalregret}
    T\cdot  \textsc{GL-OPT} - \E\left[\sum_{t\in [T]}\sum_{j\in[M]}\totv_{j}(\rho_{j,t})\right] \leq \mathcal{O}(T^{2/3}).
\end{align}
Recalling $\overline{\bm{\rho}}_{T} = \left(\frac{1}{T}\sum_{t\in[T]} \rho_{j,t}\right)_{j\in [M]}$ is the vector of time-averaged per-channel budgets, we have 
$ \textsc{GL-OPT} - \sum_{j \in [M]}\E\left[\totv_{j}(\overline{\rho}_{T,j})\right] \leq \mathcal{O}(T^{-1/3})$, and further $ \sum_{j \in [M]}\E\left[\totv_{j}(\overline{\rho}_{T,j}) -\gamma \overline{\rho}_{T,j}\right] \geq -\mathcal{O}(T^{-1/2})$ and $\rho - \sum_{j \in [M]}\E[\overline{\rho}_{T,j}] \geq -\mathcal{O}(T^{-1/2})$. {\color{red} in words, say this means the constraint of the problem are satisfied in expectation. }
\end{theorem}

{\color{red} NG: could we say sth about why this is a good bound?}
% \textit{Proof sketch.}
% Proposition \ref{prop:ubbenchlag} allows us to decompose total regret into two parts, namely the error induced by the UCB component in our algorithm, and the error due to deviations from complementary slackness:
% \begin{align}
% \begin{aligned}
%       & T\cdot  \textsc{GL-OPT} - \E\left[\sum_{t\in [T]}\sum_{j\in[M]}\totv_{j}(\rho_{j,t})\right] \\
%      ~\leq~& \sum_{j\in [M]}\underbrace{\sum_{t\in[T]} 
%      \E\left[\mathcal{L}_{j}(\rho_{j}^{*}(t), \lambda_{t}, \mu_{t})  - \mathcal{L}_{j}(\rho_{j,t}, \lambda_{t}, \mu_{t})\right]}_{\leq \mathcal{O}\left(\discerr T + \underline{\slope} T + \frac{1}{\underline{\slope}\discerr}\right)}+ \underbrace{\sum_{t\in[T]}\E\left[\lambda_{t}g_{1,t} + \mu_{t}g_{2,t}\right]}_{ \mathcal{O}\left( \eta  T + \frac{1}{\eta}\right)}
%       \end{aligned}
%  \end{align}
%  Here, the first bound follows from Lemma \ref{lem:ucbregret}, and the second bound follows from Lemma \ref{lem:boundcs}. By taking $\underline{\slope} = \discerr = T^{-1/3}$ and $\eta = 1/\sqrt{T}$, we can obtain Eq. \eqref{eq:finalregret}.  The conversion error for $\overline{\bm{\rho}}_{T}$, namely $\textsc{GL-OPT} - \sum_{j \in [M]}\totv_{j}(\overline{\rho}_{T,j}) \leq \mathcal{O}(T^{-1/3})$, follows directly from concavity of $\totv_{j}(\rho_{j})$ in $\rho_{j}$ for all $j\in [M]$ according to Lemma \ref{lem:Vstruct}. Constraint approxmations at $\overline{\bm{\rho}}_{T}$ follows from Lemma \ref{lem:approxconst} and again concavity of $\totv_{j}(\rho_{j})$.
 




% \begin{lemma}[Bounding dual variables and Lagrangian]
% \label{lem:dualvarub}
% Let $(\lambda_{t},\mu_{t})_{t\in [T]}$ be the variables generated from Algorithm \ref{alg:omducb}. Assuming the stepsize $\eta > 0$ satisfies $\eta < \frac{1}{M \max\left\{\totv, \rho, \totv^{2}\right\}}$, there exists some absolute constant $\dualub_{F} > 0$ that depends only on the support of value-cost pairs  $F = F_{1} \times \dots \times F_{M}$ as well as aggregate ROI and budget $(\gamma,\rho)$ such that $\lambda_{t},\mu_{t} \leq \dualub_{F}$ for all $t \in [T]$. Moreover, for any for any $t\in [T]$, $j\in [M]$ and $\rho_{j} \in [0,\rho]$ we have 
% \begin{align}
%    -\left(1+\gamma \right)\rho\dualub_{F}
%    ~\leq~ \mathcal{L}_{j}(\rho_{j},\lambda_{t},\mu_{t})~\leq~(1+\dualub_{F})\Bar{\totv}\,.
% \end{align}
% \end{lemma}
% See proof in Appendix \ref{pf:lem:dualvarub}.


% \begin{lemma}[Approximate constraint satisfaction]
% \label{lem:approxconst}
% Assume Assumption \ref{ass:feas} holds. If Algorithm \ref{alg:omducb} is run with stepsize $\eta = 1/\sqrt{T}$ such that $\eta < \frac{1}{M \max\left\{\totv, \rho, \totv^{2}\right\} }$, then we have 
% \begin{align*}
%      \frac{1}{T}\sum_{t\in[T]}g_{1,t} \geq -\dualub_{F}/\sqrt{T} \text{ and }
%   \frac{1}{T}\sum_{t\in[T]}g_{2,t} \geq -\dualub_{F}/\sqrt{T} 
% \end{align*}
% where we recall $g_{1,t} = \sum_{j\in [M]}\left(\totv_{j}(\rho_{j,t};\bm{z}_{t}) - \gamma \rho_{j,t}\right)$, $g_{2,t} = \rho - \sum_{j\in [M]}\rho_{j,t}$, and $\dualub_{F} >0 $ is an absolute constant defined in Lemma \ref{lem:dualvarub} that depends only on the support $F = F_{1} \times \dots F_{M}$.
% \end{lemma}



\subsection{Extension to strict constraint satisfaction: UCB-SGD-II}
In Theorem \ref{thm:regret}, we showed that the final output of the UCB-SGD Algorithm \ref{alg:omducb} outputs a per-channel budget profile $\overline{\bm{\rho}}_{T} = \left(\frac{1}{T}\sum_{t\in[T]} \rho_{j,t}\right)_{j\in [M]}$ that satisfies both ROI and budget constraints in $\textsc{CH-OPT}(\mathcal{I}_{\budg})$ approximately, i.e. there can be at most violations in the magnitude of $\mathcal{O}(T^{-1/2})$ for both constraints. In this subsection, we present a modification to UCB-SGD that enables us to achieve no-constraint violations, while still maintaining the $\mathcal{O}(T^{-1/3})$ accuracy in total conversion. Similar modification techniques have been introduced in \cite{balseiro2022best,feng2022online}. 

Our modification strategy handles ROI and budget constraint satisfactions differently. For budget constraints, we simply terminate the entire algorithm once the total spend comes close to $\rho T$. Regarding the ROI constraint, we develop two phases. Phase 1 is a ``safety phase'' where we conservatively utilize channel levers to accumulate a positive ``ROI balance'', i.e. in this phase (assume ending in period $T'$) we hope to achieve $\sum_{t\in [T']}g_{1,t} \geq \Theta(\sqrt{T})$ {\color{red}NG: $\Theta(\sqrt{T})$ or $\Theta(\sqrt{T'})$?}, where we recall $g_{1,t}$ defined in step 4 of Algorithm \ref{alg:omducb} can be viewed as the ROI constraint violations in period $t$. For phase 2, we then naively run SGD-UCB. Here, we aim to have a positive ROI balance in phase 1 that will be used to  compensate possible constraint violations in phase 2 when we run SGD-UCB. 

We remark that in order to implement the safety phase to attain a positive ROI balance, we resort to per-channel ROIs $(\gamma_{j})_{j\in[M]}$, since setting $\gamma_{j} = \gamma$ for all channels will ensure that our ROI balance increases. {\color{red}NG: did not understand  ``since setting $\gamma_{j} = \gamma$ for all channels will ensure that our ROI balance increases"} From a high level,  SGD-UCB attempts to approximate the optimal solution for $\textsc{CH-OPT}(\mathcal{I}_{\budg})$ by solely using the per-channel budget lever, whereas in the above modification with the usage of per-channel ROIs hopes to approximate an optimal solution to 
$\textsc{CH-OPT}(\mathcal{I}_{G})$ 
for the general option (see Eq. \eqref{eq:option}) which is inspired by the fact that  $\textsc{CH-OPT}(\mathcal{I}_{G}) = \textsc{CH-OPT}(\mathcal{I}_{\budg})=\textsc{GL-OPT}$ according to Lemma \ref{cor:roiredund} and Corollary \ref{cor:roiredund}. We call this modified algorithm SGD-UCB-II, and summarize details in Algorithm \ref{alg:omducb2}. {\color{red} NG: this is a nice insight. We show that if we are OK with satisfying the constraint with some small error, considering per-channel ROI constraint is not required. But, this is no longer the case where we cannot tolerate any constraint violations.}

\begin{algorithm}[H]
    \centering
    \caption{SGD-UCB-II}\label{alg:omducb2}
    \footnotesize
    \begin{algorithmic}[1]
    \Require{Set $B_{1}=\rho T$, and $g_{1,0} = 0$.}
    \While{$\sum_{t' \in [t-1]}g_{1,t'} \leq \sqrt{T}\log(T)$}
    \If{$B_{t} < M\rho $ {\color{red} NG: what is $B_t$? I know what it is. But, I don't think you defined it anywhere. }}
         \State Terminate  algorithm and output $\overline{\bm{\rho}}_{t} = \left(\frac{1}{t}\sum_{t'\in[t]} \rho_{j,t'}\right)_{j\in [M]}$.
    \EndIf
    \State  Set $\gamma_{j,t} = \gamma$ and $\rho_{j,t} = \rho$ for all $j \in [M]$ 
    \State Observe $\left\{\totv_{j}(\rho_{j,t};\bm{z}_{t}) \right\}_{j \in [M]}$, and calculate $g_{1,t} = \sum_{j \in M} \left(\totv_{j}(\rho_{j,t};\bm{z}_{t}) -  \gamma \rho_{j,t}\right)$
    \State Calculate $B_{t+1} = B_{t} - \sum_{j\in [M]}\rho_{j,t}$.
    \State Increment $t \leftarrow t+1$
	\EndWhile
 \State For remaining $T - t$ periods, set $\hat{\rho} = B_{t}/(T-t)$, and run SGD-UCB$(\gamma,\hat{\rho})$  in Algorithm \ref{alg:omducb}.
 \State Output $\overline{\bm{\rho}}_{T} = \left(\frac{1}{T}\sum_{t\in[T]} \rho_{j,t}\right)_{j\in [M]}$.
    \end{algorithmic}
\end{algorithm}
Our main result in this subsection is the following Theorem \ref{thm:regret2}:
\begin{theorem}
\label{thm:regret2}
    Let $\overline{\bm{\rho}} \in [0,\rho]^{M}$ be the final output of SGD-UCB-II in Algorithm \ref{alg:omducb2}. Then under the same assumptions and SGD-UCB parameter choices in Theorem \ref{thm:regret}, we have
$ \textsc{GL-OPT} - \sum_{j \in [M]}\E\left[\totv_{j}(\overline{\rho}_{j})\right]\leq \mathcal{O}(T^{-1/3})$, and further $\sum_{j \in [M]}\E\left[\totv_{j}(\overline{\rho}_{j}) -\gamma \overline{\rho}_{j}\right]\geq 0 $ and $ \sum_{j \in [M]} \E\left[\overline{\rho}_{j}\right]\leq \rho$. 
\end{theorem}

==> 4_online_v1.tex <==
In this section, we develop an efficient algorithm to solve for per-channel budgets that optimize
$\textsc{CH-OPT}(\mathcal{I}_{\budg})$ defined in Eq. \eqref{eq:chopt}, which achieves the theoretical optimal conversion, namely $\textsc{GL-OPT}$, as illustrated in Theorem \ref{thm:budgonlysuff}. In particular, we consider algorithms that run over $T > 0$ periods, where each period for example corresponds to the duration of 1 hour or 1 day. At the end of $T$ periods, the algorithm  produces some per-channel budget profile $(\rho_{j})_{j\in [M]}\in [0,\rho]^{M}$ that approximates $\textsc{CH-OPT}(\mathcal{I}_{\budg})$,  and satisfies aggregate budget and ROI constraints, namely 
\begin{align}
\begin{aligned}
\label{eq:constraintT}
 &  \text{ROI:} \quad  \sum_{j \in M} \totv_{j}(\rho_{j}) \geq \gamma \sum_{j \in M} \totc_{j}(\rho_{j}), ~\text{ and }~ \text{Budget:} \quad  \sum_{j\in [M]}\totc_{j}(\rho_{j})\leq \rho\,,
 \end{aligned}
\end{align}
where we recall the expected conversion and spend functions $(\totv_{j}(\rho_{j}),\totc_{j}(\rho_{j}))$ defined in Eq. \eqref{eq:budperchannel}.

The algorithm proceeds as follows: at the beginning of period $t\in [T]$, the advertiser sets per-channel budgets $(\rho_{j,t})_{j\in [M]}$, while simultaneously values and costs $\bm{z}_{t}=(\bm{v}_{j,t}, \bm{d}_{j,t})\in \R_{+}^{M_{j}}\times \R_{+}^{M_{j}}$ are sampled (independently in each period) from  finite support $F = F_{1}\times \dots F_{M}$ according to discrete distributions $(\bm{p}_{j})_{j\in[M]}$. Each channel $j$ then takes as input $\rho_{j,t} \in [0,\rho]$ and procures ads on behalf of the advertiser, and reports the total realized conversion $\totv_{j}(\rho_{j,t};\bm{z}_{t})$ as well as total spend $\totc_{j}(\rho_{j,t};\bm{z}_{t}) $ to the advertiser, where $\totv_{j}(\rho_{j,t};\bm{z}_{t})$ and $\totc_{j}(\rho_{j,t};\bm{z}_{t})$ are defined in Eq. \eqref{eq:budperchannel}. For simplicity we also assume for any realization $\bm{z} = (\bm{v}_{j},\bm{d}_{j}) \in F$ we have the ordering $\frac{v_{j,1}}{d_{j,1}} > \frac{v_{j,2}}{d_{j,2}} > \dots  > \frac{v_{j,m_{j}}}{d_{j,m_{j}}}$ for all channels $j \in [M]$.

Here, we highlight that the advertiser receives \textit{bandit feedback} from channels, i.e. the advertiser only observes the numerical values $\totv_{j}(\rho_{j,t}; \bm{z}_{t})$ and $\totc_{j}(\rho_{j,t}; \bm{z}_{t})$, but does not get to observe 
$\totv_{j}(\rho_{j}'; \bm{z}')$ and $\totc_{j}(\rho_{j}'; \bm{z}')$ evaluated at any other per-channel budget $\rho_{j}'\neq \rho_{j,t}$ and realized value-cost pairs $\bm{z}'\neq \bm{z}_{t}$. More discussions on challenges that arise from this bandit feedback structure can be found in 
Section \ref{subsec:algo}.

% \begin{algorithm}[H]
%     \centering
%     \caption{Explore-exploit under noisy bandit feedback}\label{alg:ee}
%     \footnotesize
%     \begin{algorithmic}[1]
%     \Require Exploration length $E$, budget discretization $\discerr > 0$ s.t. $\budgset = \{\budg_{h}\}_{h\in \left[{\rho}/{\discerr}\right]}$ where $\budg_{h} = h\discerr$. Stepsizes $\{\eta\}_{t\in[T]}$.
% {\Statex{\textbf{Exploration}}}:
%     \For{$h \in \left[\frac{\rho}{\discerr}\right]$ and $j\in [M]$}
%         \State Set budget $\budg_{h}$ for $E$ periods in channel $j$, and record empirical channel value $\Bar{\totv}_{j}(\budg_{h})$
%     \EndFor
%     {\Statex{\textbf{Exploitation}}}:
% 	\For{$t = EM  \left[{\rho}/{\discerr}\right]\dots T$ }
% 	 \State For each channel $j\in [M]$ set primal decision
%         \begin{align}
%           \rho_{j,t} = \arg\max_{\rho_{j}\in \budgset}\quad (1+\lambda_{t})\Bar{\totv}_{j}(\rho_{j}) - \left(\lambda_{t} \gamma + \mu_{t} \right)\rho_{j} 
%           \end{align}
%     \State Update dual variables
%         with realized values $\left\{\widetilde{\totv}_{j}(\rho_{j,t}) \right\}_{j \in [M]}$
%         \begin{align}
%         & \lambda_{t+1} =\lambda_{t} - \eta \cdot \left(\sum_{j \in M} \widetilde{\totv}_{j} -  \gamma \rho_{j,t}\right)\\
%         &  \mu_{t+1}  = \mu_{t} - \eta \cdot \left(\rho - \sum_{j\in [M]} \rho_{j,t}\right)
%         \end{align}
% 	\EndFor
%     \end{algorithmic}
% \end{algorithm}

We also make the following Assumption \ref{ass:budgetbind} that states that if the advertiser allocates any feasible per-channel budget to a channel $j\in [M]$, the channel will almost surely deplete the entire budget in the impression procurement process. This is a natural assumption that mimics practical scenarios, e.g. small businesses who have moderate-sized budgets.
\begin{assumption}[Moderate budgets]
\label{ass:budgetbind}
 We assume the total budget is finite, i.e. $\rho < \infty$, and for any channel $j \in [M]$, value-cost realization $\bm{z} = (\bm{v}, \bm{d}) \in F_{j}$, and per-channel budget $\rho_{j} \in [0,\rho]$, the optimal solution $\bm{x}_{j}^{*}(\rho;\bm{z})$ defined in Eq. \eqref{eq:budperchannelsol} is budget binding, i.e. $\totc_{j}(\rho_{j};\bm{z}) = \bm{d}_{j}^{\top}\bm{x}_{j}^{*}(\rho_{j};\bm{z}) = \rho_{j}$.
\end{assumption}
% Under Assumption \ref{ass:budgetbind}, we can show that the total spend in each channel exactly matches the input per-channel budget, and we present the proof in Appendix \ref{pf:prop:budgetbind} 
% \begin{proposition}
% \label{prop:budgetbind}
% Under Assumption \ref{ass:budgetbind}, for any channel $j\in [M]$ and per-channel budget $\rho_{j}\in [0,\rho]$, the optimal solution $\bm{x}_{j}^{*}(\rho_{j};\bm{z})$ defined in Eq. \eqref{eq:budperchannelsol} is budget binding, i.e. $\totc_{j}(\rho_{j};\bm{z}) =\bm{d}_{j}^{\top}\bm{x}_{j}^{*}(\rho_{j};\bm{z}) = \rho_{j}$. 
% \end{proposition}

\subsection{The SGD-UCB algorithm to optimize per-channel budgets}
\label{subsec:algo}
Here, we describe our algorithm to solve for optimal per-channel budgets w.r.t.  $\textsc{CH-OPT}(\mathcal{I}_{\budg})$. Similar to most algorithms for constrained optimization, we take a dual stochastic gradient descent (SGD) approach; see a comprehensive survey on dual descent methods in \cite{bertsekas2014constrained}. First, we consider the Lagrangian functions w.r.t. $\textsc{CH-OPT}(\mathcal{I}_{\budg})$ where we let  $\cont = (\lambda, \mu) \in \R_{+}^{2}$ be the dual variables corresponding to the ROI and budget constraints, respectively:
\begin{align}
    \label{eq:Lagrangian}
    \mathcal{L}_{j}(\rho_{j}, \cont; \bm{z}_{j}) =  (1+\lambda)\totv_{j}(\rho_{j};\bm{z}_{j}) - (\lambda \gamma  + \mu) \rho_{j} ~\text{ and }~\mathcal{L}_{j}(\rho_{j}, \cont) = \E\left[  \mathcal{L}_{j}(\rho_{j}, \cont; \bm{z}_{j})\right]\,.
\end{align}
Then, in each period $t\in [T]$ given dual  variables $\cont_{t} = (\lambda_{t},\gamma_{t})$, SGD decides on a primal decision, i.e. per-channel budget $(\rho_{j,t})_{j\in[M]}$ by optimizing the following:
\begin{align}
\label{eq:SGDprimal}
    \rho_{j,t} ~=~ \arg\max_{\rho_{j}\in [0,\rho]}\mathcal{L}_{j}(\rho_{j}, \cont_{t};\bm{z}_{t})\,.
\end{align}
Having observed the realized values $\left(\totv_{j}(\rho_{j,t};\bm{z}_{t})\right)_{j\in[M]}$ (note that spend is $(\rho_{j,t})_{j\in [M]}$ in light of Assumption \ref{ass:budgetbind}),  we calculate the current period violation in budget and ROI constraints, namely  $g_{1,t}:= \sum_{j \in M} \left(\totv_{j}(\rho_{j,t};\bm{z}_{t}) -  \gamma \rho_{j,t}\right)$ and $g_{2,t} = \rho - \sum_{j\in [M]} \rho_{j,t}$. Next, we update dual variables via $ 
\lambda_{t+1} = \left(\lambda_{t} - \eta g_{1,t}\right)_{+} \text{ and } \mu_{t+1}  = \left(\mu_{t} - \eta g_{2,t}\right)_{+}$, where $\eta$ is some pre-specified step size.\footnote{Here, the dual updates follow the vanilla gradient descent approach, and one can also employ more general mirror descent updates; see e.g. \cite{balseiro2022best}.}

However, the above SGD approach faces a fatal drawback, namely we cannot realistically find the primal decisions by solving Eq. \eqref{eq:SGDprimal} since the function $\mathcal{L}_{j}(\cdot, \cont_{t};\bm{z}_{t})$ is unknown due to the  bandit feedback  structure. Therefore, we provide a modification to SGD to handle this issue. Before we present our approach, we briefly note that although bandit feedback prevents the naive application of SGD for our problem of interest, this may not be the case in other online advertising scenarios that involve relevant learning tasks, underlining the challenges of our problem; see following Remark \ref{rmk:banditfeedback} for details.
\begin{remark}
\label{rmk:banditfeedback}
Our problem of interest under bandit feedback is more difficult than similar problems in related works that study online bidding strategies under budget and ROI constraints; see e.g. \cite{balseiro2017budget,balseiro2022best,feng2022online}. To illustrate, consider for instance  \cite{balseiro2017budget} in which a budget constrained advertiser's primal decision at period $t$ is to submit a bid value  $b_{t}$ after observing her value $v_{t}$. The advertiser competes with some unknown  highest competing bid $d_{t}$ in the market, and after submitting bid $b_{t}$, does not observe $d_{t}$ if she does not win the competition, which involves a semi-bandit feedback structure. Nevertheless, the corresponding Lagrangian under SGD takes the special form $\mathcal{L}_{j}(b, \mu_{t};\bm{z}_{t}) =\left(v_{t} - (1+\mu_{t})d_{t}\right)\I\{b_{t} \geq d_{t}\}$ where $\mu_{t}$ is the dual variable w.r.t. the budget constraint.  This simply allows an advertiser to optimize for her primal decision by bidding $\arg\max_{b\geq 0} \mathcal{L}_{j}(b, \cont_{t};\bm{z}_{t}) = \frac{v_{t}}{1+\mu_{t}}$. So even though \cite{balseiro2017budget,balseiro2022best,feng2022online} study dual SGD under bandit feedback, the special structures of their problem instances permits SGD to effectively optimize for primal decisions in each period, as opposed to Eq. \eqref{eq:SGDprimal} in our setting which can not be  solved.
\end{remark}
To resolve challenges that arise with bandit feedback in our model, we take a natural approach to augment SGD with the \textit{upper-confidence bound (UCB)} algorithm, which is well celebrated for solving learning problems under bandit feedback such as multi-arm bandits; see an introduction to bandits in \cite{slivkins2019introduction}. In particular, we first discretize our per-channel buudget decision set $[0,\rho]$ into granular ``arms'' that are separated by some distance $\discerr > 0$, so that the discretized per-channel budget decisions become
\begin{align}
\label{eq:budgetdisc}
    \budgset(\discerr) = \{a_{k}\}_{k \in [K]} \text{ where } a_{k} = (k-1)\discerr \text{ and }K := \lceil{\rho}/{\discerr}\rceil + 1\,.
\end{align}
In the following we will use the terms ``per-channel budget'' and ``arm'' interchangeably. In the spirit of UCB, in each period $t$ we maintain some estimate $\left(\Hat{\totv}_{j,t}(a_{k})\right)_{j\in[M]}$ of the conversions $\left(\totv_{j}(a_{k})\right)_{j\in [M]}$ as well as an upper confidence bound $\ucb_{j,t}(a_{k})$ for each arm $a_{k}$ using historical payoffs from periods in which arm $a_{k}$ is pulled. Finally, we update primal decisions for each channel $j\in[M]$ using the ``best arm'' $\rho_{j,t} = \arg\max_{a_{k}\in \budgset(\discerr)}~(1+\lambda_{t})\left(\Hat{\totv}_{j,t}(a_{k}) +  \ucb_{j,t}(a_{k})\right) - \left(\lambda_{t} \gamma + \mu_{t} \right)a_{k}$. We summarize our algorithm, called SGD-UCB, in the following Algorithm \ref{alg:omducb}.

\begin{algorithm}[ht]
    \centering
    \caption{SGD-UCB}\label{alg:omducb}
    \footnotesize
    \begin{algorithmic}[1]
    \Require Budget discretization decision set  $\budgset(\discerr)$ defined in Eq.\eqref{eq:budgetdisc}. Step size $\eta > 0$. Initialize $ N_{j,1}(a_{k}) = \Hat{\totv}_{j,1}(a_{k})  = 0$ for all $j \in [M]$ and $k\in [K]$, and dual variables $\lambda_{1} = \mu_{1}= 0$.
    % \For{$t = 1 \dots K$ }
    % \State Set identical budgets in each channel with the $t$'th arm, i.e. $\bm{\rho}_{t} = (a_{t},a_{t}\dots a_{t})\in \budgset(\discerr)^{M}$.
    % \EndFor
    \\
    \textbf{Output:} Per channel budget.  {\color{red} it seems that you did not update the algorithm. Any reason?}  
	\For{$t = 1 \dots T$ }
	 \State \textbf{Update (primal) per-channel budget.} For each channel $j\in [M]$ set (primal) per-channel budget:
  \begin{itemize}
      \item If $t \leq K$, set $\rho_{j,t} = a_{t}$.
      \item If $t > K$, set
      \begin{align}
        \begin{aligned}
        \label{eq:choosearm}
          & \rho_{j,t} = \arg\max_{a_{k}\in \budgset(\discerr)}~\Hat{\totv}_{j,t}(a_{k}) +  \ucb_{j,t}(a_{k}) - \frac{\lambda_{t} \gamma + \mu_{t}}{1+\lambda_{t}} a_{k}, ~\text{ where } \ucb_{j,t}(a_{k}) = \sqrt{\frac{2\log(T)}{N_{j,t}(a_{k})}} 
           \end{aligned}
          \end{align}
  \end{itemize}
    \State  Observe realized values $\left\{\totv_{j}(\rho_{j,t};\bm{z}_{t}) \right\}_{j \in [M]}$, and update for each arm $k \in [K]$:
    \begin{align}
    \begin{aligned}
        & N_{j,t+1}(a_{k}) =  N_{j,t}(a_{k}) + \I\{\rho_{j,t} = a_{k}\}\\
        & \Hat{\totv}_{j,t+1}(a_{k}) = \frac{1}{N_{j,t+1}(a_{k})} \left(N_{j,t}(a_{k}) \Hat{\totv}_{j,t}(a_{k}) + \totv_{j}(\rho_{j,t};\bm{z}_{t}) \I\{\rho_{j,t} = a_{k}\}\right) \quad, \text{ for } j = 1 \dots M
        \end{aligned}
    \end{align}
    \State \textbf{Update dual variables.} Update dual variables with $g_{1,t}:= \sum_{j \in M} \left(\totv_{j}(\rho_{j,t};\bm{z}_{t}) -  \gamma \rho_{j,t}\right)$ and $g_{2,t} = \rho - \sum_{j\in [M]} \rho_{j,t}$:
    % \begin{align}
    %     \label{eq:dualupdate}
        % \begin{aligned}
        % & \dot{h}(\widetilde{\lambda}_{t+1})= \dot{h}(\lambda_{t}) - \epsilon g_{1,t} \text{ and } \dot{h}(\widetilde{\mu}_{t+1})= \dot{h}(\mu_{t}) - \epsilon g_{2,t} \\
        % &  \lambda_{t+1}  = \arg\min_{\lambda\geq 0} \breg_{h}(\lambda,\widetilde{\lambda}_{t+1}) \text{ and }  \mu_{t+1}  = \arg\min_{\mu\geq 0} \breg_{h}(\mu,\widetilde{\mu}_{t+1})
        % \end{aligned}
        % \end{align}
        % where $\breg_{h}(x,y) = h(x) - h(y) - \dot{h}(y)(y-x)$ is the Bregman divergence w.r.t. $h:\R \to \R$.
        \begin{align}
        \label{eq:dualupdate}
        \begin{aligned}
     \lambda_{t+1} = \left(\lambda_{t} - \eta g_{1,t}\right)_{+} \text{ and } \mu_{t+1}  = \left(\mu_{t} - \eta g_{2,t}\right)_{+}
        \end{aligned}
        \end{align}
	\EndFor
 \State Output $\overline{\bm{\rho}}_{T} = \left(\frac{1}{T}\sum_{t\in[T]} \rho_{j,t}\right)_{j\in [M]}$.
    \end{algorithmic}
\end{algorithm}
We remark that there has been very recent works that combine SGD with Thompson sampling which is another well-known algortithm for solving bandit problems (e.g. \cite{ding2021efficient} and references therein), and works that employ SGD in bandit problems (e.g. \cite{han2021generalized}). Yet to the best of our knowledge, approach to augment SGD with UCB is novel.

\subsection{Analyzing the SGD-UCB algorithm}
\label{subsec:analyzealgo}
% In this subsection, we analyze the performance of SGD-UCB in Algorithm \ref{alg:omducb}.  Our strategy is to show the cumulative loss over $T$ periods, namely $T\cdot  \textsc{GL-OPT} - \E\left[\sum_{t\in [T]}\sum_{j\in[M]}\totv_{j}(\rho_{j,t})\right] = \mathcal{O}(T^{\zeta})$ for some $\zeta \in (0,1)$, because using concavity of the $\totv_{j}(\cdot)$ functions directly yields an optimization accuracy $\textsc{GL-OPT} - \E\left[\sum_{j\in[M]}\totv_{j}\left(\frac{\sum_{t\in [T]\rho_{j,t}}}{T}\right)\right]\leq \mathcal{O}(T^{-(1-\zeta})$. Now, the following Proposition \ref{prop:ubbenchlag} allows us to decompose $T\cdot  \textsc{GL-OPT} - \E\left[\sum_{t\in [T]}\sum_{j\in[M]}\totv_{j}(\rho_{j,t})\right]$ into two main parts, namely the error induced by the UCB in our algorithm, and the error due to SGD (or what is typically viewed as the deviations from  complementary slackness):

In this subsection, we analyze the performance of SGD-UCB in Algorithm \ref{alg:omducb}, and present accuracy guarantees on the final output $\overline{\bm{\rho}}_{T} = \left(\frac{1}{T}\sum_{t\in[T]} \rho_{j,t}\right)_{j\in [M]}$ of the algorithm. The backbone of our analysis strategy is to show the cumulative conversion loss over $T$ periods, namely $T\cdot  \textsc{GL-OPT} - \E\left[\sum_{t\in [T]}\sum_{j\in[M]}\totv_{j}(\rho_{j,t})\right]$ consists of two main parts, namely the error induced by the UCB in our algorithm, and the error due to SGD (or what is typically viewed as the deviations from  complementary slackness), as shows in the following Proposition \ref{prop:ubbenchlag}. Then we further bound each part, respectively.
\begin{proposition}
\label{prop:ubbenchlag}
For any channel $ j\in [M]$ define $\rho_{j}^{*}(t) = \arg\max_{\rho_{j\in[M]}}\mathcal{L}_{j}(\rho_{j};\cont_{t})$ to be the optimal per-channel budget w.r.t. dual variables $\cont_{t}=(\lambda_{t},\mu_{t})_{t\in [T]}$ during period $t\in[T]$. Then we have 
 \begin{align}
 \begin{aligned}
 \label{eq:decompregret}
     & T \cdot\textsc{GL-OPT} - \sum_{t\in [T]}\sum_{j\in[M]}\E\left[\totv_{j}(\rho_{j,t})\right] \\ ~\leq~&  M\Bar{V}K +
     \sum_{j\in [M]}\underbrace{\sum_{t> K} 
     \E\left[\mathcal{L}_{j}(\rho_{j}^{*}(t), \lambda_{t}, \mu_{t})  - \mathcal{L}_{j}(\rho_{j,t}, \lambda_{t}, \mu_{t})\right]}_{\text{UCB error}}+ \underbrace{\sum_{t >K}\E\left[\lambda_{t}g_{1,t} + \mu_{t}g_{2,t}\right]}_{\text{SGD complementary slackness deviations}}\,,
      \end{aligned}
 \end{align}
\end{proposition}
 where we recall the definitions of $g_{1,t}$ and $g_{2,t}$ in step 4 of Algorithm \ref{alg:omducb}, and the fact that the conversion $ \totv_{j}(\rho_{j};\bm{z}_{j})$ is bounded above by absolute constant $\Bar{\totv} \in (0,\infty)$ almost surely for any channel $j\in[M]$, $(\gamma_{j},\rho_{j})$ and realization $\bm{z}_{j}$.

The bound on SGD complementary slackness violation is presented in the following Lemma \ref{lem:boundcs}, and follows a standard analyses for SGD; we refer readers to the proof in Appendix \ref{pf:lem:boundcs}.  {\color{red} did we update the paper by having the stopping rule version?}
\begin{lemma}[Bounding complementary slackness deviations]
\label{lem:boundcs}
Recall $g_{1,t} = \sum_{j\in [M]}\left(\totv_{j}(\rho_{j,t};\bm{z}_{t}) - \gamma \rho_{j,t}\right)$, $g_{2,t} = \rho - \sum_{j\in [M]}\rho_{j,t}$ and $\eta > 0$ the step size defined in Algorithm \ref{alg:omducb}. Then we have
    \begin{align}
    \sum_{t>K} \E\left[\lambda_{t}g_{1,t} + \mu_{t}g_{2,t}  \right] ~\leq~ 
    \mathcal{O}\left( \eta  T + \frac{1}{\eta}\right)\,.
    \end{align}
\end{lemma}
\textbf{Challenges in bounding UCB error due to adversarial contexts and continuum-arm dicretization.}
Bounding our UCB error is much more challenging than doing so in classic stochastic multi-arm bandit settings: first, our setup involves discretizing a continuum of arms i.e. our discretization in  Eq.\eqref{eq:budgetdisc} for $[0,\rho]$; second, and more importantly, the dual variables $\{\cont_{t}\}_{t\in[T]}$ are effectively \textit{adversarial contexts} since they are updated via SGD instead of being stochastically sampled from some nice distribution, and correspondingly the Lagrangian function $\mathcal{L}_{j}(a_{k},\cont_{t};\bm{z}_{t})$ can be viewed as a reward function that maps any arm-context pair $(a_{k},\cont_{t})$ to (stochastic) payoffs.  Moreover, the UCB error in Eq.\eqref{eq:decompregret}
concerns a dynamic benchmark $\mathcal{L}_{j}(\rho_{j}^{*}(t),\cont_{t};\bm{z}_{t})$ instead of a single-arm benchmark across all contexts, namely $\max_{a\in\budgset(\discerr)}\mathcal{L}_{j}(a,\cont_{t};\bm{z}_{t})$ . Both continuum-arms and dynamic benchmarks under adversarial contexts have been notorious in making reward function estimations highly inefficient; see e.g. discussions in \cite{agrawal1995continuum,agarwal2014taming}. We further elaborate on additional challenges that adversarial contexts bring about:
\begin{itemize}
    \item \textbf{Boundedness of rewards.} In classic stochastic multi-arm bandtis and UCB, losses in total rewards grow linearly with the magnitude of rewards. In our setting, the reward function, i.e. the Lagrangian function $\mathcal{L}_{j}(a_{k},\cont_{t};\bm{z}_{t})$, scales linearly with the magnitude of contexts (see Eq. \eqref{eq:Lagrangian}, so large contexts (i.e. large dual variables) may lead to large losses.
    \item \textbf{Context-dependent exploration-exploitation tradeoffs.} The typical trade-off for arm exploration and exploitation in our setting depends on the particular values of the contexts (i.e. the dual variables), which means there may exist ``bad'' contexts that lead to poor tradeoffs that require significantly more explorations to achieve accurate estimates of arm rewards than  other ``good'' contexts. We elaborate more in Lemma \ref{lem:ucbregret} and discussions thereof.
\end{itemize}
 In the following, we first handle continuum arm discretization and dynamic contextual benchmarks via analyzing structural properties of the reward (i.e. Lagrangian) functions. Fortunately,  the specific form of conversion functions $\totv(\rho_{j};\bm{z})$ defined in Eq. \eqref{eq:budperchannelsol} imposes a salient structure on the Lagrangian for pulling an arm. Specifically, the following lemma shows that the Lagrangian is continuous, piece-wise linear, concave, and unimodal\footnote{We say a real-valued function $f:\R\to \R$ is unimodal if there exists some $y^{*}$ such that $f(y)$ strictly increases when $y \leq y^{*}$ and  strictly decreases when $y \geq y^{*}$.}; we present the proof in Appendix \ref{pf:lem:Vstruct}
% \begin{definition}[Unimodal functions]
% We say a real-valued function $f:\R\to \R$ is unimodal if there exists some $y^{*}$ such that $f(y)$ strictly increases when $y \leq y^{*}$ and  strictly decreases when $y \geq y^{*}$.
% \end{definition}
\begin{lemma}[Structural properties of conversion  and Lagrangian functions]
\label{lem:Vstruct}
\begin{itemize}
\item
For any channel $j\in [M]$ and per-channel budget $\rho_{j}$, the conversion function $\totv_{j}(\rho_{j})$ is continuous, piece-wise linear, strictly increasing, and concave. In particular,  $\totv_{j}(\rho_{j})$ takes the form
\begin{align}
\label{eq:Vstruct}
        \totv_{j}(\rho_{j}) = \sum_{n\in [S_{j}]} \left(s_{j,n} \rho_{j} + b_{j,n}\right)\I\{r_{j,n-1}\leq \rho_{j} \leq r_{j,n}\}\,,
\end{align}
where the parameters $S_{j} \in \N$ and $\{(s_{j,n},b_{j,n},r_{j,n})\}_{n\in [S_{j}]}$ only depend on the support $F_{j}$ and distribution $\bm{p}_{j}$ from which value-to-cost pairs are sampled.  These parameters satisfy
$s_{j,1} > s_{j,2} > \dots > s_{j,S_{j}} > 0$ and $0=r_{j,0} < r_{j,1} < r_{j,2} < \dots < r_{j,S_{j}} =\rho$, as well as $b_{j,n} > 0$ s.t. $s_{j,n} r_{j,n} + b_{j,n} = s_{j,n+1} r_{j,n} + b_{j,n+1}$ for all $n \in [S_{j}-1]$, implying $\totv_{j}(\rho_{j}) $ is continuous  in $\rho_j$.
\item For any dual variables $\cont = (\lambda,\mu) \in \R_{+}^{2}$, the Lagrangian function $ \mathcal{L}_{j}(\rho_{j},\cont)$ defined in Eq. \eqref{eq:Lagrangian} is continuous, piece-wise linear, concave, and unimodal in $\rho_{j}$. In particular,
\begin{align}
\label{eq:lagrrep}
        \mathcal{L}_{j}(\rho_{j}, \cont) =  \sum_{n\in [S_{j}]} \left( \slope_{j,n}(\cont) \rho_{j} + (1+\lambda)b_{j,n}\right)\I\{r_{j,n-1}\leq \rho_{j} \leq r_{j,n}\}\,,
\end{align}
where the slope $\slope_{j,n}(\cont) = (1+\lambda) s_{j,n} -(\mu + \gamma \lambda)$. 
Then, this also implies $\arg\max_{\rho_{j}\geq 0} \mathcal{L}_{j}(\rho_{j}, \cont) = \max\{r_{j,n}:n=0,1\dots, S_{j}~,\slope_{j,n}(\cont) \geq 0\}$.
\end{itemize}
\end{lemma}
In fact,  for any realized value-cost pairs $\bm{z}$, the ``realization 
versions'' of the conversion and Lagrangians functions, namely $\totv_{j}(\rho_{j};\bm{z}) $ and $\mathcal{L}_{j}(\rho_{j}, \cont;\bm{z})$,  also satisfy the same properties as those of $\totv_{j}(\rho_{j})$ and $\mathcal{L}_{j}(\rho_{j}, \cont)$, respectively. We provide a visual illustration for these structural properties in Figure \ref{fig:lagr}. 

\begin{figure}[ht]
\begin{center}
\includegraphics[width=0.8\textwidth]{lagr.png}
\caption{Illustration of Lagrangian functions defined in Eq. \eqref{eq:Lagrangian} with $M_{j} = 2$ auctions in channel $j$, and support $F_{j}$ that contains 3 elements,  $\bm{z}_{(1)} = (\bm{v}_{(1)},\bm{d}_{(1)}) = ((8,2), (2,3))$, $\bm{z}_{(2)} = ((3,4), (1,4))$, $\bm{z}_{(3)} = ((8,1), (4,2))$, and context $\cont = (\lambda,\mu) = (4,2)$. In light of Lemma \ref{lem:Vstruct}, $S_{j} = 5$, where the ``turning points'' $r_{j,0} \dots r_{j,S_{j}}$ are indicated on the x-axis, and the optimal budget w.r.t. $\cont$ is $\arg\max_{\rho_{j}\in [0,\rho]}\mathcal{L}_{j}(\rho_{j};\cont) = r_{j,2}$. The adjacent slopes in Eq. \eqref{eq:adj} are $\slope_{j}^{-}(\cont) = \slope_{j,2}(\cont)$, and  $\slope_{j}^{+}(\cont) = \slope_{j,3}(\cont)$, respectively.}
\label{fig:lagr}
\end{center}
\end{figure}




We now handle the reward boundedness issue in the Lagrangian functions defined in Eq. \eqref{eq:Lagrangian} that arise from adversarial contexts. In the following Lemma \ref{lem:dualvarub}, we show that 
the Lagrangian functions, as well as dual variables, are indeed bounded by some absolute constants under a mild feasibility Assumption \ref{ass:feas} stated below:
\begin{assumption}[Strictly feasible global ROI constraints]
\label{ass:feas}
For any realization of value-cost pairs  $\bm{z} =(\bm{v}_{j},\bm{d}_{j})_{j\in[M]} \in F_{1}\times \dots F_{M}$, the realized version of the ROI constraint in \textsc{GL-OPT} defined in Eq. \ref{eq:glopt} is strictly feasible, i.e. the set $\left\{\bm{x}= (\bm{x}_{j})_{j\in [M]}: \bm{x}_{j} \in [0,1]^{m_{j}} \text{ for }\forall j\in [M],~\sum_{j\in[M]}\bm{v}_{j}^{\top} \bm{x}_{j} > \gamma\sum_{j\in[M]}\bm{d}_{j}^{\top}\bm{x}_{j}\right\}$ is nonempty.\footnote{Equivalently, for any realization of value-cost pairs  $\bm{z} = (\bm{v}_{j},\bm{d}_{j})_{j\in[M]}$ there always exists a channel $j\in [M]$ and an auction  $n\in [m_{j}]$ in this channel  whose value-to-cost ratio is at least $\gamma$, i.e. $v_{j,n} >  \gamma d_{j,n}$.}
\end{assumption}
\begin{lemma}[Bounding dual variables and Lagrangian functions]
\label{lem:dualvarub}
Let $(\lambda_{t},\mu_{t})_{t\in [T]}$ be the variables generated from Algorithm \ref{alg:omducb}. Under Assumption \ref{ass:feas}, and assuming the step size $\eta > 0$ satisfies $\eta < \frac{1}{M \sqrt{(\Bar{\totv}+\gamma\rho)^{2} + \rho^{2}}}$, there exists some absolute constant $\dualub_{F} > 0$ that depends only on the support of value-cost pairs  $F = F_{1} \times \dots \times F_{M}$, as well as aggregate target ROI and budget $(\gamma,\rho)$,  such that $\lambda_{t},\mu_{t} \leq \dualub_{F}$ for all $t \in [T]$. Moreover, for any for any $t\in [T]$, $j\in [M]$ and $\rho_{j} \in [0,\rho]$ we have 
\begin{align}
   -\left(1+\gamma \right)\rho\dualub_{F}
   ~\leq~ \mathcal{L}_{j}(\rho_{j},\cont_{t})~\leq~(1+\dualub_{F})\Bar{\totv}\,.
\end{align} 
\end{lemma}
See the proof in Appendix \ref{pf:lem:dualvarub}.

Finally, we address the context-dependent exploration-exploitation tradeoff. We remark that
this tradeoff is embodied in the ``flatness'' of the reward function that depends on adversarial contexts. To illustrate (see e.g. Figure \ref{fig:lagr}), we define the slopes that are adjacent to the optimal budget $\arg\max_{\rho_{j}\in[0,\rho]} \mathcal{L}_{j}(\rho_{j},\cont)$ for any $\cont = (\lambda,\mu)$ as followed: assuming the optimal budget $\arg\max_{\rho_{j}\in[0,\rho]} \mathcal{L}_{j}(\rho_{j},\cont)$ is located at the $n$th ``turning point'' $r_{j,n}$ we have
\begin{align}
\label{eq:adj}
\begin{aligned}
    & \slope_{j}^{-}(\cont) = \slope_{j,n}(\cont) 
    ~\text{ and }~ \slope_{j}^{+}(\cont) = \slope_{j,n+1}(\cont)
  \end{aligned}  
\end{align}
Similar to standard multi-arm bandits exploration-exploitation tradeoffs, the flatter the slope (e.g. $\slope_{j}^{-}(\cont)$ is close to 0), the more pulls required to accurately estimate rewards for sub-optimal arms on the slope, but the lower the loss in conversion for pulling sub-optimal arms. Our setting is challenging because the magnitude of this tradeoff depends on the adversarial contexts $\cont_{t}$, i.e., the dual variables, which requires delicate treatments. In the following Lemma  \ref{lem:ucbregret} where we bound the UCB error, we handle this context-dependent tradeoff by separately analyzing periods during which the adjacent slopes $\slope_{j}^{-}(\cont)$ and $\slope_{j}^{+}(\cont)$ are less or greater than some parameter $\underline{\slope}$, and characterize the context-dependent tradeoff w.r.t. flatness of adjacent slopes using $\underline{\slope}$.
\begin{lemma}[Bounding the UCB error in  per-channel budgets]
\label{lem:ucbregret}
Assume the discretization width $\discerr$ satisfies $\discerr < \underline{r}_{j}:= \min_{n \in [S_{j}]}r_{j,n} - r_{j,n-1}$, where $S_{j}$ and $\{r_{j,n}\}_{n=0}^{S_{j}}$ are defined in Lemma \ref{lem:Vstruct}. Then we have
\begin{align}
        \sum_{t > K} 
     \E\left[\mathcal{L}_{j}(\rho_{j}^{*}(t), \cont_{t}) - \mathcal{L}_{j}(\rho_{j,t}, \cont_{t})\right]~\leq~ \widetilde{\mathcal{O}}\left(\discerr T + \underline{\slope} T + \frac{1}{\underline{\slope}\discerr} + \frac{1}{\discerr T}\right)\,,
    \end{align} 
    where $\underline{\slope} > 0$ is any small positive absolute constant that we can specify later, and recall $\rho_{j}^{*}(t) = \arg\max_{\rho_{j\in[M]}}\mathcal{L}_{j}(\rho_{j};\cont_{t})$ is the optimal per-channel budget w.r.t. dual variables $\cont_{t}$. $\widetilde{\mathcal{O}}$ hides all logarithmic factors.
\end{lemma}
 We refer the readers to Appendix \ref{pf:lem:ucbregret} for the proof. Note that the parameter $\underline{\slope}$ will be chosen later. Finally, returning to bounding the UCB error in Proposition \ref{prop:ubbenchlag}, we put together Lemmas \ref{lem:boundcs} and \ref{lem:ucbregret}, and obtain the main result of this section in the following Theorem \ref{thm:regret} whose proof we detail in Appendix \ref{pf:thm:regret}.
 % {\color{red} IMPORTANT: Here is a high level issue that we need to step back and think about it. In the problem we have there is are optimal dual solutions that lead to an optimal primal solution, where I highlight that the optimal primal solution is static/fixed. Let's call it $\rho-\text{opt}$. But, in the proof, instead of comparing our performance with that of $\rho-\text{opt}$, we compare it with $\rho^*(t)$, which is dynamic benchmark. Two questions: why do we consider such a strong benchmark? Is it necessary? and if yes, why? the second question is that how can we manage to get a low regret w.r.t. such a strong dynamic benchmark? It seems to good to be true. Having a discussion on these two points seem necessary to me.  }
\begin{theorem}[Putting everything together]
\label{thm:regret}
Assume assumptions  \ref{ass:budgetbind} and \ref{ass:feas} hold. Let $(\rho_{j,t})_{j\in [M], t\in [T]}$ be the per-channel budgets generated from Algorithm \ref{alg:omducb} and assume we take step size $\eta = \Theta(1/\sqrt{T})$, discretization width $\discerr = \Theta(T^{-1/3}) $, and $\underline{\slope} = \Theta(T^{-1/3})$ in Lemma \ref{lem:ucbregret}. Then for large enough $T$ we have $ T\cdot  \textsc{GL-OPT} - \E\left[\sum_{t\in [T]}\sum_{j\in[M]}\totv_{j}(\rho_{j,t})\right] \leq \mathcal{O}(T^{2/3})$.
% \begin{align}
% \label{eq:finalregret}
%     T\cdot  \textsc{GL-OPT} - \E\left[\sum_{t\in [T]}\sum_{j\in[M]}\totv_{j}(\rho_{j,t})\right] \leq \mathcal{O}(T^{2/3}).
% \end{align}
Recalling $\overline{\bm{\rho}}_{T} = \left(\frac{1}{T}\sum_{t\in[T]} \rho_{j,t}\right)_{j\in [M]}$ is the vector of time-averaged per-channel budgets, this implies
\begin{align*}
    \textsc{GL-OPT} - \sum_{j \in [M]}\E\left[\totv_{j}(\overline{\rho}_{T,j})\right] \leq \mathcal{O}(T^{-1/3})\,,
\end{align*}
as well as approximate constraint satisfaction
\begin{align*}
     \sum_{j \in [M]}\E\left[\totv_{j}(\overline{\rho}_{T,j}) -\gamma \overline{\rho}_{T,j}\right] \geq -\mathcal{O}(T^{-1/2}),~\text{ and }\rho - \sum_{j \in [M]}\E[\overline{\rho}_{T,j}] \geq -\mathcal{O}(T^{-1/2})
\end{align*}
% $ \textsc{GL-OPT} - \sum_{j \in [M]}\E\left[\totv_{j}(\overline{\rho}_{T,j})\right] \leq \mathcal{O}(T^{-1/3})$, and further $ \sum_{j \in [M]}\E\left[\totv_{j}(\overline{\rho}_{T,j}) -\gamma \overline{\rho}_{T,j}\right] \geq -\mathcal{O}(T^{-1/2})$ and $\rho - \sum_{j \in [M]}\E[\overline{\rho}_{T,j}] \geq -\mathcal{O}(T^{-1/2})$. {\color{red} in words, say this means the constraint of the problem are satisfied in expectation. }
\end{theorem}

{\color{red} you can refer to numerical results where you study the impact of $T$ on the performance of the algorithm.}
Here, we note that the above approxamate constraint satisfaction is in expectation, similar to our definition of $\textsc{CH-OPT}(\mathcal{I}_{\budg})$
defined in Eq. \eqref{eq:chopt}. To conclude, we make an important remark that distinguishes our result in Theorem \ref{thm:regret} with related literature on convex optimization.
% \textit{Proof sketch.}
% Proposition \ref{prop:ubbenchlag} allows us to decompose total regret into two parts, namely the error induced by the UCB component in our algorithm, and the error due to deviations from complementary slackness:
% \begin{align}
% \begin{aligned}
%       & T\cdot  \textsc{GL-OPT} - \E\left[\sum_{t\in [T]}\sum_{j\in[M]}\totv_{j}(\rho_{j,t})\right] \\
%      ~\leq~& \sum_{j\in [M]}\underbrace{\sum_{t\in[T]} 
%      \E\left[\mathcal{L}_{j}(\rho_{j}^{*}(t), \lambda_{t}, \mu_{t})  - \mathcal{L}_{j}(\rho_{j,t}, \lambda_{t}, \mu_{t})\right]}_{\leq \mathcal{O}\left(\discerr T + \underline{\slope} T + \frac{1}{\underline{\slope}\discerr}\right)}+ \underbrace{\sum_{t\in[T]}\E\left[\lambda_{t}g_{1,t} + \mu_{t}g_{2,t}\right]}_{ \mathcal{O}\left( \eta  T + \frac{1}{\eta}\right)}
%       \end{aligned}
%  \end{align}
%  Here, the first bound follows from Lemma \ref{lem:ucbregret}, and the second bound follows from Lemma \ref{lem:boundcs}. By taking $\underline{\slope} = \discerr = T^{-1/3}$ and $\eta = 1/\sqrt{T}$, we can obtain Eq. \eqref{eq:finalregret}.  The conversion error for $\overline{\bm{\rho}}_{T}$, namely $\textsc{GL-OPT} - \sum_{j \in [M]}\totv_{j}(\overline{\rho}_{T,j}) \leq \mathcal{O}(T^{-1/3})$, follows directly from concavity of $\totv_{j}(\rho_{j})$ in $\rho_{j}$ for all $j\in [M]$ according to Lemma \ref{lem:Vstruct}. Constraint approxmations at $\overline{\bm{\rho}}_{T}$ follows from Lemma \ref{lem:approxconst} and again concavity of $\totv_{j}(\rho_{j})$.
 

\begin{remark}
\label{rmk:onepoint}
In light of Lemma \ref{lem:Vstruct}, the 
advertiser's optimization problem $\textsc{CH-OPT}(\mathcal{I}_{\budg})$ in Eq. \eqref{eq:chopt} effectively becomes a convex problem (see Proposition \ref{prop:convexprob} in Appendix \ref{app:onlineadd}). Hence it may be tempting for one to directly employ off-the-shelf convex optimization algorithms. However, our problem involves stochastic bandit feedback, and more importantly, \textit{uncertain constraints}, meaning that we cannot analytically determine whether a primal decision satisfies the constraints of the problem. For example, in $\textsc{CH-OPT}(\mathcal{I}_{\budg})$, for some primal decision $(\rho_{j})_{j\in[M]}$, we cannot determine whether the ROI constraint  $\sum_{j \in M} \E\left[\totv_{j}(\gamma_{j},\rho_{j};\bm{z}_{j}) - \gamma \totc_{j}(\gamma_{j},\rho_{j};\bm{z}_{j})\right]\geq 0$ holds because the distribution $(\bm{p}_{j})_{j\in[M]}$ from which $\bm{z}$ is sampled is unknown. To the best of our knowledge, there are only two recent works that handle a similar stochastic bandit feedback, and uncertain constraint setting, namely \cite{usmanova2019safe} and \cite{nguyen2022stochastic}. Nevertheless, our setting is more challenging because these works consider a ``two-point estimation'' regime where one can make function evaluations to the objective and constraints twice each period, whereas our setting involves ``one-point estimation'' such that we can only make function calls once per period. We note the optimal oracle complexities for unknown constraint convex optimization with one-point bandit feedback, remains an open problem.\footnote{See Table 4.1 in \cite{larson2019derivative} for best known  complexity bounds for one-point bandit feedback setups.}
\end{remark}



\subsection{Extension to strict constraint satisfaction: UCB-SGD-II}
In Theorem \ref{thm:regret}, we showed that the final output of the UCB-SGD Algorithm \ref{alg:omducb} outputs a per-channel budget profile $\overline{\bm{\rho}}_{T} = \left(\frac{1}{T}\sum_{t\in[T]} \rho_{j,t}\right)_{j\in [M]}$ that satisfies both ROI and budget constraints in $\textsc{CH-OPT}(\mathcal{I}_{\budg})$ approximately, i.e. there can be at most violations in the magnitude of $\mathcal{O}(T^{-1/2})$ for both constraints. In this subsection, we present a modification to UCB-SGD that enables us to achieve no-constraint violations, while still retaining the $\mathcal{O}(T^{-1/3})$ accuracy in total conversion. Similar modification techniques have been introduced in \cite{balseiro2022best,feng2022online}. 

Our modification strategy handles ROI and budget constraint satisfactions differently. For budget constraints, we simply maintain a spend balance $B_{t}$ in each period starting from $B_{1} = 0$, and increase the balance by the expenditure in each period. When the balance nears $\rho T$, i.e. total spend comes close to $\rho T$, we simply terminate the algorithm. Regarding the ROI constraint, we develop two phases. Phase 1 is a ``safety buffer phase'' where we conservatively set per-channel budgets to accumulate a positive ``ROI balance'', i.e. in this phase (assume ending in period $T_{1}$) we hope to achieve $\sum_{t\in [T_{1}]}g_{1,t} \geq \Theta(\sqrt{T})$, where we recall $-g_{1,t}$ defined in step 4 of Algorithm \ref{alg:omducb} can be viewed as the ROI constraint violations in period $t$. For phase 2, we then naively run SGD-UCB. The motivation for this two-phase design is that we aim to have a buffer, i.e. positive ROI balance, in phase 1 that can compensate for possible constraint violations in phase 2 when we run SGD-UCB (see Theorem \ref{thm:regret}). We call our algorithm SGD-UCB-II which we present in Algorithm \ref{alg:omducb2}.

We remark that in order to implement the buffer phase 1 to attain a positive ROI balance, we rely on the following Assumption \ref{ass:channelfeas} which is a strengthened version of Assumption \ref{ass:feas} that states in each channel there is always an auction that has a value-to-cost ratio above the global target ROI $\gamma$. Then by setting a small budget  we denote as $\beta$, the channel will only procure impressions with high value-to-cost ratios (due to the structure of conversion functions in Lemma \ref{lem:Vstruct}), and thus ensuring that the ROI balance increases.

\begin{algorithm}[ht]
    \centering
    \caption{SGD-UCB-II}\label{alg:omducb2}
    \footnotesize
    \begin{algorithmic}[1]
    \Require{Set spend balance $B_{1}=0$, and $g_{1,0} = 0$, $\beta > 0$} 
    \phase{Accumulate ROI balance buffer}
    \While{$\sum_{t' \in [t-1]}g_{1,t'} \leq \sqrt{T}\log(T)$}
    \If{$B_{t} + M\rho  > \rho T$}
         \State Terminate  algorithm and output $\overline{\bm{\rho}} = \left(\frac{1}{T}\sum_{t'\in[t]} \rho_{j,t'}\right)_{j\in [M]}$.
    \EndIf
    \State  Set per-channel budget to be $\beta$ for all channels.  Observe conversion $\totv_{j}(\beta;\bm{z}_{t})$ for all $j \in [M]$, and calculate
    \begin{align*}
        g_{1,t} = \sum_{j \in M} \left(\totv_{j}(\beta;\bm{z}_{t}) -  \gamma  \beta\right)\,.
    \end{align*}
    \State Calculate $B_{t+1} = B_{t} + M\beta$.
    \State Increment $t \leftarrow t+1$
	\EndWhile
 \State Denote end period of Phase 1 as $T_{1} = t-1$.
 \phase{Run SGD-UCB}
 \State For remaining $T - T_{1}$ periods, run SGD-UCB  in Algorithm \ref{alg:omducb} with a spend balance check during each period $t$:
 \If{$B_{t} + M\rho  > \rho T$}
 \State Terminate and output 
 $\overline{\bm{\rho}} = \left(\frac{1}{T}\sum_{t'\in[t]} \rho_{j,t'}\right)_{j\in [M]}$.
 \Else 
 \State Set per-channel budgets $\{\rho_{j,t}\}_{j\in[M]}$ according to SGD-UCB for all channels. 
 \State Update spend balance $B_{t+1} = B_{t} + \sum_{j\in [M]}\rho_{j,t}$.
 \EndIf
    \end{algorithmic}
\end{algorithm}


\begin{assumption}[Strictly feasible per-channel ROI constraints]
\label{ass:channelfeas}
Fix any channel $j\in [M]$ and any realization of value-cost pairs  $\bm{z}_{j} =(\bm{v}_{j},\bm{d}_{j}) \in F_{j}$, the channel's optimization problem in Eq. \ref{eq:budperchannelsol} is strictly feasible, i.e. the set $\left\{\bm{x}_{j} \in [0,1]^{m_{j}}: \bm{v}_{j}^{\top} \bm{x}_{j} > \gamma\bm{d}_{j}^{\top}\bm{x}_{j}\right\}$ is nonempty.\footnote{Equivalently, for any realization of value-cost pairs  $\bm{z}_{j} = (\bm{v}_{j},\bm{d}_{j})$ there always exists an auction $n\in [m_{j}]$ in this channel  whose value-to-cost ratio is at least $\gamma$, i.e. $v_{j,n} >  \gamma d_{j,n}$.}
\end{assumption}

Our strategy to bound the performance of SGD-UCB-II is as followed: In the first phase, we show that we acquire sufficient ROI balance buffers to compensate for global ROI constraint violation in the second phase. On the other hand, conversion loss in the second phase is solely due to SGD-UCB (Algorithm \ref{alg:omducb}), and thus our proof to bound such loss follows from similar ideas in Theorem \ref{thm:regret} (but here we have to additionally handle  ``early stopping'' of UCB-SGD-II due to the spend balance check.

Note that in the  first ROI balance buffer phase, we are not optimizing for per-channel budgets which may lead to significant per-period conversion loss. Nevertheless, in the following lemma, we first show that the first ROI balance buffer phase does not last too long; We refer readers to Appendix \ref{pf:lem:boundphase1} for the proof.
\begin{lemma}[Bounding length of Phase 1]
\label{lem:boundphase1}
Recall $T_{1}\in [T]$ is the end period of Phase 1 in the SGD-UCB-II algorithm (see step 10). Denote the event $\mathcal{E} = \{T_{1}\geq 2\sqrt{T}\log^{3}(T)\}$, and take small  budget $\beta = \frac{1}{\log(T)}$ in the SGD-UCB-II algorithm.  Then, under Assumption \ref{ass:feas}, for large enough $T$ we have $\prob\left(\mathcal{E}\right)\leq \frac{1}{T}$. 
\end{lemma}

Our main result in this subsection is the following Theorem \ref{thm:regret2} which bounds the conversion loss of SGD-UCB-II. The proof is detailed in Appendix \ref{pf:thm:regret2}.
\begin{theorem}
\label{thm:regret2} 
Suppose that Assumptions \ref{ass:budgetbind} and \ref{ass:channelfeas}  hold. Let $T_{2} \in [T]$ be the termination period of SGD-UCB-II (Algorithm \ref{alg:omducb2}), and recall
 $\overline{\bm{\rho}} = \left(\frac{1}{T}\sum_{t\in[T_{2}]}\rho_{j,t}\right)_{j\in [M]}$ are the final outputs of the algorithm. Further, we input $\beta =\frac{1}{
 \log(T)} $ to the algorithm that is used for Phase 1, and in Phase 2 where we run SGD-UCB, we use the same parameters as those in Theorem \ref{thm:regret}. Then,  for large enough $T$ we have 
    $ \textsc{GL-OPT} - \sum_{j \in [M]}\E\left[\totv_{j}(\overline{\rho}_{j})\right]\leq \mathcal{O}(T^{-1/3})$, and further $\sum_{j \in [M]}\E\left[\totv_{j}(\overline{\rho}_{j}) -\gamma \overline{\rho}_{j}\right]\geq 0 $ and $\sum_{j \in [M]} \E\left[\overline{\rho}_{j}\right]\leq \rho$. 
\end{theorem}


==> A3_onlineold.tex <==

% \subsection{Proof of Proposition \ref{prop:budgetbind}}
% \label{pf:prop:budgetbind}
% Fix any channel $j$ which consists of $m_{j}$ parallel auctions, and recall that we assumed the orderding
% $\frac{v_{j,1}}{d_{j,1}} > \frac{v_{j,2}}{d_{j,2}} > \dots  > \frac{v_{j,m_{j}}}{d_{j,m_{j}}}$ for any realization $\bm{z}_{j}$. Then, with the option where the per-channel ROI is set to 0 (i.e. omitted) $\totv_{j}(\rho_{j};\bm{z}_{j})$ is exactly the LP relaxation of a 0-1 knapsack, whose optimal solution  $\bm{x}_{j}^{*}(\rho_{j};\bm{z}_{j})$ is well known to be unique, and takes the form for any auction index $n\in [m_{j}]$:
% \begin{align}
% \label{eq:knapsack}
%     x_{j,n}^{*}(\rho_{j};\bm{z}_{j}) = \begin{cases}
%     1 & \text{if } \sum_{n' \in [n]} d_{j,n'} \leq \rho_{j}\\
%     \frac{\rho_{j} - \sum_{n' \in [n-1]} d_{j,n'}}{d_{j,n}} & \text{if } \sum_{n' \in [n]} d_{j,n'} > \rho_{j}\\
%     0 & \text{otherwise}
%     \end{cases}
% \end{align}

%  We prove the claim in the proposition using a contradiction argument. Assume for any $\rho_{j} < \rho$, the solution $\bm{x}_{j}^{*}(\rho_{j};\bm{z}_{j})$ is not budget binding, i.e. $\bm{d}_{j}^{\top} \bm{x}_{j}^{*}(\rho_{j};\bm{z}_{j}) < \rho_{j}$. This implies that the knapsack solution to Eq. \eqref{eq:knapsack} is $ x_{j,n}^{*}(\rho_{j};\bm{z}_{j})  = 1$ for all $n \in [m_{j}]$, or in other words $\sum_{n \in [m_{j}]} d_{j,n} < \rho_{j} < \rho$. However, this violates 
%  Assumption \ref{ass:budgetbind} because if we set channel $j$'s budget to be $\rho > \rho_{j}$, we cannot have the budget constraint to be binding. Therefore, $\bm{x}_{j}^{*}(\rho_{j};\bm{z}_{j})$ is  budget binding for any $\rho_{j} < \rho$.
% \halmos



\subsection{Proof of Proposition \ref{prop:ubbenchlag}}
\label{pf:prop:ubbenchlag}
Let $(\rho_{j}^{*})_{j\in[M]}$ be the optimal per-channel budgets to $ \textsc{CH-OPT}(\mathcal{I}_{\budg})$. Then
\begin{align}
\begin{aligned}
     & T\cdot \textsc{GL-OPT} - \E\left[\sum_{t\in [T]}\sum_{j\in[M]}\totv_{j}(\rho_{j,t})\right] \\
    ~\overset{(i)}{\leq}~ & M\Bar{V}K + (T-K)\cdot \textsc{CH-OPT}(\mathcal{I}_{\budg}) - \E\left[\sum_{t > K}\sum_{j\in[M]}\totv_{j}(\rho_{j,t})\right]\\
     ~\overset{(ii)}{=}~ & M\Bar{V}K + \rho\sum_{t > K}\E\left[\mu_{t}\right] + \sum_{t>K}\sum_{j\in [M]} \E\left[\mathcal{L}_{j}(\rho_{j}^{*}, \lambda_{t}, \mu_{t})\right] -  \sum_{t > K}\sum_{j\in [M]}\E\left[\mathcal{L}_{j}(\rho_{j,t}, \cont_{t}) - \lambda_{t}\left(\totv_{j}(\rho_{j,t}) - \gamma\rho_{j,t}\right) + \mu_{t}\rho_{j,t}\right]\\
      ~\overset{(iii)}{\leq}~ & M\Bar{V}K +  \sum_{j\in [M]} \sum_{t > K} 
     \E\left[\mathcal{L}_{j}(\rho_{j}^{*}(t), \cont_{t}) - \mathcal{L}_{j}(\rho_{j,t}, \cont_{t})\right] +  \sum_{t > K}\left(\lambda_{t}g_{1,t} + \mu_{t}g_{2,t}\right)\,.
    \end{aligned}
\end{align}
Here, (i) follows from Theorem \ref{thm:budgonlysuff} that states $\textsc{GL-OPT} =   \textsc{CH-OPT}(\mathcal{I}_{\budg})$; (ii) follows from the $ \textsc{CH-OPT}(\mathcal{I}_{\budg}) = \sum_{j\in[M]}\totv_{j}(\rho_{j}^{*})$ and the definition of the Lagrangian in Eq. \eqref{eq:Lagrangian};  
in (ii) we define $\rho_{j}^{*}(t) = \arg\max_{\rho_{j}\geq 0} \mathcal{L}_{j}(\rho_{j}, \cont_{t})$ to be the optimal budget that maximizes the Lagrangian w.r.t. the dual variables $\cont_{t}=(\lambda_{t},\mu_{t})$.
\halmos





\subsection{Proof of Lemma \ref{lem:Vstruct}}
\label{pf:lem:Vstruct}
We first show for any realization $\bm{z} = (\bm{z}_{j})_{j\in [M]} = (\bm{v}_{j},\bm{d}_{j})_{j\in [M]} $, the conversion function $\totv_{j}(\rho_{j};\bm{z}_{j})$
is piecewise linear, strictly increasing, and concave for any $j \in [M]$. 

Fix any channel $j$ which consists of $m_{j}$ parallel auctions, and recall that we assumed the orderding
$\frac{v_{j,1}}{d_{j,1}} > \frac{v_{j,2}}{d_{j,2}} > \dots  > \frac{v_{j,m_{j}}}{d_{j,m_{j}}}$ for any realization $\bm{z}_{j}$. Then, with the option where the per-channel ROI is set to 0 (i.e. omitted) $\totv_{j}(\rho_{j};\bm{z}_{j})$ is exactly the LP relaxation of a 0-1 knapsack, whose optimal solution  $\bm{x}_{j}^{*}(\rho_{j};\bm{z}_{j})$ is well known to be unique, and takes the form for any auction index $n\in [m_{j}]$:
\begin{align}
\label{eq:knapsack}
    x_{j,n}^{*}(\rho_{j};\bm{z}_{j}) = \begin{cases}
    1 & \text{if } \sum_{n' \in [n]} d_{j,n'} \leq \rho_{j}\\
    \frac{\rho_{j} - \sum_{n' \in [n-1]} d_{j,n'}}{d_{j,n}} & \text{if } \sum_{n' \in [n]} d_{j,n'} > \rho_{j}\\
    0 & \text{otherwise}
    \end{cases}
\end{align}
where we denote $d_{j,0} =0$. With this form, it is easy to see
\begin{align}
\label{eq:pieceline}
   \totv_{j}(\rho_{j};\bm{z}_{j}) = \bm{v}_{j}^{\top} \bm{x}_{j}^{*}(\rho_{j};\bm{z}_{j})=  \sum_{n \in [m_{j}]}\left(\frac{v_{j,n}}{d_{j,n}}\rho_{j}+ \widetilde{b}_{j,n}\right)\I\left\{d_{j,0}+ \dots +d_{j,n-1}\leq \rho_{j}\leq d_{j,0}+ \dots +d_{j,n} \right\}
   \end{align}
where we denote $d_{j,0} =0$ and also $\widetilde{b}_{j,n} = \sum_{n' \in [n-1]} v_{j,n'} - \frac{v_{j,n}}{d_{j,n}}\cdot \left(\sum_{n' \in [n-1]} d_{j,n'}\right)$ and $ v_{j,0} = 0$. It is easy to check that any two line segments, say $[X_{n-1},X_{n}]$ and $[X_{n},X_{n+1}]$ where we write $X_{n} =  d_{j,0}+ \dots +d_{j,n} $, intersect at $\rho_{j} =X_{n}$, because $\frac{v_{j,n}}{d_{j,n}}\rho_{j}+ \widetilde{b}_{j,n} = \frac{v_{j,n+1}}{d_{j,n+1}}\rho_{j}+ \widetilde{b}_{j,n+1}$
at $\rho_{j} =X_{n}$. Hence, from Eq. \eqref{eq:pieceline} we can conclude $ \totv_{j}(\rho_{j};\bm{z}_{j})$ is continuous, which further implies it is piecewise linear and strictly increasing. Further, the ordering
$\frac{v_{j,1}}{d_{j,1}} > \frac{v_{j,2}}{d_{j,2}} > \dots  > \frac{v_{j,m_{j}}}{d_{j,m_{j}}}$ implies that the slopes on each segment $[X_{n},X_{n+1}]$ decreases as $n$ increases, which implies  $ \totv_{j}(\rho_{j};\bm{z}_{j})$  is concave.

Since $\totv_{j}(\rho_{j})= \E\left[\totv_{j}(\rho_{j};\bm{z}_{j})\right]$, where the expectation is taken w.r.t. randomness in $\bm{z}_{j}$, and since the $\bm{z}_{j}$ is sampled from some discrete distribution $\bm{p}_{j}$ on finite support $F_{j}$, $\totv_{j}(\rho_{j})$ is simply a weighted average over all $\left(\totv_{j}(\rho_{j};\bm{z}_{j})\right)_{\bm{z}_{j} \in F_{j}}$ with weights in $\bm{p}_{j}$, so $\totv_{j}(\rho_{j})$ is also continuous, piecewise linear, strictly increasing, and concave, and thus can be written as Eq. \eqref{eq:Vstruct} with parameters $\{(s_{j,n},b_{j,n},r_{j,n})\}_{n\in [S_{j}]}$ that only depend on the support $F_{j}$ and distribution $\bm{p}_{j}$. 

Finally, according to the definition of $\mathcal{L}_{j}(\rho_{j},\cont)= \E\left[\mathcal{L}_{j}(\rho_{j},\cont;\bm{z}_{j})\right]$ and $  \mathcal{L}_{j}(\rho_{j}, \cont; \bm{z}_{j}) =  (1+\lambda)\totv_{j}(\rho_{j};\bm{z}_{j}) - (\lambda \gamma  + \mu) \rho_{j} $
as defined in Eq. \eqref{eq:Lagrangian}, we have
\begin{align}
\label{eq:Elagr}
    \mathcal{L}_{j}(\rho_{j},\cont) = (1+\lambda)\totv_{j}(\rho_{j}) - (\lambda \gamma  + \mu) \rho_{j}
\end{align}
which implies $ \mathcal{L}_{j}(\rho_{j},\cont)$ is continuous, piecewise linear, and concave because $\totv_{j}(\rho_{j})$ is continuous, piecewise linear, and concave as shown above. Combining Eq. \eqref{eq:Elagr} and the representation of $\totv_{j}(\rho_{j})$ in Eq. \eqref{eq:Vstruct}, we have
\begin{align}
        \mathcal{L}_{j}(\rho_{j}, \cont) =  \sum_{n\in [S_{j}]} \left( \slope_{j,n}(\cont) \rho_{j} + (1+\lambda)b_{j,n}\right)\I\{r_{j,n-1}\leq \rho_{j} \leq r_{j,n}\}\,.
\end{align}
where the slope $\slope_{j,n}(\cont) = (1+\lambda) s{j,n} -(\mu + \gamma \lambda)$ decreases in $n$. Thus at the point $r_{j,n^{*}} = \max\{r_{j,n}:n=0,1\dots, S_{j}~,\slope_{j,n}(\cont) \geq 0\}$ in which the slope to the right turns negative for the first time, $ \mathcal{L}_{j}(\rho_{j}, \cont) $ takes its maximum value
$\max_{\rho_{j}\geq 0} \mathcal{L}_{j}(\rho_{j}, \cont)$, because to the left of  $r_{j,n^{*}}$, namely the region
$[0,r_{j,n^{*}}]$, $\mathcal{L}_{j}(\rho_{j}, \cont) $ strictly increases because slopes are positive; and to the right of  $r_{j,n^{*}}$, namely the region $[r_{j,n^{*}},\rho]$, $\mathcal{L}_{j}(\rho_{j}, \cont) $ strictly decreases because slopes are negative.
\halmos 






\subsection{Proof for Lemma \ref{lem:dualvarub}}
\label{pf:lem:dualvarub}


We first present some definitions for convenience: denote $\cont = (\lambda, \mu)$, $\cont_{t} = (\lambda_{t}, \mu_{t})$, and $\bm{z}_{t} = (\bm{v}_{t},\bm{d}_{t})$. For any realization $\bm{z} = (\bm{v},\bm{d}) = (\bm{v}_{j},\bm{d}_{j})_{j\in[M]} \in F_{1}\times \dots F_{M}$ of values and costs across channels, define the dual function 
\begin{align}
\label{eq:dualfunc}
\begin{aligned}
    \mathcal{L}_{d}(\cont;\bm{z}) ~=~& \max_{\bm{\rho}\in [0,\rho]^{M}} \sum_{j\in[M]}\totv_{j}(\rho_{j};\bm{z}) + 
\lambda \sum_{j\in [M]}\left(\totv_{j}(\rho_{j};\bm{z}) - \gamma \rho_{j}\right) + \mu\left(\rho - \sum_{j\in [M]}\rho_{j}\right)\\
~=~& \mu \rho + \max_{\bm{\rho}\in [0,\rho]^{M}}\mathcal{L}(\bm{\rho},\cont;\bm{z})\,.
\end{aligned}
\end{align}
From standard convex analysis we know that $ \mathcal{L}_{d}$ is convex in $(\lambda,\mu)$, which implies for any $\cont' = (\lambda',\mu')$
\begin{align}
\label{eq:convex}
    (\cont' -\cont)^{\top} \nabla  \mathcal{L}_{d}(\cont;\bm{z}) \leq \mathcal{L}_{d}(\cont';\bm{z})-\mathcal{L}_{d}(\cont;\bm{z})
\end{align}


We prove the lemma by induction that 
\begin{align}
    \lambda_{t},\mu_{t} \leq \dualub_{F} := 1 + \frac{\max_{\bm{z}\in F_{1}\times \dots F_{M}}\bm{e}^{\top}\bm{v} + 1}{\min_{\bm{z}\in F_{1}\times \dots F_{M}}\left\{\sum_{j\in [M]}\left(\totv_{j}(\rho_{(\bm{z}),j};\bm{z}) - \gamma \rho_{j}\right), \rho - \sum_{j\in [M]}\rho_{(\bm{z}),j} \right\}} 
\end{align}
Here, in Proposition \ref{prop:slater} we defined $\bm{\rho}_{(\bm{z})}$ for any  $\bm{z}$ such that Slater's condition holds, i.e. $\sum_{j\in [M]}\left(\totv_{j}(\rho_{(\bm{z}),j};\bm{z}) - \gamma \rho_{j}\right) > 0$ and 
$\rho - \sum_{j\in [M]}\rho_{(\bm{z}),j}  > 0$. 

The base case for $t = 1$ is satisfied trivially since we take $\bm{\cont}_{t} = 0$. Now assume $\norm{\cont_{t}}\leq \dualub_{F}$, and we will show $\norm{\cont_{t+1}}\leq \dualub_{F}$ by considering two different case:


\textbf{Case (A):} If $\mathcal{L}_{d}(\bm{c}_{t};\bm{z}_{t}) > \mathcal{L}_{d}(\bm{0};\bm{z}_{t}) + \eta M^{2}\Bar{\totv}^{2}$.

Define $\bm{g}_{t} = (g_{1,t},g_{2,t})$ where we recall $g_{1,t} = \sum_{j\in [M]}\left(\totv_{j,t}(\rho_{j,t}) - \gamma \rho_{j,t}\right)$ and $g_{2,t} = \rho - \sum_{j\in [M]}\rho_{j,t}$. 
From Eq. \eqref{eq:omdtelescope} in the proof of Lemma \ref{lem:omdtelescope}, we have for any $\lambda\geq 0$ and $\mu\geq 0$,
\begin{align*}
\begin{aligned}
    & (\lambda- \lambda_{t+1})^{2} ~\leq~
  (\lambda- \lambda_{t})^{2} + 2\eta\left(\lambda-\lambda_{t}\right) g_{1,t} + \eta^{2} M^{2}\Bar{\totv}^{2}\\
  & (\mu- \mu_{t+1})^{2} ~\leq~
  (\mu- \mu_{t})^{2} + 2\eta\left(\mu-\mu_{t}\right) g_{1,t} + \eta^{2} M^{2}\Bar{\totv}^{2}\,.
  \end{aligned}  
\end{align*}
By summing the two inequalities and taking $\lambda = \mu = 0$ we get
\begin{align}
\label{eq:dualvarubtelescope}
\begin{aligned}
\norm{\cont_{t+1}}^{2} ~\leq~& \norm{\cont_{t}}^{2} +  2\eta\left(\cont_{t} \right)^{\top} \bm{g}_{t}  +  2\eta^{2}M^{2}\Bar{\totv}^{2}\\
~\overset{(i)}{\leq}~ & \norm{ \cont_{t}}^{2} +  2\eta\left(\mathcal{L}_{d}(\bm{0};\bm{z}_{t})-\mathcal{L}_{d}(\bm{c}_{t};\bm{z}_{t})\right)+  2\eta^{2} M^{2}\Bar{\totv}^{2}& 
\,,
\end{aligned}
\end{align}
where in (i) we applied Eq. \eqref{eq:convex} with $\bm{z} =\bm{z}_{t}$ and used the fact that $\bm{g}_{t} = (g_{1,t},g_{r,t})= \nabla \mathcal{L}_{d}(\bm{c}_{t};\bm{z}_{t})$.

Then from Eq. \eqref{eq:dualvarubtelescope} and the assumption $\mathcal{L}_{d}(\bm{c}_{t};\bm{z}_{t}) > \mathcal{L}_{d}(\bm{0};\bm{z}_{t}) + \eta M^{2}\Bar{\totv}^{2}$  we have
\begin{align*}
    \max\{\lambda_{t},\mu_{t}\}\leq \norm{\cont_{t+1}} < \norm{\cont_{t}}\leq \dualub_{F}
\end{align*}
where the final inequality follows from the induction hypothesis.


\textbf{Case (B):}  If $\mathcal{L}_{d}(\bm{c}_{t};\bm{z}_{t}) \leq \mathcal{L}_{d}(\bm{0};\bm{z}_{t}) + \eta M^{2}\Bar{\totv}^{2}$, then 
\begin{align}
\label{eq:bounddualvar0}
\begin{aligned}
 & \mathcal{L}_{d}(\bm{0};\bm{z}_{t}) + \eta M^{2}\Bar{\totv}^{2} \\
 ~\geq~ &\mathcal{L}_{d}(\bm{c}_{t};\bm{z}_{t}) \\
 ~\overset{(i)}{=}~& 
\mu_{t} \rho + \max_{\bm{\rho}\in [0,\rho]^{M}}\mathcal{L}(\bm{\rho},\cont_{t};\bm{z}_{t})\\
~\overset{(ii)}{\geq}~& 
\mu_{t} \rho + \mathcal{L}(\bm{\rho}_{(\bm{z}_{t})},\cont_{t};\bm{z}_{t})\\
~=~& \sum_{j\in[M]}\totv_{j}(\rho_{(\bm{z}_{t}),j};\bm{z}_{t}) + 
\lambda_{t} \sum_{j\in [M]}\left(\totv_{j}(\rho_{(\bm{z}_{t}),j};\bm{z}_{t}) - \gamma \rho_{j}\right) + \mu_{t}\left(\rho - \sum_{j\in [M]}\rho_{(\bm{z}_{t}),j}\right)\\
~\geq~& \lambda_{t} \sum_{j\in [M]}\left(\totv_{j}(\rho_{(\bm{z}_{t}),j};\bm{z}_{t}) - \gamma \rho_{j}\right) + \mu_{t}\left(\rho - \sum_{j\in [M]}\rho_{(\bm{z}_{t}),j}\right)\\
~\overset{(iii)}{\geq}~& \left(\lambda_{t} +\mu_{t} \right)
\cdot \min_{\bm{z}\in F_{1}\times \dots F_{M}}\left\{\sum_{j\in [M]}\left(\totv_{j}(\rho_{(\bm{z}),j};\bm{z}) - \gamma \rho_{j}\right), \rho - \sum_{j\in [M]}\rho_{(\bm{z}),j} \right\}\,.
\end{aligned}
\end{align}
Here, (i) follows from the definition  of the dual function in Eq. \eqref{eq:dualfunc}; in (ii) we recall the definition of $\bm{\rho}_{(\bm{z})}$ that satisfies the Slater's condition in Lemma \ref{prop:slater}; in (iii), we used the fact that $\lambda_{t},\mu_{t}\geq 0$ and also under Slater's condition we have for any $\bm{z}$, $\sum_{j\in [M]}\left(\totv_{j}(\rho_{(\bm{z}),j};\bm{z}) - \gamma \rho_{j}\right) > 0$ and 
$\rho - \sum_{j\in [M]}\rho_{(\bm{z}),j}  > 0$. 


On the other hand, we have $\eta M^{2}\bar{\totv}^{2} < 1$ and also $\mathcal{L}_{d}(\bm{0};\bm{z}_{t}) = \max_{\bm{\rho}\in [0,\rho]^{M}}\sum_{j\in [M]}\totv_{j}(\rho_{j};\bm{z}_{t}) =\max_{\bm{z}\in F_{1}\times \dots F_{M}}\bm{e}^{\top}\bm{v}$. Hence combining this with Eq. \eqref{eq:bounddualvar0} we get 
\begin{align}
    \lambda_{t} +\mu_{t} < \frac{\max_{\bm{z}\in F_{1}\times \dots F_{M}}\bm{e}^{\top}\bm{v} + 1}{\min_{\bm{z}\in F_{1}\times \dots F_{M}}\left\{\sum_{j\in [M]}\left(\totv_{j}(\rho_{(\bm{z}),j};\bm{z}) - \gamma \rho_{j}\right), \rho - \sum_{j\in [M]}\rho_{(\bm{z}),j} \right\}} := \dualub_{F} - 1
\end{align}
which further implies $ \lambda_{t},\mu_{t}\leq \dualub_{F} - 1$. Hence, we can finally conclude
\begin{align}
    \lambda_{t+1} = \left(\lambda_{t} - \eta g_{1,t} \right)_{+} \leq \lambda_{t} + \eta |g_{1,t}|\leq \norm{\cont_{t}} - 1 + \eta M\bar{\totv} < \dualub_{F} 
\end{align}
where in the final inequality we used the fact that $\eta M \bar{\totv} < 1$. A similar bound holds for $\mu_{t+1}$.
\halmos





\subsection{Proof for Lemma \ref{lem:ucbregret}}
\label{pf:lem:ucbregret}

For simplicity, for any context $\cont$, assuming the optimal budget $\arg\max_{\rho_{j}\in[0,\rho]} \mathcal{L}_{j}(\rho_{j},\cont)$ is located at the $n$th ``turning point'' $r_{j,n}$ we have
\begin{align}
\label{eq:adj2}
\begin{aligned}
    & \slope_{j}^{-}(\cont) = \slope_{j,n}(\cont) 
    ~\text{ and }~ \slope_{j}^{+}(\cont) = \slope_{j,n}(\cont) \\
    & \adj_{j}^{-}(\cont) = [r_{j,n-1},r_{j,n}]    ~\text{ and }~ \adj_{j}^{+}(\cont) = [r_{j,n},r_{j,n+1}]  \,.
  \end{aligned}  
\end{align}
Further, define the following 
\begin{align}
\label{eq:UCBdefs}
\begin{aligned}
    &  \Delta_{k}(\cont) =  \max_{\rho_{j}\in [0,\rho]}\mathcal{L}_{j}(\rho_{j}, \cont) -  \mathcal{L}_{j}(a_{k}, \cont) \\
    & \contset(\underline{\slope}) = \left\{\cont \in \{\cont_{t}\}_{t\in [T]}: \slope_{j}^{-}(\cont) > \underline{\slope},~ |\slope_{j}^{+}(\cont)| > \underline{\slope}\right\} \text{ for } n = 0 \dots S_{j} \\
    & \contset_{n} = \Big\{\cont \in \{\cont_{t}\}_{t\in [T]}: r_{j,n} = \arg\max_{\rho_{j}\geq 0} \mathcal{L}_{j}(\rho_{j},\cont)\Big\} \text{ for } n = 0 \dots S_{j} \\
    & m_{k}(\cont) = \frac{8\log(T)}{\Delta_{k}^{2}(\cont)} \text{ for } \forall (k,\cont) \text{ s.t. }\Delta_{k}(\cont) > 0 \,.
    \end{aligned}
\end{align}
where $S_{j}$ and $\{r_{j,n}\}_{j\in [S_{j}]}$ are defined in Lemma \ref{lem:Vstruct}. The set $\contset_{k,n} $ represents all context $\cont_{t}$ under which the optimal $\arg\max_{\rho_{j}\geq 0} \mathcal{L}_{j}(\rho_{j},\cont_{t})$ is taken at the $n$th ``turning point'' $r_{j,n}$ of $\mathcal{L}_{j}(\rho_{j},\cont_{t})$ which is piecewiese linear in $\rho_{j}$ and also the two slopes adjacent to 
$r_{j,n}$, namely $\slope_{j,n}(\cont)$ and $\slope_{j,n+1}(\cont)$ satisfy $\slope_{j,n}(\cont) > \underline{\slope}$ and $|\slope_{j,n+1}(\cont)| > \underline{\slope}$. Further it is easy to see that $\contset = \cup_{n=0}^{S_{j}}\contset_{n}$.

Further, define $N_{k,t} = \sum_{\tau\leq t-1}\I\{\rho_{j,\tau} = a_{k}\}$ to be the number of times arm $k$ is pulled up to time $t$. we get
\begin{align}
\begin{aligned}
    &  \sum_{ t \in [T]}\mathcal{L}_{j}(\rho_{j,t}^{*}, \cont_{t}) - \mathcal{L}_{j}(\rho_{j,t}, \cont_{t}) = X_{1}+X_{2} + X_{3} \quad \text{ where }\\
    & X_{1} = \sum_{t\in[T]:\cont_{t} \notin \contset(\underline{\slope})}  \sum_{k\in [K]} \Delta_{k}(\cont_{t}) \I\{\rho_{j,t} = a_{k}, N_{k,t} \leq m_{k}(\cont_{t})\}\\
    & X_{2} = \sum_{t\in[T]:\cont_{t} \in \contset}   \sum_{k\in [K]}\Delta_{k}(\cont_{t}) \I\{\rho_{j,t} = a_{k}, N_{k,t} \leq m_{k}(\cont_{t})\}\\
    & X_{3} = \sum_{k\in [K]}\sum_{ t \in [T]} \Delta_{k}(\cont_{t}) \I\{\rho_{j,t} = a_{k}, N_{k,t} > m_{k}(\cont_{t})\}
    \end{aligned}
\end{align}
In Section \ref{subsubsec:X1}, we show that $X_{1} \leq \mathcal{O}(\discerr T + \underline{\slope}T + \frac{1}{\discerr})$; in Section \ref{subsubsec:X2}  we show that $X_{2} \leq \mathcal{O}(\discerr T + \frac{1}{\discerr \underline{\slope}})$;
 in Section \ref{subsubsec:X3}  we show that $X_{3} \leq \mathcal{O}(1)$.

\subsubsection{Bounding $X_{1}$.}
\label{subsubsec:X1}
At each context $\cont_{t} \notin \contset(\underline{\slope})$, we separate the set of arms $[K]$ into two groups, namely arms that lie at the left and right adjacent edges of optimal, namely $a_{k}\in \adj_{j}^{-}(\cont_{t}) \cup  \adj_{j}^{+}(\cont_{t})$ and all other arms (recall the sets $\adj_{j}^{-}$ and $\adj_{j}^{+}$ are defined in Eq. \eqref{eq:adj2}).

(1) For arm $k$ such that $a_{k} \in \adj_{j}^{-}(\cont_{t})$, recall Lemma \ref{lem:Vstruct} that $\mathcal{L}_{j}(a,\cont_{t})$ is linear in $a$ for $a \in \adj_{j}^{-}(\cont_{t})$, so $\Delta_{k}(\cont_{t}) = \slope_{j}^{-}(\cont_{t})\cdot (\rho_{j,t}^{*} - a_{k}) \leq \underline{\slope} (r_{j,n} - r_{j,n}) \leq  \underline{\slope} \rho$, so summing over all such $k$  we get 
\begin{align}
\label{eq:X1near}
\begin{aligned}
   &  \sum_{t\in[T]:\cont_{t} \notin \contset(\underline{\slope})}  ~\sum_{k\in[K]:a_{k} \in \adj_{j}^{-}(\cont_{t})}  \Delta_{k}(\cont_{t}) \I\{\rho_{j,t} = a_{k}, N_{k,t} \leq m_{k}(\cont_{t})\} \\
   ~\leq~& \sum_{t\in[T]:\cont_{t} \notin \contset(\underline{\slope})}   ~\sum_{k\in[K]:a_{k} \in \adj_{j}^{-}(\cont_{t})}  \underline{\slope} \rho \cdot  \I\{\rho_{j,t} = a_{k}, N_{k,t} \leq m_{k}(\cont_{t})\}  ~\leq~ \underline{\slope} \rho T = \mathcal{O}(\underline{\slope}T )\,.
   \end{aligned}
\end{align}

(2) For arm $k$ such that $a_{k} < \min \adj_{j}^{-}(\cont_{t})$, we further split contexts into groups $\contset_{n}$ for $n = 0 \dots S_{j}$ (defined in Eq. \eqref{eq:UCBdefs}) based on whether the corresponding optimal budget w.r.t. the Lagrangian at the context is taken at the $n$th ``turning point'' (see Figure \ref{fig:lagr} of illustration). Then, for each context group $n$ by defining  $k':=\max\{k: a_{k} < r_{j,n-1}\}$ to be the arm closest to and less than $r_{j,n-1}$, we have
\begin{align}
\label{eq:nbadslope}
\begin{aligned}
   & \sum_{t\in[T]:\cont_{t} \in \contset_{n}/\contset(\underline{\slope})} ~ \sum_{k\in[K]:a_{k} < \min \adj_{j}^{-}(\cont_{t})} ~  \Delta_{k}(\cont_{t}) \I\{\rho_{j,t} = a_{k}, N_{k,t} \leq m_{k}(\cont_{t})\} \\
    ~\overset{(i)}{=}~ & \sum_{t\in[T]:\cont_{t} \in \contset_{n}/\contset(\underline{\slope})} ~ \sum_{k\in[K]:a_{k} < r_{j,n-1}} ~  \Delta_{k}(\cont_{t}) \I\{\rho_{j,t} = a_{k}, N_{k,t} \leq m_{k}(\cont_{t})\} \\
    ~=~ &  \sum_{t\in[T]} \sum_{\cont \in \contset_{n}/\contset(\underline{\slope})} ~ \sum_{k\in[K]:a_{k} < r_{j,n-1}} \Delta_{k}(\cont) \I\{\cont_{t} = \cont, \rho_{j,t} = a_{k}, N_{k,t} \leq m_{k}(\cont)\}\\
    ~\overset{(ii)}{\leq}~ &  \sum_{t\in[T]} \sum_{\cont \in \contset_{n}/\contset(\underline{\slope})} ~ \left(\Delta_{k'}(\cont) \I\{\cont_{t}=\cont\} + \sum_{k\in[K]:a_{k} < r_{j,n-1}-\discerr} \Delta_{k}(\cont) \I\{\cont_{t} = \cont, \rho_{j,t} = a_{k}, N_{k,t} \leq m_{k}(\cont)\}\right)\\
   ~\overset{(iii)}{\leq}~ & \left((1+\dualub_{F})s_{j,n-1} \discerr + \rho \underline{\slope}\right) T + \sum_{k\in[K]:a_{k} < r_{j,n-1}-\discerr} ~ \sum_{\cont \in \contset_{n}/\contset(\underline{\slope})} \Delta_{k}(\cont) Y_{k}(\cont)
\end{aligned}
\end{align}
where in the final equality we defined $ Y_{k}(\cont)=  \sum_{t\in [T]} \I\{\cont_{t} = \cont, \rho_{j,t} = a_{k}, N_{k,t} \leq m_{k}(\cont)\}$. In (i) we used the fact that the left end of the left adjacent region, i.e. $
\min \adj_{j}^{-}(\cont_{t})$ is exactly $r_{j,n-1}$ because for context $\cont_{t} \in \contset_{n}$ the optimal budget $\arg\max_{\rho_{j}\in[0,\rho]} \mathcal{L}_{j}(\rho_{j},\cont_{t})$ is at the $n$th turning point; in (ii) we used the definition $k':=\max\{k: a_{k} < r_{j,n-1}\}$; (iii) follows the fact that under a context $\cont \in \contset_{n}/\contset(\underline{\slope})$,  we have $\arg\max_{\rho_{j}\in [0,\rho]} \mathcal{L}_{j}(\rho_{j}, \cont) = r_{j,n}$ so
\begin{align*}
    \Delta_{k'}(\cont) ~=~& \mathcal{L}_{j}(r_{j,n},\cont) -   \mathcal{L}_{j}(r_{j,n-1},\cont) + \mathcal{L}_{j}(r_{j,n-1},\cont) - \mathcal{L}_{j}(a_{k'},\cont)\\
     ~=~&  \slope_{j}^{-}(\cont) (r_{j,n} - r_{j,n-1}) + \slope_{j,n-1}(\cont)(r_{j,n-1} - a_{k'}) \\
     ~\overset{(iv)}{\leq}~ & \underline{\slope}\rho + \slope_{j,n-1}(\cont) \discerr\\
       ~\overset{(v)}{\leq}~ & \underline{\slope}\rho + (1+\dualub_{F})s_{j,n-1}\discerr
     \,,
\end{align*}
where in (iv) we used the fact that $\cont \in \contset_{n}/\contset(\underline{\slope})$ so $ \slope_{j}^{-}(\cont) \leq \underline{\slope}$, as well as $k'$ lies on the line segment between points $r_{j,n-2}$ and $r_{j,n-1}$ since $\discerr < \min_{n' \in [S_{j}]} r_{j,n'} - r_{j,n'-1}$; in (v) we recall $\slope_{j,n-1}(\cont) = (1+\lambda)s_{j,n-1} - (\mu + \gamma\lambda) \leq (1+\dualub_{F})s_{j,n-1}$ where $\dualub_{F}$ is defined in Lemma \ref{lem:dualvarub}.

We now bound $\sum_{\cont \in \contset_{n}/\contset(\underline{\slope})} \Delta_{k}(\cont) Y_{k}(\cont)$ in Eq. \eqref{eq:nbadslope}.  It is easy to see the following inequality for any sequence of context $\cont_{(1)}, \dots , \cont_{(\ell)} \in \{\cont_{t}\}_{t\in[T]}$:
\begin{align}
\label{eq:numbadarms}
    Y_{k}(\cont_{(1)}) + \dots +  Y_{k}(\cont_{(\ell)}) \leq \max_{\ell'=1\dots \ell} m_{k}(\cont_{(\ell')})\,. 
\end{align}
This is because 
\begin{align*}
   \sum_{\ell'\in [\ell]}  Y_{k}(\cont_{(\ell')}) ~=~ &\sum_{t\in[T]} \sum_{\ell'\in [\ell]}  \I\{\cont_{t} =\cont_{(\ell')}, \rho_{j,t} = a_{k}, N_{k,t} \leq m_{k}(\cont_{(\ell')})\}\\
     ~\leq~& \sum_{t\in[T]}  \sum_{\ell'\in [\ell]}  \I\{\cont_{t}= \cont_{(\ell')}, \rho_{j,t} = a_{k}, N_{k,t} \leq \max_{\ell'=1\dots \ell} m_{k}(\cont_{(\ell')})\}\\
      ~=~& \sum_{t\in[T]} \I\{\cont_{t} \in \{\cont_{(\ell')}\}_{\ell'\in[\ell]}, \rho_{j,t} = a_{k}, N_{k,t} \leq \max_{\ell'=1\dots \ell} m_{k}(\cont_{(\ell')})\}\\
        ~\leq~& \max_{\ell'=1\dots \ell} m_{k}(\cont_{(\ell')})\,.
\end{align*}
For simplicity denote $L = |\contset_{n}/\contset(\underline{\slope})|$, and order contexts in $\cont \in \contset_{n}/\contset(\underline{\slope})$ as $\{\cont_{(\ell)}\}_{\ell \in [L]}$ s.t. 
$\Delta_{k}(\cont_{(1)}) > \Delta_{k}(\cont_{(2)}) > \dots >\Delta_{k}(\cont_{(L)})$, or equivalently 
$m_{k}(\cont_{(1)}) < m_{k}(\cont_{(2)}) < \dots  < m_{k}(\cont_{(L)})$ according to Eq.\eqref{eq:UCBdefs}. Then multiplying Eq. \eqref{eq:numbadarms} by 
by $\Delta_{k}(\cont_{(\ell)}) - \Delta_{k}(\cont_{(\ell+1)})$ (which is strictly positive due to the ordering of contexts), and summing $\ell = 1 \dots L$  we get 
\begin{align}
\begin{aligned}
\label{eq:slope}
    &\sum_{\cont \in \contset_{n}/\contset(\underline{\slope})} \Delta_{k}(\cont) Y_{k}(\cont) = \sum_{\ell \in [L]} \Delta_{k}(\cont_{(\ell)}) Y_{k}(\cont_{(\ell)})\\
    ~\leq~&  \sum_{\ell \in [L]} m_{k}(\cont_{(\ell)}) \left( \Delta_{k}(\cont_{(\ell)}) -  \Delta_{k}(\cont_{(\ell+1)})\right)\\
    ~\overset{(i)}{=}~& 8\log(T)\sum_{\ell \in [L-1]} \frac{ \Delta_{k}(\cont_{(\ell)}) -  \Delta_{k}(\cont_{(\ell+1)})}{\Delta_{k}^{2}(\cont_{(\ell)})}\\
    ~\overset{(ii)}{\leq}~& 8\log(T) \int_{z = \Delta_{k}(\cont_{(L)})}\frac{dz}{z^{2}}\\
     ~=~& \frac{8\log(T)}{\Delta_{k}(\cont_{(L)})} ~\overset{(iii)}{=} \frac{8\log(T)}{\min_{\cont \in \contset_{n}/\contset(\underline{\slope})} \Delta_{k}(\cont)}\,.
     \end{aligned}
\end{align}
Here  (i) follows from the definition in Eq. \eqref{eq:UCBdefs} where we defined $m_{k}(\cont) = \frac{8\log(T)}{\Delta_{k}^{2}(\cont)}$; both (ii) and (iii) follow from the ordering of contexts so that $\Delta_{k}(\cont_{(1)}) > \Delta_{k}(\cont_{(2)}) > \dots >\Delta_{k}(\cont_{(L)})$. 
% Now combining Eq. \eqref{eq:slope} and \eqref{eq:nbadslope} we get 
% \begin{align}
% \label{eq:slope1}
%    \sum_{t\in[T]:\cont_{t} \in \contset_{n}/\contset(\underline{\slope})} ~ \sum_{k\in[K]:a_{k} < \min \adj_{j}^{-}(\cont_{t})} ~  \Delta_{k}(\cont_{t}) \I\{\rho_{j,t} = a_{k}, N_{k,t} \leq m_{k}(\cont_{t})\}  ~\leq~ \sum_{k\in[K]:a_{k} < r_{j,n-1}} \frac{8\log(T)}{\min_{\cont \in \contset_{n}/\contset(\underline{\slope})} \Delta_{k}(\cont)}
% \end{align}
Note that for any $\cont \in \contset_{n}/\contset(\underline{\slope})$ and arm $k$ such that $a_{k} < r_{j,n-1}$, we have
\begin{align}
\label{eq:slope2}
\begin{aligned}
  \Delta_{k}(\cont) ~=~& \mathcal{L}_{j}(r_{j,n},\cont) -   \mathcal{L}_{j}(r_{j,n-1},\cont) + \mathcal{L}_{j}(r_{j,n-1},\cont) - \mathcal{L}_{j}(a_{k},\cont)\\
  ~>~&  \mathcal{L}_{j}(r_{j,n-1},\cont) - \mathcal{L}_{j}(a_{k},\cont)\\
  ~\overset{(i)}{\geq} ~&  \slope_{j,n-1}(\cont) (r_{j,n-1} - a_{k})\\
   ~\overset{(ii)}{\geq} ~& \left( \slope_{j,n-1}(\cont) -  \slope_{j,n}(\cont)\right) (r_{j,n-1} - a_{k})\\
    ~\overset{(iii)}{=} ~& (1+\lambda)\left(s_{j,n-1}-s_{j,n}\right) (r_{j,n-1} - a_{k})\\
     ~> ~& \left(s_{j,n-1}-s_{j,n}\right) (r_{j,n-1} - a_{k})
\end{aligned}
\end{align}
where in (i) we recall the slope $\slope_{j,n-1}(\cont)$ is defined in Lemma \ref{lem:Vstruct} and further (i) follows from concavity of $ \mathcal{L}_{j}(\rho{j},\cont)$ in the first argument $\rho_{j}$; in (ii) we used the fact that $ \slope_{j,n}(\cont)\geq 0$ since the optimal budget 
$\arg\max_{\rho_{j}\in [0,\rho]} \mathcal{L}_{j}(\rho_{j}, \cont)$ is taken at the $n$th turning point, and is the largest turning point whose left slope is non-negative from  Lemma \ref{lem:Vstruct}; (iii) follows from the definition $\slope_{j,n'}(\cont) = (1+\lambda)s_{j,n'} - (\mu+\gamma\lambda)$ for any $n'$. 


Finally combining Eq. \eqref{eq:nbadslope}, \eqref{eq:slope} and \eqref{eq:slope2}, and summing over $n = 1 \dots S_{j}$ we get
\begin{align}
\begin{aligned}
\label{eq:X1secbound}
  & \sum_{t\in[T]:\cont_{t} \notin \contset(\underline{\slope})} ~ \sum_{k\in[K]:a_{k} < \min \adj_{j}^{-}(\cont_{t})} ~  \Delta_{k}(\cont_{t}) \I\{\rho_{j,t} = a_{k}, N_{k,t} \leq m_{k}(\cont_{t})\}   \\
 ~=~& \sum_{n\in [S_{j}]} \sum_{t\in[T]:\cont_{t} \in \contset_{n}/\contset(\underline{\slope})} ~ \sum_{k\in[K]:a_{k} < \min \adj_{j}^{-}(\cont_{t})} ~  \Delta_{k}(\cont_{t}) \I\{\rho_{j,t} = a_{k}, N_{k,t} \leq m_{k}(\cont_{t})\} \\
 ~\leq~& \sum_{n\in [S_{j}]}\left((1+\dualub_{F})s_{j,n-1} \discerr + \rho \underline{\slope}\right) T  + \sum_{n\in [S_{j}]}~\sum_{k\in[K]:a_{k} < r_{j,n-1}-\discerr} \frac{8\log(T)}{\left(s_{j,n-1}-s_{j,n}\right) (r_{j,n-1} - a_{k})}\\
 ~\overset{(i)}{\leq}~& \sum_{n\in [S_{j}]}\left((1+\dualub_{F})s_{j,n-1} \discerr + \rho \underline{\slope}\right) T  + \sum_{n\in [S_{j}]}~\sum_{\ell=1}^{K} \frac{8\log(T)}{\left(s_{j,n-1}-s_{j,n}\right) \ell \discerr}\\
 ~\leq~& \sum_{n\in [S_{j}]}\left((1+\dualub_{F})s_{j,n-1} \discerr + \rho \underline{\slope}\right) T  + \frac{8\log(T)\log(K)}{\discerr} \sum_{n\in [S_{j}]}~\frac{1}{\left(s_{j,n-1}-s_{j,n}\right)}\\
 ~=~& \mathcal{O}(\discerr T + \underline{\slope}T + \frac{1}{\discerr})\,.
 \end{aligned}
\end{align}
Note that (i) follows because for all $a_{k} < r_{j,n-1} - \discerr$, the $a_{k}$'s distances from $r_{j,n-1}$ are at least $\discerr, 3\discerr, 2\discerr \dots $. 

(3) The cases where arm $a_k \in \adj_{j}^{+}(\cont_{t})$ and $a_{k} > \max \adj_{j}^{+}(\cont_{t})$
are symmetric to $a_k \in \adj_{j}^{-}(\cont_{t})$ and $a_{k} < \min \adj_{j}^{+}(\cont_{t})$, respectively, and we omit from this paper. 

Therefore, combining Eq. \eqref{eq:X1near} and \eqref{eq:X1secbound} we  can conclude 
\begin{align}
    X_{1} \leq  \mathcal{O}(\discerr T + \underline{\slope}T + \frac{1}{\discerr})
\end{align}



\subsubsection{Bounding $X_{2}$.}
\label{subsubsec:X2}
We first rewrite $X_{2}$ as followed
\begin{align}
\label{eq:X2all}
\begin{aligned}
    X_{2} ~=~& \sum_{t\in[T]:\cont_{t} \in \contset(\underline{\slope})} \sum_{k\in [K]} \Delta_{k}(\cont_{t}) \I\{\rho_{j,t} = a_{k}, N_{k,t} \leq m_{k}(\cont_{t})\} \\
     ~=~& \sum_{t\in[T]}\sum_{n\in[S_{j}]}\sum_{k\in [K]}\sum_{\cont \in \contset_{n}\cap \contset(\underline{\slope})}  \Delta_{k}(\cont) \I\{\cont_{t}=\cont, \rho_{j,t} = a_{k}, N_{k,t} \leq m_{k}(\cont)\} \\
     ~\overset{(i)}{=}~& 
   \sum_{n\in[S_{j}]}\sum_{k\in [K]}\sum_{\cont \in \contset_{n}\cap \contset(\underline{\slope})} \Delta_{k}(\cont) Y_{k}(\cont)\\
    ~\overset{(ii)}{=}~&  T \discerr (1+\dualub_{F}) \sum_{n\in[S_{j}]} \left(s_{j,n} + s_{j,n+1}\right) + 
   \sum_{n\in[S_{j}]}~\sum_{k\in [K]/\{k_{n}^{-},k_{n}^{+}\}}~\sum_{\cont \in \contset_{n}\cap \contset(\underline{\slope})} \Delta_{k}(\cont) Y_{k}(\cont)\,.
    \end{aligned}
\end{align}
where in (i) we define 
$Y_{k}(\cont) =  \sum_{t\in[T]}\I\{\cont_{t} = \cont, \rho_{j,t} = a_{k}, N_{k,t} \leq m_{k}(\cont)\}$;  in (ii) for any context $\cont \in \contset_{n}\cap \contset(\underline{\slope})$, the optimal budget $\arg\max_{\rho_{j}\in [0,\rho]} \mathcal{L}_{j}(\rho_{j}, \cont) = r_{j,n}$ is taken at the $n$th turning point per the definition of $\contset_{n}$ in Eq. \eqref{eq:UCBdefs}, and further we defined $k_{n}^{-}:= \max\{k\in [K]: a_{k} < r_{j,n}\}$ to be the arm closest to and no greater than  $r_{j,n}$, whereas  $k_{n}^{+}:= \min\{k\in [K]: a_{k} > r_{j,n}\}$ to be the arm closest to and no less than  $r_{j,n}$. Thus for small enough $\discerr < \min_{n'\in[S_{j}]}r_{j,n'} - r_{j,n'-1} $,  $k_{n}^{-}$ lies on the line segment between $r_{j,n-1}$ and $r_{j,n}$, so $\Delta_{k_{n}^{-}}(\cont) = \slope_{j}^{-}(\cont)(r_{j,n} - a_{k_{n}^{-}}) \leq \slope_{j}^{-}(\cont) \discerr \leq (1+\dualub_{F})s_{j,n-1} \discerr$, where in the final inequality follows from the definition of  $\slope_{j}^{-}(\cont) = \slope_{j,n}(\cont) = (1+\lambda)s_{j,n} - (\mu + \gamma\lambda) \leq (1+\lambda)s_{j,n} \leq (1+\dualub_{F})s_{j,n}$ where $\dualub_{F}$ is defined in Eq. \eqref{lem:dualvarub}. A similar bound holds for 
$\Delta_{k_{n}^{+}}(\cont)$. 


Then, following the same logic as Eq. \eqref{eq:numbadarms}, \eqref{eq:slope}, \eqref{eq:slope2} in Section \ref{subsubsec:X1} where we bound $X_{1}$, we can bound $\sum_{\cont \in \contset_{n}\cap \contset(\underline{\slope})} \Delta_{k}(\cont) Y_{k}(\cont)$ as followed:
\begin{align}
\label{eq:X2slope}
    \sum_{\cont \in \contset_{n}\cap \contset(\underline{\slope})} \Delta_{k}(\cont) Y_{k}(\cont) \leq \frac{8\log(T)}{\min_{\cont \in \contset_{n}\cap \contset(\underline{\slope})}\Delta_{k}(\cont)}\,.
\end{align}

Now, the set $k\in [K]/\{k_{n}^{-},k_{n}^{+}\}$ in Eq. \eqref{eq:X2all} can be split into two sets, namely $\{k\in [K]: a_{k} < r_{j,n} - \discerr\}$ and $\{k\in [K]: a_{k} > r_{j,n} + \discerr\}$ due to the definitions $k_{n}^{-}:= \max\{k\in [K]: a_{k} < r_{j,n}\}$ and $k_{n}^{+}:= \min\{k\in [K]: a_{k} > r_{j,n}\}$. Therefore, for any $k$ s.t. $ a_{k} < r_{j,n} - \discerr$ and any $\cont \in  \contset_{n}\cap \contset(\underline{\slope})$, 
\begin{align*}
    \Delta_{k}(\cont) = \mathcal{L}_{j}(r_{j,n},\cont) - \mathcal{L}_{j}(a_{k},\cont) \geq \slope_{j}^{-}(\cont) (r_{j,n} - a_{k}) \geq \underline{\slope}  (r_{j,n} - a_{k}),,
\end{align*}
where the final inequality follows from the definition of $\contset(\underline{\slope})$ in Eq. \eqref{eq:UCBdefs} such that $ \slope_{j}^{-}(\cont) \geq \underline(\slope) $ for $\cont \contset(\underline{\slope})$. Hence combining this with Eq. \eqref{eq:X2slope} we have
\begin{align}
\label{eq:X2last}
    \sum_{k\in [K]:a_{k} < r_{j,n}- \discerr}~ \sum_{\cont \in \contset_{n}\cap \contset(\underline{\slope})} \Delta_{k}(\cont) Y_{k}(\cont) \leq  \sum_{k\in [K]:a_{k} < r_{j,n}- \discerr}\frac{8\log(T)}{ \underline{\slope}  (r_{j,n} - a_{k})} \overset{(i)}{\leq} \sum_{\ell=1}^{K}\frac{8\log(T)}{ \underline{\slope} \ell \discerr} \leq\frac{8\log(T)\log(K)}{\underline{\slope} \discerr} 
\end{align}
where (i) follows because for all $a_{k} < r_{j,n} - \discerr$, the $a_{k}$'s distances from $r_{j,n-1}$ are at least $\discerr, 3\discerr, 2\discerr \dots $. Symmetrically, we can show an identical bound for the set  $\{k\in [K]: a_{k} > r_{j,n} + \discerr\}$. Hence, combining Eq. \eqref{eq:X2all} and \eqref{eq:X2last} we can conclude
\begin{align}
    X_{2}\leq \mathcal{O}\left(\discerr T + \frac{1}{\discerr \underline{\slope}}\right).
\end{align}

\subsubsection{Bounding $X_{3}$.}
\label{subsubsec:X3}
For any arm $k \in [K]$, denote $ \ucbtot_{t}(a_{k}) =\Bar{\totv}_{t}(a_{k})  - \frac{\lambda_{t} \gamma + \mu_{t} }{1+\lambda_{t}}a_{k}$. Also, define $\Bar{\mathcal{L}} = \left(1+\gamma \right)\rho\dualub_{F} + (1+\dualub_{F})\Bar{\totv}$, where $\dualub_{F}$ is specified in Lemma \ref{lem:dualvarub}, and $a_{t}^{*} = \arg\max_{a_{k'}\in \budgset(\discerr)} \mathcal{L}_{j}(a_{k'}, \cont_{t})$ for convenience. Then we bound $X_{3}$ as followed 
\begin{align}
\label{eq:X3first}
\begin{aligned}
   X_{3} ~=~&  \sum_{t\in[T]} \E\left[\Delta_{k}(\cont) \I\{ \rho_{j,t} = a_{k}, N_{k,t} > m_{k}(\cont)\}\right] \\
    ~\overset{(i)}{\leq}~& \Bar{\mathcal{L}}\cdot \prob\left(\rho_{j,t} = a_{k}, N_{k,t} > m_{k}(\cont_{t})\right)\\
    ~\leq~& \Bar{\mathcal{L}} \cdot  \sum_{t\in[T]} \prob\left(\ucbtot_{t}(a_{k}) +  \ucb_{j,t}(a_{k}) \geq \ucbtot_{t}(a_{t}^{*})+  \ucb_{j,t}(a_{t}^{*}), N_{k,t} > m_{k}(\cont_{t})\right)\,,
\end{aligned}
\end{align}
where (i) follows from Lemma \ref{lem:dualvarub} such that $  -\left(1+\gamma \right)\rho\dualub_{F}
 ~\leq~ \mathcal{L}_{j}(\rho_{j},\cont_{t})~\leq~(1+\dualub_{F})\Bar{\totv}$ for all $j \in [M]$, $t\ in [T]$, $\rho_{j} \in [0,\rho]$ and $\cont_{t}$.

Now let $\Bar{\ucbtot}_{n}(a_{k})$ denote the average conversion of arm $k$ over its first $n$ pulls, i.e. letting $\tau = \min\{t\in [T]:N_{k,t} = n\}$ be the period during which arm $k$ is pulled for the $n$th time, then 
$\Bar{\ucbtot}_{n}(a_{k}) =\Bar{\totv}_{j,\tau}(a_{k})$, where $\Bar{\totv}_{j,\tau}$ is defined in Algorithm \ref{alg:omducb}. Hence, we continue as follwoed 
\begin{align}
\label{eq:X3sec}
\begin{aligned}
 &\prob\left(\ucbtot_{t}(a_{k}) +  \ucb_{j,t}(a_{k}) \geq \ucbtot_{t}(a_{t}^{*})+  \ucb_{j,t}(a_{t}^{*}), N_{k,t} > m_{k}(\cont_{t})\right)\\
    ~\leq~&  \prob\left(\max_{m_{k}(\cont_{t}) < n \leq t} \Bar{\ucbtot}_{n}(a_{k}) + \ucb_{t}(a_{k}) - \frac{\lambda_{t} \gamma + \mu_{t} }{1+\lambda_{t}}a_{k} \geq \min_{1\leq n'\leq t}\Bar{\ucbtot}_{n}(a_{t}^{*}) + \ucb_{t}(a_{t}^{*}) - \frac{\lambda_{t} \gamma + \mu_{t} }{1+\lambda_{t}}a_{t}^{*}
    \right)\\
    ~\leq~& \sum_{ n = \left\lceil m_{k}(\cont_{t}) \right\rceil+1}^{t}\sum_{n'=1}^{t}\prob\left(\Bar{\ucbtot}_{n}(a_{k}) + \ucb_{n}(a_{k}) - \frac{\lambda_{t} \gamma + \mu_{t} }{1+\lambda_{t}}a_{k} > \Bar{\ucbtot}_{n'}(a_{t}^{*}) + \ucb_{n'}(a_{t}^{*}) - \frac{\lambda_{t} \gamma + \mu_{t} }{1+\lambda_{t}}a_{t}^{*}
    \right)
    \end{aligned}
\end{align}
Now, when the event $\left\{\Bar{\ucbtot}_{n}(a_{k}) + \ucb_{n}(a_{k}) - \frac{\lambda_{t} \gamma + \mu_{t} }{1+\lambda_{t}}a_{k} > \Bar{\ucbtot}_{n}(a_{t}^{*}) + \ucb_{n'}(a_{t}^{*}) - \frac{\lambda_{t} \gamma + \mu_{t} }{1+\lambda_{t}}a_{t}^{*}
    \right\}$ occurs, it is easy to see that one of the following events must also occur:
\begin{align}
\label{eq:event}
\begin{aligned}
    & \mathcal{G}_{1,n} =\left\{  \Bar{\ucbtot}_{n}(a_{k})  \geq \totv(a_{k}) + \ucb_{n}(a_{k})\right\} \\
    & \mathcal{G}_{2,n'} =\left\{  \Bar{\ucbtot}_{n'}(a_{t}^{*})  \leq \totv(a_{t}^{*}) -\ucb_{n}(a_{t}^{*}) \right\}\\
    & \mathcal{G}_{3} =\left\{   \totv(a_{t}^{*}) -  \frac{\lambda_{t} \gamma + \mu_{t} }{1+\lambda_{t}}a_{t}^{*}~<~ \totv(a_{k}) - \frac{\lambda_{t} \gamma + \mu_{t} }{1+\lambda_{t}}a_{k}  + 2 \cdot \ucb_{n}(a_{k}) \right\}\\
    \end{aligned}
\end{align}
Note that for $n > m_{k}(\cont_{t})$, we have 
$\ucb_{n}(a_{k}) = \sqrt{\frac{2\log(T)}{n}} < \sqrt{\frac{2\log(T)}{m_{k}(\cont_{t})}} = \frac{\Delta_{k}(\cont_{t})}{2}$ since we defined $m_{k}(\cont) = \frac{8\log(T)}{\Delta_{k}^{2}(\cont)}$ in Eq. \eqref{eq:UCBdefs}. Therefore
\begin{align*}
    \totv(a_{k}) - \frac{\lambda_{t} \gamma + \mu_{t}}{1+\lambda_{t}}a_{k} + 2 \cdot \ucb_{n}(a_{k}) <  \underbrace{\totv(a_{k}) - \frac{\lambda_{t} \gamma + \mu_{t}}{1+\lambda_{t}}a_{k}}_{=\mathcal{L}(a_{k},\cont_{t})} + \Delta_{k}(\cont_{t}) ~\overset{(i)}{=}~ \underbrace{\totv(a_{t}^{*}) -  \frac{\lambda_{t} \gamma + \mu_{t} }{1+\lambda_{t}}a_{t}^{*}}_{=\mathcal{L}(a_{t}^{*},\cont_{t}) = \max_{a\in \budgset(\discerr)}\mathcal{L}(a,\cont_{t})}
\end{align*}
where (i) follows from the definition of $\Delta_{k}(\cont) = \max_{a\in \budgset(\discerr)}\mathcal{L}(a,\cont) - \mathcal{L}(a_{k},\cont)$ in Eq. \eqref{eq:UCBdefs} for any context $\cont$. This implies that event $\mathcal{G}_{3}$ in Eq. \eqref{eq:event} cannot hold for $n >  m_{k}(\cont_{t})$. Therefore
\begin{align}
\label{eq:X3third}
    \prob\left(\Bar{\ucbtot}_{n}(a_{k}) + \ucb_{n}(a_{k}) - \frac{\lambda_{t} \gamma + \mu_{t} }{1+\lambda_{t}}a_{k} > \Bar{\ucbtot}_{n'}(a_{t}^{*}) + \ucb_{n'}(a_{t}^{*}) - \frac{\lambda_{t} \gamma + \mu_{t} }{1+\lambda_{t}}a_{t}^{*}
    \right)~\leq~\prob\left(\mathcal{G}_{1,n} \cup \mathcal{G}_{2,n'}
    \right)
\end{align}

From standard UCB analysis and the Azuma Hoeffding's inequality, we have $\prob(\mathcal{G}_{1,n} )\leq \frac{\Bar{\totv}}{T^{4}}$ and  $\prob(\mathcal{G}_{2,n'} )\leq \frac{\Bar{\totv}}{T^{4}}$. Hence combining Eq. \eqref{eq:X3first} \eqref{eq:X3sec}, \eqref{eq:X3third} we can conclude

\begin{align}
\begin{aligned}
 X_{3} ~\leq~& \sum_{t\in[T]}\sum_{n = \left\lceil m_{k}(\cont_{t}) \right\rceil+1}^{t}\sum_{n'=1}^{t}\left(\prob\left(\mathcal{G}_{1,n}\right) + \prob\left(\mathcal{G}_{2,n'}
    \right)\right)\\
    ~\leq~& \sum_{t\in[T]}\ \sum_{n = \left\lceil m_{k}(\cont_{t}) \right\rceil+1}^{t}\sum_{n'=1}^{t} \frac{2\Bar{\totv}}{T^{4}}\\
     ~\leq~&  \frac{2\Bar{\totv}}{T}
    \end{aligned}
\end{align}
\halmos


\subsection{Proof for Lemma \ref{lem:boundcs}}
\label{pf:lem:boundcs}
Recall $g_{1,t} = \sum_{j\in [M]}\left(\totv_{j,t}(\rho_{j,t}) - \gamma \rho_{j,t}\right)$ and $g_{2,t} = \rho - \sum_{j\in [M]}\rho_{j,t}$ defined in Algorithm \ref{alg:omducb}.
% Let $\mathcal{H}_{t}$ be the sigma-algebra generated by $\{(\bm{v}_{j,\tau},\bm{d}_{j,\tau})_{j\in [M]}\}_{\tau = 1 \dots t}$, then we recognize $(\rho_{j,t},\lambda_{t},\mu_{t})$ are $\mathcal{H}_{t-1}$-measurable, and further
% \begin{align}
% \begin{aligned}
%     &\E\left[\lambda_{t}g_{1,t} + \mu_{t}g_{2,t}| \mathcal{H}_{t-1}\right] \\ ~=~ & \E\left[\lambda_{t} \sum_{j\in [M]}\left(\totv_{j,t}(\rho_{j,t}) - \gamma \rho_{j,t}\right) + \mu_{t}\left( \rho - \sum_{j\in [M]}\rho_{j,t}\right)\Big|  \mathcal{H}_{t-1}\right] \\
%     ~\overset{(i)}{=}~ & \lambda_{t} \sum_{j\in [M]}\left(\totv_{j}(\rho_{j,t}) - \gamma \rho_{j,t}\right) + \mu_{t}\left( \rho - \sum_{j\in [M]}\rho_{j,t}\right)\\
%     ~=~ & g_{t}\,,
%     \end{aligned}
% \end{align}
% where in (i) we used $\E\left[\totv_{j,t}(\rho_{j,t})|\mathcal{H}_{t-1}\right]=\totv_{j}(\rho_{j,t}) $. Therefore we have
% \begin{align}
% \label{eq:history}
%      \sum_{t\in[T]} \E\left[g_{t}\right] = \sum_{t\in[T]} \E\left[\E\left[\lambda_{t}g_{1,t} + \mu_{t}g_{2,t}| \mathcal{H}_{t-1}\right]\right] =\sum_{t\in[T]} \E\left[\lambda_{t}g_{1,t} + \mu_{t}g_{2,t}\right]\,.
% \end{align}
% Next, 

Now from lemma \ref{lem:omdtelescope}, we have for any $\lambda\geq 0$ and $\mu\geq 0$,
\begin{align*}
\begin{aligned}
    & \sum_{t} \left(\lambda_{t} - \lambda\right) g_{1,t} \leq  \frac{\eta M^{2}\Bar{\totv}^{2}}{2} \cdot T +  \frac{1}{2\eta}(\lambda- \lambda_{1})^{2}\\
    & \sum_{t} \left(\mu_{t} - \mu\right) g_{2,t} \leq  \frac{\eta \rho^{2}}{2} \cdot T +  \frac{1}{2\eta}(\mu- \mu_{1})^{2}\,.
  \end{aligned}  
\end{align*}
By taking $\lambda = \mu = 0$ and recalling $\lambda_{1} = \mu_{1} = 0$, we get the desired bound in the statement of the lemma. 
\halmos


\subsection{Proof for Theorem \ref{thm:regret}}
\label{pf:thm:regret}
Starting from Proposition \ref{prop:ubbenchlag}, we get
\begin{align}
\begin{aligned}
    T\cdot \textsc{GL-OPT} - \E\left[\sum_{t\in [T]}\sum_{j\in[M]}\totv_{j}(\rho_{j,t})\right]~\leq~& M\Bar{V}K +  \sum_{j\in [M]} \sum_{t > K} 
     \E\left[\mathcal{L}_{j}(\rho_{j}^{*}(t), \cont_{t}) - \mathcal{L}_{j}(\rho_{j,t}, \cont_{t})\right] +  \sum_{t > K}\left(\lambda_{t}g_{1,t} + \mu_{t}g_{2,t}\right)\\
     ~\overset{(i)}{\leq}~&M\Bar{V}K  + \mathcal{O}\left(\underline{\slope}T + \discerr T + \frac{1}{\underline{\slope} \discerr}\right) + \mathcal{O}\left(\eta T + \frac{1}{\eta}\right)
     \end{aligned}
\end{align}
where in (i) we applied Lemma \ref{lem:ucbregret} and \ref{lem:boundcs}. Taking $\eta = 1/\sqrt{T}$, $\discerr = \underline{\slope} = T^{-1/3}$ (i.e. $K = t^{1/3}$ yields $ T\cdot \textsc{GL-OPT} - \E\left[\sum_{t\in [T]}\sum_{j\in[M]}\totv_{j}(\rho_{j,t})\right] \leq \mathcal{O}(T^{2/3})$. According to Lemma \ref{lem:Vstruct}, $\totv_{j}(\rho_{j})$ is concave for all $j \in [M]$, so
\begin{align}
\begin{aligned}
    \mathcal{O}(T^{-1/3})~\geq~& \textsc{GL-OPT} -  \frac{1}{T}\sum_{t\in [T]} \E\left[\sum_{j\in[M]}\totv_{j}(\rho_{j,t})\right] \\
    ~\geq~&  \textsc{GL-OPT}  - \E\left[ \sum_{j\in[M]}  \totv_{j}\left(\frac{1}{T}\sum_{t\in [T]} \rho_{j,t}\right)\right]\\
     ~\geq~&  \textsc{GL-OPT}  - \E\left[ \sum_{j\in[M]}\totv_{j}(\Bar{\rho}_{T,j})\right]
     \end{aligned}
\end{align}
where in the final equality we used the definition $\Bar{\bm{\rho}}_{T}$ as defined in Algorithm \ref{alg:omducb}. 


On the other hand, Lemma \ref{lem:boundcs} shows 
\begin{align}
\begin{aligned}
    -\mathcal{O}(1/\sqrt{T}) ~\leq~& \frac{1}{T}\sum_{t\in[T]} \E\left[g_{1,t}\right]\\
    ~=~& \frac{1}{T}\sum_{t\in[T]}\sum_{j\in [M]}\E\left[\left(\totv_{j}(\rho_{j,t};\bm{z}_{t}) - \gamma \rho_{j,t}\right)\right]\\
     ~=~& \frac{1}{T}\sum_{t\in[T]}\sum_{j\in [M]}\E\left[\left(\totv_{j}(\rho_{j,t}) - \gamma \rho_{j,t}\right)\right]\\
    ~\overset{(i)}{\leq}~&\sum_{j\in [M]}\left(\totv_{j}\left( \frac{1}{T}\sum_{t\in[T]}\rho_{j,t}\right) - \gamma \cdot \frac{1}{T}\sum_{t\in[T]}\rho_{j,t}\right)\\
     ~=~&\sum_{j\in [M]}\left(\totv_{j}\left(\Bar{\rho}_{T,j}\right) - \gamma \Bar{\rho}_{T,j}\right)\,.
     \end{aligned}
\end{align}
where in (i) we again applied concavity of $\totv_{j}(\rho_{j})$. We omit the analysis for the budget constraint as it is similar to the above.
\halmos




\subsection{Additional Results for Section \ref{sec:online}}
\label{app:onlineadd}

Assumption \ref{ass:feas} ensures that for any realization $\bm{z}=(\bm{v},\bm{d})$ there must be some per-channel budget allocation that allows the advertiser to satisfy her ROI constraints as illustrated in the following proposition
\begin{proposition}[Slater's condition]
\label{prop:slater}
Assume Assumption \ref{ass:feas} holds. Let  $\bm{z}=(\bm{v},\bm{d}) = (\bm{v}_{j},\bm{d}_{j})_{j\in[M]} \in F_{1}\times \dots F_{M}$ be any realization of values and costs across all channels, then there exists some per-channel budget allocation $\rho_{(\bm{z})} \in [0,\rho]^{M}$ s.t. $ \sum_{j \in M} \totv_{j}(\rho_{(\bm{z}),j};\bm{z} ) > \gamma \sum_{j \in M} \rho_{(\bm{z}),j}$ and $ \sum_{j\in [M]}\rho_{(\bm{z}),j} < \rho$.
\end{proposition}
\textit{Proof.} Under Assumption \ref{ass:feas}, it is easy to see for any realization of value-cost pairs  $\bm{z} = (\bm{v}_{j},\bm{d}_{j})_{j\in[M]}$ there always exists a channel $j\in [M]$ in which there is an auction $n\in [m_{j}]$ whose value-to-cost ration is at least $\gamma$, i.e. $v_{j,n} >  \gamma d_{j,n}$. Since we assumed the ordering $\frac{v_{j,1}}{d_{j,1}} > \frac{v_{j,2}}{d_{j,2}} > \dots  > \frac{v_{j,m_{j}}}{d_{j,m_{j}}}$, we know that 
$\frac{v_{j,1}}{d_{j,1}}\geq \frac{v_{j,n}}{d_{j,n}} > \gamma$. Now, in Eq. \eqref{eq:pieceline} within the proof of Lemma \ref{lem:Vstruct}, we showed 
\begin{align*}
   \totv_{j}(\rho_{j};\bm{z}_{j}) = \bm{v}_{j}^{\top} \bm{x}_{j}^{*}(\rho_{j};\bm{z}_{j})=  \sum_{n \in [m_{j}]}\left(\frac{v_{j,n}}{d_{j,n}}\rho_{j}+ \widetilde{b}_{j,n}\right)\I\left\{d_{j,0}+ \dots +d_{j,n-1}\leq \rho_{j}\leq d_{j,0}+ \dots +d_{j,n} \right\}
\end{align*}
where $\widetilde{b}_{j,n} = \sum_{n' \in [n-1]} v_{j,n'} - \frac{v_{j,n}}{d_{j,n}}\cdot \left(\sum_{n' \in [n-1]} d_{j,n'}\right)$ and $  d_{j,0} = v_{j,0} = 0$. Hence by taking $\rho_{j} = \underline{\rho}$ for some $ \underline{\rho} < \min\{d_{j,1},\rho\}$, we have $\totv_{j}(\underline{\rho}; \bm{z}_{j}) = \frac{v_{j,1}}{d_{j,1}}\underline{\rho} > \gamma \underline{\rho}$. Therefore, constructing $\rho_{(\bm{z}),j} = (0,\dots,0,\rho_{j},0\dots 0)$ for $\rho_{j} = \underline{\rho}$ satisfies $ \sum_{j \in M} \totv_{j}(\rho_{(\bm{z}),j};\bm{z} ) > \gamma \sum_{j \in M} \rho_{(\bm{z}),j}$ and $ \sum_{j\in [M]}\rho_{(\bm{z}),j} < \rho$.
\halmos

\begin{lemma}[Approximate constraint satisfaction]
\label{lem:approxconst}
Assume Assumption \ref{ass:feas} holds. If Algorithm \ref{alg:omducb} is run with stepsize $\eta = 1/\sqrt{T}$ such that $\eta < \frac{1}{M \max\left\{\totv, \rho, \totv^{2}\right\} }$, then we have 
\begin{align*}
     \frac{1}{T}\sum_{t\in[T]}g_{1,t} \geq -\dualub_{F}/\sqrt{T} \text{ and }
  \frac{1}{T}\sum_{t\in[T]}g_{2,t} \geq -\dualub_{F}/\sqrt{T} 
\end{align*}
where we recall $g_{1,t} = \sum_{j\in [M]}\left(\totv_{j}(\rho_{j,t};\bm{z}_{t}) - \gamma \rho_{j,t}\right)$, $g_{2,t} = \rho - \sum_{j\in [M]}\rho_{j,t}$, and $\dualub_{F} >0 $ is an absolute constant defined in Lemma \ref{lem:dualvarub} that depends only on the support $F = F_{1} \times \dots F_{M}$.
\end{lemma}

\textit{Proof.}
According to the dual update step in Algorithm \ref{alg:omducb} wee have
\begin{align}
    \lambda_{t+1} = \left(\lambda_{t} - \eta g_{1,t}\right)_{+} \geq \lambda_{t} - \eta g_{1,t}
\end{align}
Summing from $t = 1 \dots T-1$ and telescoping, we get
\begin{align}
    \lambda_{T} \geq \lambda_{1} - \eta \sum_{t\in[T]}g_{1,t} = - \eta \sum_{t\in[T]}g_{1,t} 
\end{align}
From Lemma \ref{lem:dualvarub}, we have $ \lambda_{T} \leq \dualub_{F}$ for some absolute constant $\dualub_{F} >0$, therefore we have
\begin{align}
    \sum_{t\in[T]}g_{1,t} \geq -\frac{\dualub_{F}}{\eta} 
\end{align}
since we take $\eta = 1/\sqrt{T}$. A similar bound holds for $ \sum_{t\in[T]}g_{2,t}$.
\halmos

\begin{lemma}
\label{lem:omdtelescope}
    Let $(\lambda_{t},\mu_{t})_{t\in[T]}$ be the dual variables generated by Algorithm \ref{alg:omducb}. Then for any $\lambda,\mu\geq 0$ we have
\begin{align}
\label{eq:CSbound}
\begin{aligned}
    & \sum_{t} \left(\lambda_{t} - \lambda\right) g_{1,t} \leq  \frac{\eta M^{2}\Bar{\totv}^{2}}{2} \cdot T +  \frac{1}{2\eta}(\lambda- \lambda_{1})^{2}\\
    & \sum_{t} \left(\mu_{t} - \mu\right) g_{2,t} \leq  \frac{\eta \rho^{2}}{2} \cdot T +  \frac{1}{2\eta}(\mu- \mu_{1})^{2}\,.
  \end{aligned}  
\end{align}
where we  recall $g_{1,t} = \sum_{j\in [M]}\left(\totv_{j,t}(\rho_{j,t}) - \gamma \rho_{j,t}\right)$ and $g_{2,t} = \rho - \sum_{j\in [M]}\rho_{j,t}$. 
\end{lemma}
\textit{Proof.}
It only remains to prove Eq. \eqref{eq:CSbound}. Starting with the first inequality w.r.t. $\lambda_{t}$'s, we have
\begin{align}
\label{eq:decompCS}
    \left(\lambda_{t} - \lambda\right) g_{1,t} =  \left(\lambda_{t+1} - \lambda\right) g_{1,t}  +  \left(\lambda_{t} - \lambda_{t+1}\right) g_{1,t} 
\end{align}
Since $\lambda_{t+1} = \left(\lambda_{t} - \eta g_{1,t}\right)_{+} = \arg\min_{\lambda\geq0}\left(\lambda - \left(\lambda_{t} - \eta g_{1,t}\right)\right)^{2}$, we have
\begin{align}
    \left(\lambda_{t+1} - \left(\lambda_{t} - \eta g_{1,t}\right)\right)\cdot (\lambda - \lambda_{t+1}) \geq 0\,.
\end{align}
So we have
\begin{align}
\begin{aligned}
     \left(\lambda_{t+1} - \lambda\right) g_{1,t}~\leq~ & \frac{1}{\eta}(\lambda_{t+1} - \lambda_{t})\cdot(\lambda - \lambda_{t+1})\\
     ~=~& \frac{1}{2\eta}\left((\lambda- \lambda_{t})^{2} - (\lambda- \lambda_{t+1})^{2}-(\lambda_{t+1}- \lambda_{t})^{2}\right)
     \end{aligned}
\end{align}
Plugging the above back into Eq. \eqref{eq:decompCS} we get
\begin{align}
\label{eq:omdtelescope}
\begin{aligned}
     \left(\lambda_{t} - \lambda\right) g_{1,t} ~\leq~&  \left(\lambda_{t} - \lambda_{t+1}\right) g_{1,t}  +  \frac{1}{2\eta}\left((\lambda- \lambda_{t})^{2} - (\lambda- \lambda_{t+1})^{2}-(\lambda_{t+1}- \lambda_{t})^{2}\right)\\
     ~\leq~&  
   \frac{\eta}{2}g_{1,t}^{2}  +  \frac{1}{2\eta}\left((\lambda- \lambda_{t})^{2} - (\lambda- \lambda_{t+1})^{2}\right)\\
    ~\leq~&  
   \frac{\eta M^{2}\Bar{\totv}^{2}}{2}  +  \frac{1}{2\eta}\left((\lambda- \lambda_{t})^{2} - (\lambda- \lambda_{t+1})^{2}\right)\,,
   \end{aligned}
\end{align}
where the final inequality follows from the fact that $\totv_{j,t}(\rho_{j,t})\leq \Bar{\totv}$ for any $j\in [M]$ and $t\in [T]$ so $g_{1,t}\leq M\Bar{\totv}$. Summing the above over $t =1\dots T$ and telescoping we get
\begin{align*}
    \sum_{t} \left(\lambda_{t} - \lambda\right) g_{1,t} \leq  \frac{\eta M^{2}\Bar{\totv}^{2}}{2} \cdot T +  \frac{1}{2\eta}(\lambda- \lambda_{1})^{2}
\end{align*}
Following the same arguments above we can show 
\begin{align*}
   \sum_{t} \left(\mu_{t} - \mu\right) g_{2,t} \leq  \frac{\eta \rho^{2} }{2} \cdot T +  \frac{1}{2\eta}(\mu- \mu_{1})^{2}
\end{align*} 
\halmos



\begin{proposition}
\label{prop:convexprob}
    Under Assumption \ref{ass:feas}, the advertiser's per-channel only budget optimization problem, namely $\textsc{CH-OPT}(\mathcal{I}_{\budg})$ is a convex problem.
\end{proposition}
\text{Proof.}
Recalling the $\textsc{CH-OPT}(\mathcal{I}_{\budg})$ in Eq. \eqref{eq:chopt} and the definition of $\mathcal{I}_{\budg}$ in Eq. \eqref{eq:option}, we can write $\textsc{CH-OPT}(\mathcal{I}_{\budg})$ as
\begin{align}
\begin{aligned}
   \textsc{CH-OPT}(\mathcal{I}_{\budg})=  \max_{(\gamma_{j})_{j\in [M]}\in \mathcal{I}} ~&~ \sum_{j \in M} \totv_{j}(\rho_{j})\\
    \text{s.t. } &  \sum_{j \in M} \totv_{j}(\rho_{j}) \geq \gamma \sum_{j \in M} \rho_{j}\\
   &   \sum_{j\in [M]}\rho_{j}\leq \rho\,,
    \end{aligned}
\end{align}
Here we used the definition $\totv_{j}(\rho_{j}) = \E\left[\totv_{j}(\rho_{j};\bm{z}_{j})\right]$ in Eq. \eqref{eq:budperchannel}, and $\totc_{j}(\rho_{j};\bm{z}_{j}) = \rho_{j}$ for any $\bm{z}_{j}$ under Assumption \ref{ass:feas}. According to Lemma \ref{lem:Vstruct}, $\totv_{j}(\rho_{j})$ is concave in $\rho_{j}$ for any $j$, so the objective of $\textsc{CH-OPT}(\mathcal{I}_{\budg})$ maximizes a concave function. For the feasibility region, assume $\rho_{j}$ and $\rho_{j}'$ are feasible, then defining $\rho_{j}'' = \theta \rho_{j} +  (1-\theta)\rho_{j}'$ for any $\theta \in [0,1]$, we know that 
\begin{align*}
\begin{aligned}
     \sum_{j \in M} \left(\totv_{j}(\rho_{j}'') - \gamma  \rho_{j}''\right) 
     ~\overset{(i)}{\geq}~ &  \sum_{j \in M} \left(\theta\totv_{j}(\rho_{j})  +(1-\theta)\totv_{j}(\rho_{j}')  - \gamma  \rho_{j}''\right)\\
      ~=~ &  \theta\sum_{j \in M} \left(\totv_{j}(\rho_{j}) - \gamma  \rho_{j}\right) + (1-\theta)
     \sum_{j \in M} \left(\totv_{j}(\rho_{j}') - \gamma  \rho_{j}'\right)\\
       ~\overset{(ii)}{\geq}~ & 0
       \end{aligned}
\end{align*}
where (i) follows from concavity of $\totv_{j}(\rho_{j})$ and (ii) follows from feasiblity of $\rho_{j}$ and $\rho_{j}'$. On the other hand it is apparent that $\sum_{j\in [M]}\rho_{j}'' \leq\rho$. Hence we conclude that for any $\rho_{j}$ and $\rho_{j}'$  feasible,  $\rho_{j}'' = \theta \rho_{j} +  (1-\theta)\rho_{j}'$  is also feasible, so the feasible region of 
$\textsc{CH-OPT}(\mathcal{I}_{\budg})$ is convex. This concludes the statement of the proposition. \halmos
